Generating Private Synthetic Data with Genetic Algorithms

We study the problem of efficiently generating differentially private synthetic data that approximate the statistical properties of an underlying sensitive dataset. In recent years, there has been a growing line of work that approaches this problem using first-order optimization techniques. However, such techniques are restricted to optimizing differentiable objectives only, severely limiting the types of analyses that can be conducted. For example, first-order mechanisms have been primarily successful in approximating statistical queries only in the form of marginals for discrete data domains. In some cases, one can circumvent such issues by relaxing the task's objective to maintain differentiability. However, even when possible, these approaches impose a fundamental limitation in which modifications to the minimization problem become additional sources of error. Therefore, we propose Private-GSD, a private genetic algorithm based on zeroth-order optimization heuristics that do not require modifying the original objective. As a result, it avoids the aforementioned limitations of first-order optimization. We empirically evaluate Private-GSD against baseline algorithms on data derived from the American Community Survey across a variety of statistics--otherwise known as statistical queries--both for discrete and real-valued attributes. We show that Private-GSD outperforms the state-of-the-art methods on non-differential queries while matching accuracy in approximating differentiable ones.

==> Arxiv/algorithms/gsd_efficient.tex <==


\newcommand{\elite}{\mathcal{E}}

\begin{algorithm}[!htb]
\caption{Private Genetic Algorithm for Synthetic Data ($\GSD$) \label{alg:GSD}}
\begin{algorithmic}[1]
\STATE \textbf{Require:} The search space $\cX^{N'}$ of mixed-type synthetic datasets with $N'$ rows and $d$ features, number of generations $G$, population size $P$, elite  set size $E$.
\STATE \textbf{Input:} A set of $m$ queries $Q:\cX^* \rightarrow [0,1]^m$, (noisy) query answers $\hat{a}\in [0, 1]^m$.

\STATE Set the objective function for the synthetic datasets:
\begin{align*}
    L(\Dhat) = \| \hat{a} - Q(\Dhat)\|_2
\end{align*}

\STATE Initialize elite set $\elite_1 \leftarrow \{\Dbar_{1, i} \in \cX^{N'}: i \in [E]\}$ of synthetic datasets with $N'$ rows.
\FOR{$g = 1, \ldots, G$}
    
    \STATE Set $\Dhat^\star_{g} \leftarrow \argmin_{\Dhat \in \elite_{g}} L(\Dhat)$.

    \STATE  Define a population of $P+E$ synthetic datasets:
    $$\cP_g = \{\Dtil_{g, 1},\ldots, \Dtil_{g, P}\}\cup \elite_g$$
    where each member of $ \{\Dtil_{g, 1},\ldots, \Dtil_{g, P}\}$ is generated as follows:
    
    \FOR{$p=1, \ldots, P / 2$}
    
        \STATE \textbf{Mutate:} 
        Initialize $\Dtil_{g, p}$ equal to $\Dhat_g^\star$. Then, sample a row $i\sim U([N'])$, feature $j\sim U([d])$ and value  $v \sim U\pp{\cX_j}$.  Update  $\Dtil_{g, p}$ as follows:
        $$ \Dtil_{g, p}(i, j) \leftarrow v$$
    % \begin{align*}
    % \forall_{r\in [N'/2], c\in [d]}\quad 
    % \Dtil_{g, p}(r, c) = 
    %         \begin{cases} 
    %          v \sim U\pp{\cX_j} & \text{ if } r = i \text{ and } c = j \\ 
    %       \Dhat^\star_g(r, c) & \text{otherwise}
    %     \end{cases}  
    % \end{align*}


    \ENDFOR
    \FOR{$p=P/2+1, \ldots, P$}
        \STATE \textbf{Cross:}Initialize $\Dtil_{g, p}$ equal to $\Dhat_g^\star$. Then, sample two rows  $i_1, i_2\sim U([N'])$,  a feature $j\sim U([d])$, and elite member $\Dbar \sim U(\elite_g)$ and update  $\Dtil_{g, p}$ as follows: 
        $$\Dtil_{g, p}(i_1, j)  \leftarrow \Dbar(i_2, j) $$

        
%         \begin{align*}
% % \quad \text{such that}\quad 
% \forall_{r\in [N']\backslash [N'/2], c\in [d]} \quad 
% \Dtil_{g, p}(r, c) = 
%         \begin{cases}  \Dbar(i_2, c) & \text{ if } r = i_1 \text{ and } c = j \\ 
%       \Dhat^\star_g(r, c) & \text{otherwise}
%     \end{cases}  
% \end{align*}
    \ENDFOR
    \STATE Set $\elite_{g+1}$ as top $E$ members from population $\cP_g$  with respect to \emph{minimizing} objective $L(\cdot)$.
\ENDFOR
\STATE \textbf{return } $\Dhat_G^\star$
\end{algorithmic}
\end{algorithm}

==> Arxiv/algorithms/privga.tex <==

\newcommand{\elite}{\mathcal{E}}

\begin{algorithm}[!htb]
\caption{Private Genetic Algorithm ($\privGA$) \label{alg:privGA}}
\begin{algorithmic}[1]
\STATE \textbf{Require:} The search space $\cX^n$ of mixed-type synthetic datasets with $n$ rows and $d$ features, number of generations $G$, population size $N$, elite  set size $E$.
% crossover function $\gamma:\cX^n\times\cX^n\rightarrow\cX^n$, mutation function $\psi:\cX^n\rightarrow\cX^n$.
% number of synthetic rows $n'$,
% privacy parameter $\rho>0$. \\
% \STATE\textbf{Input:} Dataset $D$, $m$ statistical queries $Q$.

% \STATE Privatize statistics $\hat{a} \leftarrow Q(D) + \cN\pp{0, \frac{m}{2\rho}}$ and set objective function:
% \begin{align*}
%   f_{Q, \hat{a}}(\Dhat) = \|\hat{a} - Q(\Dhat) \|
% \end{align*}
\STATE \textbf{Input:} A set of $m$ queries $Q:\cX^n \rightarrow [0,1]^m$, (noisy) query answers $\hat{a}\in [0, 1]^m$.

\STATE Set the objective function for the synthetic datasets:
\begin{align*}
    L(\Dhat) = \| \hat{a} - Q(\Dhat)\|_2
\end{align*}

{{\color{blue}\# Define sparse-mutation and row-crossover functions. }}
\FUNCTION{ Sparse Mutation $\psi(\Dhat)$:}
\item Uniformly sample a row $r\in[n]$, a column $c\in[d]$  and a value $v \sim \cX_c$ from the domain of feature $c$.
\item \textbf{Output} $\Dhat_{\text{muta}}$ where the value of its $r$-th row and $c$-th column is $v$ and everywhere else is equal to $\Dhat$.
\ENDFUNCTION

\FUNCTION{ Row Crossover $\gamma(\Dhat_a, \Dhat_b)$:}
\item Uniformly sample two rows $r_a, r_b\in[n]$.
\item \textbf{Output} $\Dhat_{\text{cross}}$ having all rows from $\Dhat_a$, except row $r_a$ is placed by row $r_b$ from $\Dhat_b$ .
\ENDFUNCTION
% \STATE \textbf{function} $\psi_\sigma(\Dhat)$: \\   
% % On input $\Dhat\in \Theta$ 
%     \hspace{2mm}  Randomly select a row $r\in[n']$, a column $c\in[d]$  and  $z \sim \cN(0, \sigma^2)$.
%       \textbf{output} $\Dtil$ where its $i$-th row and $j$-th column is given by
%     \begin{align*}
%     \Dtil_{i,j} =
%     \begin{cases}
%     \Dhat_{i,j} + z & \text{if } i = r \text{ and } j = c \\
%     \Dhat_{i,j} & \text{otherwise } \\
%     \end{cases}
%     \end{align*}


{{\color{blue}\# Run genetic algorithm with $\psi$ and $\gamma$. }}
\STATE Initialize elite set $\elite_1 \leftarrow \{\Dhat_{1, i} \in \cX^n: i \in [E]\}$.
\FOR{$g = 1, \ldots, G$}
    
    %  \STATE {{\color{blue}\# Mutate each elite parameter}}
    % \FOR{$\theta_{elite} \in \elite $}
    %     \STATE Add mutation $\psi(\theta_{elite})$ to next generation $ \cP^{g}$.
    
    % \FOR{$j=1,\ldots N$}
        
    %     \STATE Randomly sample two elite members $a,b\in [E]$. 
    %     % two parents $\Dhat_{g}^a, \Dhat_{g}^b\in \elite_g$
    %     % \STATE Randomly select two parents $\Dhat_{g}^a, \Dhat_{g}^b\in \elite_g$
    %     \STATE Apply crossover and and then mutate result:
    %     $$\Dhat_{g, j}^{\text{cross}} \leftarrow \psi\pp{\gamma\pp{\Dhat_{g, a}, \Dhat_{g, b}}}$$
    %      % \STATE Add $\Dhat_{g}^{\text{cross}}$ to $ \cP_{g}$.
    % \ENDFOR
    \STATE  Define a population of $N+E$ synthetic datasets:
    $$\cP_g = \{\Dhat_{g, 1}^{\text{cross}},\ldots, \Dhat_{g, N}^{\text{cross}}\}\cup \elite_g$$
    where each $\Dhat_{g, j}^{\text{cross}}$ is constructed by sampling two elite members  $a,b\in [E]$ and then applying crossover and and then mutating:
    %
    $$\Dhat_{g, j}^{\text{cross}} \leftarrow \psi\pp{\gamma\pp{\Dhat_{g, a}, \Dhat_{g, b}}}$$
    \STATE Set $\elite_{g+1}$ as top $E$ members from population $\cP_g$ that \emph{minimize} objective $L(\cdot)$.

   % \STATE {{\color{blue}\#  Find parameter from  $\cP^{g-1}$ that minimizes $L$}}
   %  \STATE Set elite $\Dhat^g_\star\leftarrow \argmin_{\theta\in \cP^{g-1}} L(\theta)$
   %  \STATE Add $\theta^g_\star$ to next generation $\cP^{g}$.
   %  \STATE {{\color{blue}\#  Choose best $T$ from $\cP^{g-1}$ to define the {\em elite} set.}}


    
    % \STATE Add $\Dhat^g_\star$ to $\cP^{g}$.
    % \STATE {{\color{blue}/\ /\ The next generation includes the $N-T-1$ off-spring, the  and the elite parameter }}
    % \STATE Set $\cP^g \leftarrow \{\theta_1,\ldots \theta_{N-T-1}\}\uplus \text{Elite}_{g} \uplus\{\theta^g_\star\}$.
\ENDFOR
\STATE \textbf{return} $\Dhat_\star\leftarrow \argmin_{\Dhat\in \elite_{g+1}} L(\Dhat)${{\color{blue}\# best from $\elite_{g+1}$.}}
\end{algorithmic}
\end{algorithm}

==> Arxiv/algorithms/rap++.tex <==
\newcommand{\qtil}{\tilde{q}}
\begin{algorithm}[t]
\small
\begin{algorithmic}[1]
\caption{Relaxed Projection with Sigmoid Temperature Annealing}\label{alg:rappp}
% \Require   
% Let $\widetilde{\cX}\subseteq [0,1]^d$ be a relaxed data domain with dimension $d$.  
% For any query $q:\cX\rightarrow \{0,1\}^{*}$, let $\qtil: \widetilde{\cX} \times \mathbb{Z}^{+}\rightarrow [0,1]^{*}$ be its continuous \textit{Sigmoid approximation}.
\STATE \textbf{Input: } A set of $m$ sigmoid differentiable queries $\{\tilde{q}^{[\cdot]}_i\}_{i\in [m]}$, a set of $m$ target answers $\hat{a}=\{\hat{a}_i \}_{i\in [m]}$, initial inverse temperature $\sigma_1\in\mathbb{R}^+$, stopping condition $\gamma>0$, and initial dataset $\widehat{D}_1$.


% \State Initialize the loss function $L:\widetilde{\cX}^{n'}\times \mathbb{Z}^{+} \rightarrow[0,1]$:
    % $\Loss_Q(D', \sigma) = \frac{1}{|Q|} \sum_{q\in Q} \|q(D) - \qtil(D', \sigma) \|_2$ \ar{This should be defined in terms of $\hat a$ not $q(D)$ right?} \gv{Yes. will fix it.}

% \State Initialize $\widehat{D}_1 \in \mathbb{R}^{\hat{n}}$.

\FOR{$j=1$ \textbf{ to } $J$}
% \State Compute gradient: $g_t \leftarrow \nabla \Loss_2(D_{t-1}^{'},  \sigma_0 \cdot 2^{k})$ 
% \State Update: $D_{t}^{'} \leftarrow \sparsemax\pp{D_{t-1}^{'} - \alpha \cdot g_t}$ \ar{What is this? I thought we were using the ADAM optimizer?}  \gv{Yes. will fix it.}
% \State SparseMax and clip.
\STATE Set inverse temperature $\sigma_j = \sigma_1 \cdot 2^{j-1}$.
\STATE Define the sigmoid differentiable loss function: 
%
$    \Loss_j(\widehat{D}) = \sum_{i \in [m]} \left( \qtil^{[\sigma_j]}_i(\widehat{D}) - \hat{a}_i \right)^2$
%
\STATE  Starting with $\widehat{D}\leftarrow \widehat{D}_j$.
% update $\widehat{D}$ using 
Run  gradient descent on $L_j({\widehat{D}})$ until    $\|\nabla \Loss_j(\widehat{D})\| \leq \gamma$.
%
Set $\widehat{D}_{j+1} \leftarrow \widehat{D}$.
\ENDFOR
\STATE \textbf{Output} $\widehat{D}_{J+1}$
\end{algorithmic}
\end{algorithm}

==> Arxiv/docs/dp.tex <==
\section{Additional preliminaries}
\begin{definition}[Exponential Mechanism]\label{def:exponential}
Given some dataset $D\in \cX^*$, arbitrary range $\mathcal{R}$, and score function $S: \mathcal{X}^*\times\mathcal{R}\rightarrow\mathbb{R}$, the exponential mechanism $\mathcal{M}_E(D,S,\mathcal{R},\varepsilon)$ selects and outputs an element $r\in\mathcal{R}$ with probability proportional to $\exp\pp{\frac{\varepsilon S(D,r)}{2\Delta_S}},$ where $\Delta_S$
 is the sensitivity of $S$.
 \end{definition}
 


==> icml/algorithms/muta_and_cross.tex <==

\begin{algorithm}[tb]
\caption{Private Genetic Algorithm (\privGA) for Synthetic Data   \label{alg:privGA}}
\begin{algorithmic}[1]
% \STATE \textbf{Require:} Number of generations $G$, Population size $N$, Elite  set $T$, Crossover function $\gamma:\Theta\times\Theta\rightarrow\Theta$, mutation function $\psi:\Theta\rightarrow\Theta$. 
% number of synthetic rows $n'$,
% privacy parameter $\rho>0$. \\
\STATE \textbf{Require:} Synthetic data size $n'$,  mutation strength $\sigma$.
\STATE\textbf{Input:} Dataset $D\in\cX^n$ with $n$ rows and $d$ columns, $m$ statistical queries $Q:\cX^{\star} \rightarrow [0,1]^m$, privacy parameter $\rho$.

\STATE Approximate statistics with Gaussian mechanism: 
$$\hat{a} \leftarrow Q(D) + \cN\pp{0, \tfrac{m}{2 n \cdot \rho}}$$


\STATE {Define} parameter space $\Theta= [0,1]^{n'\times d}$



\STATE Define objective function $L_{\hat{a}, Q}$ as in equation \eqref{eq:obj}.
% \begin{align*}
%   f_{Q, \hat{a}}(\Dhat) = \|\hat{a} - Q(\Dhat) \|
% \end{align*}

\STATE {\color{blue} \# Define \underline{crossover} function}
\STATE \textbf{function}  $\gamma(D_a, D_b)$: On input $D_a, D_b\in \Theta$  of size $n'$ \label{line:crossoverdef}
\begin{enumerate}
    \item Combine rows $D_{ab} = D_a \uplus D_b$.
    \item  \textbf{output} a random sample of size $n'$ from $D_{ab}$.
\end{enumerate}

\STATE {\color{blue} \# Define \underline{sparse mutation} function with parameter $\sigma$}
\label{line:mutationdef}
\STATE \textbf{function} $\psi_\sigma(\Dhat)$:  On input $\Dhat\in \Theta$ 
\begin{enumerate}
    \item Randomly select a row $r\in[n']$, a column $c\in[d]$  and  $z \sim \cN(0, \sigma^2)$.
    \item  \textbf{output} $\Dtil$ where its $i$-th row and $j$-th column is given by
    \begin{align*}
    \Dtil_{i,j} =
    \begin{cases}
    \Dhat_{i,j} + z & \text{if } i = r \text{ and } j = c \\
    \Dhat_{i,j} & \text{otherwise } \\
    \end{cases}
    \end{align*}
\end{enumerate}

\item Run \simpleGA{}:
\begin{align*}
    \Dhat \leftarrow \simpleGA(\Theta, L_{\hat{a}, Q }, \gamma, \psi_\sigma)
\end{align*}

\STATE \textbf{return} $\Dhat$
\end{algorithmic}
\end{algorithm}

==> icml/algorithms/privga.tex <==

% \newcommand{\elite}{\mathcal{E}}

\begin{algorithm}[!htb]
\caption{Private Genetic Algorithm ($\privGA$) \label{alg:privGA}}
\begin{algorithmic}[1]
\STATE \textbf{Require:} The search space $\cX^n$ of mixed-type synthetic datasets with $n$ rows and $d$ features, number of generations $G$, population size $N$, elite  set size $E$.
% crossover function $\gamma:\cX^n\times\cX^n\rightarrow\cX^n$, mutation function $\psi:\cX^n\rightarrow\cX^n$.
% number of synthetic rows $n'$,
% privacy parameter $\rho>0$. \\
% \STATE\textbf{Input:} Dataset $D$, $m$ statistical queries $Q$.

% \STATE Privatize statistics $\hat{a} \leftarrow Q(D) + \cN\pp{0, \frac{m}{2\rho}}$ and set objective function:
% \begin{align*}
%   f_{Q, \hat{a}}(\Dhat) = \|\hat{a} - Q(\Dhat) \|
% \end{align*}
\STATE \textbf{Input:} A set of $m$ queries $Q:\cX^n \rightarrow [0,1]^m$, (noisy) query answers $\hat{a}\in [0, 1]^m$.

\STATE Set the objective function for the synthetic datasets:
\begin{align*}
    L(\Dhat) = \| \hat{a} - Q(\Dhat)\|_2
\end{align*}

{{\color{blue}\# Define sparse-mutation and row-crossover functions. }}
\FUNCTION{ Sparse Mutation $\psi(\Dhat)$:}
\item Uniformly sample a row $r\in[n]$, a column $c\in[d]$  and a value $v \sim \cX_c$ from the domain of feature $c$.
\item \textbf{Output} $\Dhat_{\text{muta}}$ where the value of its $r$-th row and $c$-th column is $v$ and everywhere else is equal to $\Dhat$.
\ENDFUNCTION

\FUNCTION{ Row Crossover $\gamma(\Dhat_a, \Dhat_b)$:}
\item Uniformly sample two rows $r_a, r_b\in[n]$.
\item \textbf{Output} $\Dhat_{\text{cross}}$ having all rows from $\Dhat_a$, except row $r_a$ is placed by row $r_b$ from $\Dhat_b$ .
\ENDFUNCTION
% \STATE \textbf{function} $\psi_\sigma(\Dhat)$: \\   
% % On input $\Dhat\in \Theta$ 
%     \hspace{2mm}  Randomly select a row $r\in[n']$, a column $c\in[d]$  and  $z \sim \cN(0, \sigma^2)$.
%       \textbf{output} $\Dtil$ where its $i$-th row and $j$-th column is given by
%     \begin{align*}
%     \Dtil_{i,j} =
%     \begin{cases}
%     \Dhat_{i,j} + z & \text{if } i = r \text{ and } j = c \\
%     \Dhat_{i,j} & \text{otherwise } \\
%     \end{cases}
%     \end{align*}


{{\color{blue}\# Run genetic algorithm with $\psi$ and $\gamma$. }}
\STATE Initialize elite set $\elite_1 \leftarrow \{\Dhat_{1, i} \in \cX^n: i \in [E]\}$.
\FOR{$g = 1, \ldots, G$}
    
    %  \STATE {{\color{blue}\# Mutate each elite parameter}}
    % \FOR{$\theta_{elite} \in \elite $}
    %     \STATE Add mutation $\psi(\theta_{elite})$ to next generation $ \cP^{g}$.
    
    % \FOR{$j=1,\ldots N$}
        
    %     \STATE Randomly sample two elite members $a,b\in [E]$. 
    %     % two parents $\Dhat_{g}^a, \Dhat_{g}^b\in \elite_g$
    %     % \STATE Randomly select two parents $\Dhat_{g}^a, \Dhat_{g}^b\in \elite_g$
    %     \STATE Apply crossover and and then mutate result:
    %     $$\Dhat_{g, j}^{\text{cross}} \leftarrow \psi\pp{\gamma\pp{\Dhat_{g, a}, \Dhat_{g, b}}}$$
    %      % \STATE Add $\Dhat_{g}^{\text{cross}}$ to $ \cP_{g}$.
    % \ENDFOR
    \STATE  Define a population of $N+E$ synthetic datasets:
    $$\cP_g = \{\Dhat_{g, 1}^{\text{cross}},\ldots, \Dhat_{g, N}^{\text{cross}}\}\cup \elite_g$$
    where each $\Dhat_{g, j}^{\text{cross}}$ is constructed by sampling two elite members  $a,b\in [E]$ and then applying crossover and and then mutating:
    %
    $$\Dhat_{g, j}^{\text{cross}} \leftarrow \psi\pp{\gamma\pp{\Dhat_{g, a}, \Dhat_{g, b}}}$$
    \STATE Set $\elite_{g+1}$ as top $E$ members from population $\cP_g$ that \emph{minimize} objective $L(\cdot)$.

   % \STATE {{\color{blue}\#  Find parameter from  $\cP^{g-1}$ that minimizes $L$}}
   %  \STATE Set elite $\Dhat^g_\star\leftarrow \argmin_{\theta\in \cP^{g-1}} L(\theta)$
   %  \STATE Add $\theta^g_\star$ to next generation $\cP^{g}$.
   %  \STATE {{\color{blue}\#  Choose best $T$ from $\cP^{g-1}$ to define the {\em elite} set.}}


    
    % \STATE Add $\Dhat^g_\star$ to $\cP^{g}$.
    % \STATE {{\color{blue}/\ /\ The next generation includes the $N-T-1$ off-spring, the  and the elite parameter }}
    % \STATE Set $\cP^g \leftarrow \{\theta_1,\ldots \theta_{N-T-1}\}\uplus \text{Elite}_{g} \uplus\{\theta^g_\star\}$.
\ENDFOR
\STATE \textbf{return} $\Dhat_\star\leftarrow \argmin_{\Dhat\in \elite_{g+1}} L(\Dhat)${{\color{blue}\# best from $\elite_{g+1}$.}}
\end{algorithmic}
\end{algorithm}

==> icml/docs/PrivGA.tex <==
\section{Private Genetic Algorithm (\privGA)}

We propose a genetic algorithm, $\privGA$, for learning synthetic data that minimizes the objective outlined in Equation \ref{eq:obj} to match a set of noisy statistical properties. Furthermore, the \privGA{} mechanism can be used in the adaptive framework to satisfy differential privacy. Below, we state the formal privacy guarantee of \privGA{}, which directly follows from \cref{thm:privacy}.

\begin{corollary}\label{thm:privgaguarantee} 
% For any quer
For any $\rho>0$, dataset $D$, and query set $Q$.
Running \privGA{} (\cref{alg:privGA}) under the adaptive framework satisfies $\rho$-zCDP and  $(\varepsilon, \delta)$-differential privacy for: $\varepsilon = \rho+2\sqrt{\rho\cdot \log(1/\delta)}$.
\end{corollary}

The \privGA{}  mechanism builds upon the genetic algorithm, $\simpleGA$ \citep{such2017deep}. A genetic algorithm is a method for exploring large parameter spaces through the principle of survival of the fittest to identify suitable candidate solutions for a given optimization objective. Despite the simplicity of the $\simpleGA$ algorithm, it has been demonstrated to be an effective method for training significant neural network architectures and outperforms gradient-based methods in some cases.


The standard genetic optimization process of $\privGA$ is outlined in Algorithm \ref{alg:privGA}. It commences with an initial population of $E$ elite individuals and operates over $G$ generations. At each generation, the genetic algorithm generates numerous candidates by perturbing the parameters of the elite population and ranks them according to the objective of matching noisy statistics. The top $E$ candidates then become the new elite set for the next generation. The final output is a  dataset from the elite set of the last generation, that best matches the noisy statistics.

The \privGA{} mechanism introduces two crucial modifications of the perturbation step in the standard genetic framework: \emph{sparse mutations} and \emph{row crossover}. The sparse mutation strategy is designed to discover new high-quality synthetic rows through a random search to progress toward the objective of matching statistics. Meanwhile, the principle of row crossover is to recycle high-quality rows for subsequent generations. Our proposed row crossover technique significantly enhances the convergence rate towards the objective of matching statistics, as demonstrated in Figure \ref{fig:convergence}, where $\privGA$ took approximately 15,000 generations to converge to a solution with low error. 

% The key feature of this strategy is that it only perturbs a single optimization parameter to generate a new candidate synthetic data, as opposed to the random search method proposed by \citet{such2017deep}, which applies mutation overall population parameters. This approach stabilizes the optimization process by allowing it to find and maintain high-quality synthetic rows. Figure \ref{fig:convergence} illustrates how this strategy makes steady progress towards the objective, although convergence is slow.

% Our proposed row crossover technique significantly enhances the convergence rate towards the objective of matching statistics, as demonstrated in Figure \ref{fig:convergence}. The dotted line in Figure \ref{fig:convergence} represents the performance of $\privGA$ without crossover, and the solid line represents the performance of $\privGA$ with crossover. The results clearly show the substantial improvement in convergence rate obtained through the incorporation of row crossover. 

% The fundamental principle behind row crossover is recycling high-quality rows for subsequent generations via randomly combining rows of data between synthetic datasets. As a result, high-quality synthetic rows are more likely to be repeated in future generations. We extend the intuition of how crossover works in \cref{sec:crossover}.


% \subsection{The Standard Genetic Strategy and Efficiency}
% The genetic optimization process of $\privGA$ is outlined in Algorithm \ref{alg:privGA}. It commences with an initial population of $E$ elite individuals and operates over $G$ generations. At each generation, the genetic algorithm generates numerous candidates by perturbing the parameters of the elite population and ranks them according to the objective of matching noisy statistics. The top $E$ candidates then become the new elite set for the next generation. The final output is the optimal dataset from the elite set of the last generation.

% We demonstrate that $\privGA$ is an efficient algorithm for learning synthetic datasets. Our proposed row crossover technique significantly enhances the convergence rate towards the objective of matching statistics, as demonstrated in Figure \ref{fig:convergence}. In Figure \ref{fig:convergence}, $\privGA$ took approximately 15,000 generations to converge to a solution with low error. This example involves evolving a synthetic dataset with 13 features and 2000 rows to match a set of 5000 statistics. 


% \gvcomment{Runtime bottleneck is evaluating the statistics}





% \subsection{\privGA: \simpleGA{} for Private Synthetic Data}
% % The algorithm \ref{alg:simpleGA} is general enough to solve a variate of hard optimization problem. Then, 
% For a dataset $D$ and a set of queries $Q$,  this section shows how to find a synthetic dataset with the same schema as $D$ whose answers are close to $Q(D)$ using the {\em zeroth}-order optimization procedure described in algorithm \ref{alg:simpleGA}. Essentially, our solution \privGA{}, described in algorithm \ref{alg:privGA},  runs \simpleGA{} with parameter space $\Theta=[0,1]^{n'\times d}$ \footnote{The data dimension is $d$. Moreover, the number of synthetic data rows is parameter $n'$. In practice, we choose $n'=100$ as it works well for all cases}\textemdash The parameter space $\Theta$ encodes the space of all datasets with $n'$ rows and $d$ features\textemdash and the objective function $L_{\hat{a}, Q}$ (as defined in equation \eqref{eq:obj}). The choice of parameter space $\Theta$ and loss function $L_{\hat{a}, Q}$ signal the \simpleGA{} algorithm to search the space of datasets to find one that best explains the approximate private statistics $\hat{a}$
%

% A key characteristic of \privGA{} that separates it from \simpleGA, is the choice of  {\em crossover} and {\em mutation} functions for evolving synthetic datasets. 
% These two functions control how the generations of synthetic are created. 

% The genetic strategy is very simple to implement,   

% \begin{wrapfigure}{r}{0.27\textwidth}
%   \begin{center}
%     \includegraphics[width=0.27\textwidth]{icml/images/convergence.png}
%   \end{center}
%   \caption{Convergence of \privGA{} using only \emph{sparse mutations} vs using \emph{row-crossover}. We conduct this experiments with $\varepsilon=1$ on \acsmob, which we describe later in Section \ref{sec:data}. Queries are $2$-way range marginals.}
% \label{fig:convergence}
% \end{wrapfigure}

\begin{figure}
    \centering
    \includegraphics[width=0.80\linewidth]{images/convergence.png}
     \caption{Convergence of \privGA{} using only \emph{sparse mutations} vs using \emph{row-crossover}. We conduct these experiments with $\varepsilon=1$ on \acsmob, which we describe later in Section \ref{sec:data}. Queries are $2$-way range marginals.}
\label{fig:convergence}
\end{figure}



\paragraph{Accuracy.} We note that \privGA{} inherits the  same accuracy bounds of  the \rap{} mechanism \cite{aydore2021differentially}, under the conditions that the optimization process completes exactly.  We state the formal guarantee in the Theorem \ref{thm:accurayAppendix} of the appendix. 


% \subsection{Sparse Mutation} \label{sec:mutations}
\paragraph{Sparse Mutation.} 
The purpose of mutations in the \privGA{} mechanism is to find high-quality synthetic rows by doing a random search over the data schema.  The original simple genetic algorithm proposed by \citet{such2017deep}  employs the use of independent Gaussian noise with a variance of $\sigma^2$ to mutate the population parameters. However, we find that this approach of perturbing all parameters is not stable for optimizing over synthetic datasets and  often fails to converge. 


In order to address this issue, a crucial component of our mechanism \privGA{} for synthetic dataset search is the implementation of a highly sparse mutation strategy for the population parameters encoding synthetic datasets. Specifically, when mutating a dataset $\Dhat_g$ in generation $g$, our strategy preserves the majority of high-quality rows in $\Dhat_g$, and only perturbs a single row to generate a candidate dataset $\Dhat_{g+1}$ for the next generation. 
% The other important advantage is computational. By only mutating a single row, we only need to recompute  the statistics of the row before  
% The produced synthetic datasets are then evaluated 

% To explain the intuition behind the sparse mutation strategy, we define a 
% high-quality synthetic row as one that is close to rows of the real dataset. To produce a new synthetic data candidate, the sparse mutation takes an elite dataset and mutates a single row chosen uniformly at random. If the chosen row is high quality then it is more likely that the synthetic data score will decrease and will be more likely to be discarded. Therefore, synthetic datasets that  survive will are likely to preserve already high-quality rows. In contrast, perturbing all rows can have the effect of erasing  the progress made in previous generations to find good synthetic rows.


% \subsection{Crossover}\label{sec:crossover} 
\paragraph{Crossover.} 

% The crossover function is a randomized function that we denote by $\gamma:\cX^n \times \cX^n\rightarrow \cX^n$. It takes as input two datasets and outputs an offspring dataset that combines the rows of its parents. The purpose of crossover is to pass down high-quality rows to future generations. 

% To perform a crossover operation, \privGA{} samples a pair of synthetic datasets $\Dhat_a$ and $\Dhat_b$  from the elite set and samples a row $r_a$ from $\Dhat_a$ and a row $r_b$ from $\Dhat_b$. Then, sets  $\Dhat^{\text{cross}} \leftarrow \Dhat_a$ and replaces row $r_a$ in $\Dhat^{\text{cross}} $ with $r_b$. Finally, it outputs $\Dhat^{\text{cross}}$. The idea is that since $r_b$ belonged to an elite synthetic dataset $\Dhat_b$, there is a chance that $r_b$ is a high-quality row, thus, replacing it into $\Dhat_a$ could improve its score in the objective. The crossover stop greatly improves convergence because, once the mutation step finds a well-fitting row, the crossover takes charge in reproducing it many times while it helps improve the score of datasets. 


The crossover function is a randomized function that we denote by $\gamma:\cX^n \times \cX^n\rightarrow \cX^n$. It takes two datasets as input and produces a new dataset that combines the rows of the inputs. The primary purpose of crossover is to pass down high-quality rows to future generations in the genetic process.

The crossover operation in \privGA{} is executed as follows: a pair of synthetic datasets, $\Dhat_a$, and $\Dhat_b$ are sampled from the elite set. Subsequently, a row, $r_a$, is sampled from $\Dhat_a$ and another row, $r_b$, is sampled from $\Dhat_b$. The dataset $\Dhat^{\text{cross}}$ is initialized as $\Dhat_a$, and the row $r_a$ is replaced with $r_b$ in $\Dhat^{\text{cross}}$. Finally, the resulting dataset $\Dhat^{\text{cross}}$ is output.

The rationale behind this process is that since $r_b$ belonged to an elite synthetic dataset $\Dhat_b$, there is a high likelihood that $r_b$ is a high-quality row. As a result, replacing it with $r_a$ in $\Dhat_a$ has the potential to improve its score in the objective function. The crossover operation significantly improves convergence by reproducing high-quality rows if they help improve the datasets' scores.

% \subsection{Accuracy Analysis} 
% % Our mechanism inherits the oracle accuracy guarantees proven by \citet{aydore2021differentially}. However, the accuracy of \citet{aydore2021differentially} is slightly worse error due to their objective relaxation. We state our oracle guarantee here and defer the proof to the appendix.
% \citet{bun2015differentially} shows that it is not possible to approximate prefix queries  under differential privacy. However, we provide an error analysis that is based on the assumption that the optimization routine succeeds in finding the optimal. An oracle-guarantee was also provided  in \citet{aydore2021differentially} for the RAP algorithm.



% \begin{theorem}Condition of the succes of the optimization. The error of \privGA{} is bounded by:
% \begin{align*} 
%     \sqrt{\frac{1}{m}\|Q(D) - Q(D') \|}\leq \alpha 
% \end{align*}
% with $\alpha = O\pp{\frac{\log(\cX) \log(n') }{\sqrt{\epsilon \cdot n }}}$
% \end{theorem}

% \begin{proof}

% \end{proof}



% \begin{figure}
%     \centering
%     \includegraphics[width=0.30\textwidth]{icml/images/convergence.png}
%     \caption{The dotted line demonstrates the slow convergence of \privGA{}  using only the \emph{sparse mutation} strategy. Then solid line shows how activating \emph{row-crossover} with \emph{sparse mutation} can dramatically speed up convergence. Input data is \acsmob{}(See Table \ref{tab:acs_data_attributes}), $\epsilon=1$ and queries are $2$-way marginals.}
%     \label{fig:convergence}
% \end{figure}

% Despite the improved bounds in \cref{thm:accuray} from the bounds in \citet{aydore2021differentially}, there is no guarantee about the performance of the optimization of \privGA{}. 
% However, we empirically show that the \privGA{} shows comparable performance to \rap{} over many different datasets.

%
% \begin{theorem}\label{thm:accuray}
% For a discrete data domain $\cX$ and any dataset $D$ with $n$ rows.
% Fix privacy parameters  $\rho$, a synthetic dataset size $n'$, and any set of $m$ queries $Q$. If the minimization in the projection step is solved exactly, then 
% the one-shot \privGA{} mechanism outputs a synthetic data $\Dhat$ with
%  average error bounded as
% \begin{align*}
%    \sqrt{\|\tfrac{1}{m} Q(D) - Q(\Dhat) \|_2^2} \leq \\
%    O\pp{
%    \frac{
%     \pp{\pp{\log(|\cX|/\beta}{\sqrt{\varepsilon\cdot n}}}^{1/4}
%    }{\sqrt{\epsilon\cdot n }}
%    + \frac{\log(k)}{\sqrt{n'}}
%    }
% \end{align*}
% \end{theorem}



==> icml/docs/accuracy.tex <==
\section{Accuracy Analysis of \privGA{}}

Our mechanism inherits similar oracle accuracy guarantees of the (non-adaptive) \rap{} mechanism, which were proven in \citet{aydore2021differentially}. 
% In the adaptive selection framework, the report noisy max (\cref{def:rnm}) and Gaussian mechanism (GM, \cref{def:gaussian}) are both called $K$ times, each with a privacy budget of $\rho' = \rho / (2\cdot K)$. As shown in \cref{def:gaussian} and the work of \citet{durfee2019practical}, each individual call to EM or GM satisfies $(\tfrac{\rho'}{2})$-zCDP. Thus, by the composition properties outlined in \citet{bun2016concentrated}, the combination of $2\cdot K$ $\rho'$-zCDP mechanisms satisfies $\rho$-zCDP.




\begin{theorem}\label{thm:accurayAppendix}
For a discrete data domain $\cX$ and any dataset $D\in\cX^n$ with $n$ rows.
Fix privacy parameters  $\epsilon, \delta>0$, a synthetic dataset size $n'$, and any set of $m$ queries $Q:\cX^*\rightarrow[0,1]^m$. If the one-shot \privGA{} mechanism solves the minimization in the projection step exactly, then 
the one-shot \privGA{} mechanism outputs a synthetic data $\Dhat$ with
 average error bounded as
\begin{align*}
  \sqrt{\tfrac{1}{m} \| Q(D) - Q(\Dhat) \|_2^2} \leq 
   O\pp{
   \frac{
    \pp{(\log(|\cX|/\beta)\ln(1/\delta)}^{1/4}
   }{\sqrt{\epsilon\cdot n }}
   + \frac{\log(m)}{\sqrt{n'}}
   }
\end{align*}
\end{theorem}
\begin{proof}
We follow the projection mechanism, which has the following guarantee proven by \citet{NKL}. Consider the discrete data domain $\cX$ . Let $\cX^*$ be the set of datasets of arbitrary size with rows from the domain $\cX$.

The projection mechanism by \citet{NKL}, perturbs the answers of $Q$ using the Gaussian mechanism to obtain $\hat{a} $, and then finds a synthetic dataset $\Dhat^*$ by solving the following objective
% %
\begin{align*}
    \Dhat^* \leftarrow \argmin_{\Dhat \in \cX^*} \|\hat{a} - Q(\Dhat)\|
\end{align*}
% %
with the following accuracy guarantee:
\begin{align*}
    \sqrt{ \tfrac{1}{m}\| Q(D) - Q(\Dhat^*) \|_2^2} \leq \alpha  = O\pp{\frac{\pp{\ln(|\cX| /\beta)\ln(1/\delta)}^{1/4}}{\sqrt{\epsilon\cdot n}}} 
\end{align*}

Next, let $m$ be the number of queries in $Q$.
By a simple sampling argument, proven in Lemma 3.7 of \citet{BLR08}, there exists a dataset $\Dhat$ of size $n'$ that satisfies the following:
\begin{align*}
     \|Q(\Dhat) - Q(\Dhat^*)\|_{\infty} \leq \sqrt{\frac{\log(m)}{n'}}
\end{align*}

The next step is by triangle inequality:
\begin{align*}
    \sqrt{ \tfrac{1}{m}\| Q(D) - Q(\Dhat) \|_2^2}
    &= \sqrt{ \tfrac{1}{m}\| Q(D) - Q(\Dhat^*) + Q(\Dhat^*) - Q(\Dhat) \|_2^2} \\
    %
    &\leq  \sqrt{ \tfrac{1}{m}\| Q(D) - Q(\Dhat^*) \|_2^2} + \sqrt{ \tfrac{1}{m}\|  Q(\Dhat^*) - Q(\Dhat) \|_2^2} && (\text{Triangle inequality})\\
    &\leq \sqrt{ \tfrac{1}{m}\| Q(D) - Q(\Dhat^*) \|_2^2} + \|Q(\Dhat) - Q(\Dhat^*)\|_{\infty} \\
    %
    &\leq O\pp{\frac{\pp{\ln(|\cX| /\beta)\ln(1/\delta)}^{1/4}}{\sqrt{\epsilon\cdot n}}}  + \sqrt{\frac{\log(m)}{n'}} \\
    % &\leq \sqrt{ \|\tfrac{1}{m} Q(D) - Q(\Dhat^*) \|_2^2}
    % + \|Q(\Dhat) - Q(\Dhat^*)\|_{\infty} 
\end{align*}
\end{proof}


Despite the bounds in \cref{thm:accurayAppendix} matching from the bounds in \citet{aydore2021differentially}, there is no guarantee about the performance \privGA{}'s optimization. Therefore, we empirically show that \privGA{} has comparable performance to \rap{} on matching marginal statistics over many different datasets.
In Tables \ref{tab:oneshot}, we provide results on categorical marginals and with different ACS tasks as defined in Table \ref{tab:acs_data_attributes}. This brief experiment also shows that, like in the adaptive setting, \privGA{} achieves similar performance to \rap{} on differentiable queries in the one-shot setting across many datasets. We use the same hyperparameters used in our adaptive experiments (Table \ref{tab:hyperparameters}), excluding our choices for $T$, which are not applicable in the one-shot setting.

\begin{table}[!htb]
\centering
\caption{Max and average error of one-shot mechanism ($\varepsilon=1$) with $2$-way categorical marginal queries for all ACS tasks. We also list the number of workloads for each task.}
\label{tab:oneshot}
    \begin{tabular}{l c | c c | c c }
    \toprule
    & & \multicolumn{2}{c}{Max} & \multicolumn{2}{c}{Average}\\
    & \# workloads & \rap{} & \privGA{} & \rap{} & \privGA{} \\
    \midrule
    \acsmob & 136 & 0.003005 & 0.004651 & 0.0004527 & 0.0005363 \\ 
    \acsinc & 36 & 0.002794 & 0.002722 & 0.0000208 & 0.0000341 \\ 
    \acsemp & 120 & 0.001288 & 0.003562 & 0.0001768 & 0.0003468 \\
    \acstra & 91 & 0.003919 & 0.004954 & 0.0000317 & 0.0000480 \\ 
    \acscov & 136 & 0.002156 & 0.003916 & 0.0003193 & 0.0004279 \\
    \bottomrule
\end{tabular}
\end{table}

==> icml/docs/algorithm_details.tex <==
\section{Additional algorithm details}

\subsection{Adaptive Selection}\label{appx:adaptive}

We present the Adaptive Selection framework in Algorithm \ref{alg:adaptive}, and also provide its privacy proof below.

\input{icml/algorithms/adaptive_framework.tex}

% We provide a proof sketch to Theorem \ref{thm:privacy} below.
% \begin{proof}
% \gvcomment{complete}
% \end{proof}

\subsection{\rappp{} and its limitations}\label{appx:rappp}
\input{icml/docs/rap++_v2.tex}

\subsection{Modifications to \rap{} / \gem{}}\label{appx:rapgem}

Suppose we have a data domain $\gX = \gX_1 \times \ldots \times \gX_d$ contains $d$ discrete attributes. Then both \rap{} and \gem{} model such features as a mixture of $K$ product distributions over attributes $\gX_i$ (and possible values they can take on). We denote each product distribution as $P_i = \prod_{j=1}^d P_{ij}$, where $P_{ij}$ is a distribution over the discrete values of $\gX_j$. The difference between \rap{} and \gem{} then is how each distribution $P_{ij}$ is parametrized. In \rap, the parameters $\theta$ are exactly the values $P_{ij}$. Meanwhile, \gem{} instead outputs the values $P_{ij}$ using a neural network $F_{\theta}$, which takes in as input Gaussian noise $\mathbf{z} \sim \mathcal{N}\left(0, I_K \right)$.

In either case, query answers for $k$-way categorical queries can be calculated as a product over various columns in $P_i$. For example (relaxing notation), suppose $P_{i, \textrm{COLOR}=\textrm{red}}$ and $P_{i, \textrm{SHAPE}=\textrm{circle}}$ correspond to the probabilities that attributes $\textrm{COLOR}=\textrm{red}$ and $\textrm{SHAPE}=\textrm{circle}$. Then the 2-way marginal query counting the proportion of samples that are red circles can be written down as the product query $\frac{1}{K} \sum_{i=1}^{K} P_{i, \textrm{COLOR}=\textrm{red}} \times P_{i, \textrm{SHAPE}=\textrm{circle}}$.

Now suppose we have some numerical column that has been discretized into bins. Then a $k$-way range marginal query can be simple written down as a sum of product queries. For example, suppose we have an attribute QUANTITY that has been discretized into bins of size 10. Then the $2$-way range query for proportion of samples that are red and have quantity between 1 and 20 can be written down as $\frac{1}{K} \sum_{i=1}^{K} P_{i, \textrm{COLOR}=\textrm{red}} \times \left[ P_{i, \textrm{QTY}=\textrm{1-10}} + P_{i, \textrm{QTY}=\textrm{11-20}} \right]$. Therefore, we are able to still optimize over such queries, since they are simply sums over (differentiable) product queries that the algorithms were originally designed for.

Finally, while \citet{aydore2021differentially} and \citet{liu2021iterative} propose different optimization strategies for their algorithms at each round, we introduce a simpler update procedure that we find performs well across our experiments. We present this procedure in Algorithm \ref{alg:rapgem_update}.

\begin{algorithm}[!tbh]
\caption{\rap{} / \gem{} Update}
\label{alg:rapgem_update}
\begin{algorithmic}
\STATE {\bfseries Input:} $\rap{}/\gem{}_\theta$, queries (sampled via the exponential mechanism) $Q = \anglebrack{q_1, \ldots, q_t}$, noisy answers (measured via the Gaussian mechanism) $A = \anglebrack{a_1, \ldots, a_t}$, max iterations $M$, batch size $B$ \\

\FOR{$m = 1 $ {\bfseries to} $2M$}
    \STATE Let synthetic answers $\hat{A} = \rap{}/\gem{}_\theta(Q)$
    \STATE Let errors $P = |A - \hat{A}|$
    \IF{${m \bmod 2} = 0$}
        \STATE Sample a set of query indices $S$ of size $B$ uniformly
    \ELSE
        \STATE Sample a set of query indices $S$ of size $B$ proportional to errors $P$
    \ENDIF
    \STATE Update $\theta$ via stochastic gradient decent according to $\norm{P_S}_1$
\ENDFOR
\end{algorithmic}
\end{algorithm}

==> icml/docs/conclusion.tex <==
\section{Conclusion}
We present \privGA{}, a versatile genetic algorithm that can generate synthetic data to approximate a wide range of statistical queries, regardless of their differentiability. \privGA{} uses a novel crossover and mutation routine crucial to its success. Our empirical evaluation of the \privGA{} mechanism on mixed-type data demonstrates that \privGA{} outperforms the state-of-the-art method, \rappp{}, on non-differentiable queries and matches first-order optimization methods for differentiable ones. Overall, genetic algorithms present a promising solution for generating mixed-type synthetic data, and we hope our work will inspire further exploration of such approaches in privacy research.

==> icml/docs/dp.tex <==
\section{Additional preliminaries}
\begin{definition}[Exponential Mechanism]\label{def:exponential}
Given some dataset $D\in \cX^*$, arbitrary range $\mathcal{R}$, and score function $S: \mathcal{X}^*\times\mathcal{R}\rightarrow\mathbb{R}$, the exponential mechanism $\mathcal{M}_E(D,S,\mathcal{R},\varepsilon)$ selects and outputs an element $r\in\mathcal{R}$ with probability proportional to $\exp\pp{\frac{\varepsilon S(D,r)}{2\Delta_S}},$ where $\Delta_S$
 is the sensitivity of $S$.
 \end{definition}
 


==> icml/docs/experiment.tex <==


\section{Experiments}\label{sec:experiments}

\begin{figure}
    \centering
    \includegraphics[width=0.45 \textwidth]{images/acs_histplot2.png}
    \caption{A histogram view of the \acsrealdata{} dataset.  }
    \label{fig:histplot}
\end{figure}


We conduct experiments to compare the performance of \privGA{} against baseline mechanisms in various settings. In particular, we evaluate the performance of various synthetic data mechanisms on mixed-typed data, which contain both categorical and numerical attributes. Our results demonstrate that in this setting, \privGA{} is strong mechanism in approximating various types of statistical queries, outperforming \rappp{}, the state-of-the-art method for generating synthetic data with real-valued columns. In addition, we demonstrate that \privGA{} achieves performance comparable to that of mechanisms specifically designed for---and restricted to---handling differentiable query functions for discrete data.

% In this study, we conduct experiments to compare the performance of \privGA{} against different baseline mechanisms in various settings. The primary focus of our evaluation is to assess the ability of the algorithm to approximate categorical features using publicly available data from the US census.

% The results of the categorical data type experiments indicate that \privGA{} exhibits comparable performance to mechanisms specifically designed for handling discrete data. However, the main objective of this section is to evaluate the performance of various synthetic data mechanisms when the input data contains numeric or real-valued features.

% We systematically varied the settings of the experiments, such as the type and size of the dataset, and the level of privacy required, to evaluate the performance of the algorithm. The main performance metric is the max error over the statistical queries. The results of the experiments were analyzed using various visualizations.

% The results of our experiments demonstrate that \privGA{} is a promising mechanism for approximating various types of statistical queries and mixed-type datasets. We finalize the section by showing that using the synthetic data as training data for machine learning models, and show that the models trained on synthetic data achieve test accuracy comparable to models trained on real data.  

\subsection{Data}\label{sec:data}

For our empirical evaluation, we construct datasets derived from the Folktables package \cite{ding2021retiring}, which produces datasets using samples from the American Community Survey (ACS). The ACS is collected annually by the U.S. Census Bureau to capture the demographic and economic characteristics of individuals and households in the country. In particular, Folktables provides an array of classification tasks, which are defined by a target column, a collection of mixed-type features, and some filter that specifies what samples to include.\footnote{For example, a task can be defined to include only rows with individuals over the age of 18.}

While our work is primarily focused on outputting private synthetic data that contain real-valued attributes, the tasks predefined by \citet{ding2021retiring} are dominated by categorical features.\footnote{Each has has at most 4 real-valued features.}
%
Therefore, we focus our attention to the mobility task, which contains the most real-valued features (4 in total) among all tasks. We refer to this data domain as \acsmob. Moreover, to evaluate on a dataset that is comprised primarily of real-valued attributes, we construct a new data domain called \acsreal, which contains 8 real-valued and 3 categorical attributes.

Finally, we use data from California, and normalize the data by linearly scaling real-valued columns to lie in $[0,1]$. We will refer to these two datasets as \acsmobdata{CA} and \acsrealdata{CA}, and provide more details in Table \ref{tab:data_stats}.

% We use a collection of datasets from the U.S. Census introduced in \cite{ding2021retiring}. These datasets include five pre-defined prediction tasks, each with a target column and a set of mix-type features. Each task consists of a subset of columns from the American Community Survey (ACS) corpus. The ACS is collected annually by the U.S. Census Bureau to capture the demographic and economic characteristics of individuals and households in the country.

% The ACS tasks defined originally in \cite{ding2021retiring} mostly contain categorical features (each has between 1 to 4 numeric features). Therefore, we use the original ACS tasks for our first experimental phase, where we test the synthetic data algorithms for categorical data and marginal queries. Next, we introduce a dataset of real-valued, continuous columns derived from the American Community Survey (ACS) for the second experiment phase. Specifically, we use the Folktables \cite{ding2021retiring} package to extract all the ACS real-valued columns (see Table \ref{tab:data_attributes}). We denote our newly constructed data domain as \acsreal and conduct experiments using records from various states. The \acsreal{} task contains three categorical features and nine real-valued features. We use data from California and New York, which contain 144725 and 58041 rows. We normalize the data by linearly scaling the values of each column to lie in $[0,1]$

\begin{table}[ht]
\centering
\caption{For each dataset, we list the number of rows $N$, as well as the number of real and categorical features.}
\label{tab:data_stats}
\begin{tabular}{l | c c c }
    \toprule
    Dataset & N & \# Real & \# Cat. \\
    \midrule
    \acsmobdata{CA} & 156532 & 4 & 17 \\
    \acsrealdata{CA} & 242112 & 8 & 3 \\
    \bottomrule
\end{tabular}
\end{table}

% Mobility - 3-way marginals, 84 workloads, 9415563 queries
% Mobility - 2-way range, 68 workloads, 25296 queries
% Real - 3-way range (2 num), 84 workloads, 1076320 queries

% Mobility: Domain(DEYE: 2, COW: 10, ESR: 6, RELP: 17, ANC: 5, MIG: 2, SEX: 2, MIL: 4, DREM: 2, NATIVITY: 2, DEAR: 2, RAC1P: 9, MAR: 5, GCL: 3, CIT: 5, DIS: 2, SCHL: 24, PINCP: 32, AGEP: 32, WKHP: 32, JWMNP: 32)
% Real: Domain(ESR: 6, PINCP: 2, PUBCOV: 2, AGEP: 32, POVPIP: 32, JWRIP: 32, SEMP: 32, WAGP: 32, WKHP: 32, INTP: 32, JWMNP: 32)


\subsection{Statistical queries} 

Statistical queries are essential for data analysis and decision-making, as they allow us to extract meaningful insights from large and complex datasets. In this section, we describe how we define the four sets of statistical queries that we use in our experiments. We summarize these queries in Table \ref{tab:queries} and describe them in more detail below:

%

\paragraph{Random Prefixes:} To generate a random prefix query we randomly sample a categorical column $c$ and two numeric columns $a, b$. Then we uniformly sample a target value $v$ for column $c$ and the thresholds $\tau_a,\tau_b\in[0,1]$ for the numeric columns $a$ and $b$. The corresponding prefix query $q_{\text{prefix}}$ is defined as follows:
%
\begin{align}
    q_{\text{prefix}}(x) = \mathbb{I}\{x_c = v \text{ and } x_{a}< \tau_a \text{ and } x_b < \tau_b\}
\end{align}
%
To create the query set for the prefix class, we sample $50,000$ random prefix by repeating the process from above. 

\paragraph{Random Halfspaces}

Next we describe the construction of the \emph{halfspace} queries using \cref{def:halfspace}. 
We generate a set $Q_{lin}$ of  $m=50,000$ random queries,  which is populated as follows:

1. Generate a random vector $\hat{\theta}\in \mathbb{R}^{d_{|R|}}$, where the value of each coordinate $i\in R$ is sampled as  $\hat{\theta}_i \sim \cN(0, 1)$. 
     Then  set $\theta = \hat{\theta}/\sqrt{d}$.\\
2. Sample a threshold value $\tau$ from the standard normal distribution, i.e., $\tau\sim \cN(0,1)$. \\
3. Sample a label $i\in L$ 
     and a target value for the label $y\in \cX_i$.\\
4. Add the query  $q_{i, y, R, \theta, \tau}$ to the set $Q_{lin} $.


\paragraph{$k$-way Categorical Marginals:}
We select all $3$-way marginal queries using categorical columns only. Since the query answers in a workload sum up to $1$, each workload has $\ell_2$-sensitivity $\Delta_2 = 1$.

\paragraph{$k$-way Range Marginals:}
We construct range queries using one categorical attribute and one real-valued attribute. Recall that real-valued features lie in the domain $[0,1]$. Thus, we define a workload of range queries by the set of intervals of width $\frac{1}{2^j}$ for $j \in \{1, 2, \ldots, 5\}$.

Now consider the set
\begin{align*}
    I = \{ \pp{\tfrac{i}{2^j}, \tfrac{i + 1}{2^j}}| 0\leq i< 2^j , j \in \{1, 2, \ldots, 5\} \}
\end{align*}
%
Using the same notation from definition \ref{def:range_marginals}, for real-valued feature $c$, the corresponding range workload  $Q_{c, I} =\{ q_{c, (a,b)}\}_{(a, b) \in I}$ is the set of range queries defined by intervals in $I$. This construction simulates the binary mechanism of \citep{chan2011private} for releasing sum prefixes privately.

Note that a single data point only appears in one interval of size $1/2^j$ for each $0< j \leq 5$. Therefore, adding a new data point only affects the counts of $5$ range queries in the workload $Q_{c, I}$.
By the same logic, replacing a data point affects $10$ range queries in  $Q_{c, I}$. Therefore, we say that the workload  $Q_{c,I}$ has $\ell_2$-sensitivity $\sqrt{10}$.
% \begin{align}
%     % 
% \end{align}

% is a vector where each coordinate is the answer of range query $ q_{c, (a, b)}(x)$ for an interval in $(a,b)\in I$
% \begin{align*}
%    Q_{c, I}(x) = \pp{ q_{(a, b)}(x),  } _{(a, b)\in I}
% \end{align*}

\begin{table}[!htb]
\centering
\caption{The total number of queries depends on the input data total number of features, which we denote by $d$ and  the number of categorical and numerical features, $d_{cat}$ and $d_{num}$ respectively. In addition, we list the $\ell_2$-sensitivity $\Delta_2$ of each query class (the sensitivity for categorical and range marginals is written with respect to an entire workload of queries). Note that in our experiments, the number of categorical attributes comprising both $2$- and $3$-way range marginals is always set to $1$.}
\begin{tabular}{l |c c}
    \toprule
    Query class & Query set size & $\Delta_2$ \\
    \midrule
    3-way Categorical & ${\binom{d}{3}}$ & $\sqrt{2}$ \\  
    \midrule 
    2-way Range & $d_{cat} \cdot d_{num}$ & $\sqrt{10}$ \\  
    \midrule
    3-way Range & $d_{cat} \cdot {\binom{d_{num}}{2}}$ & $\sqrt{10}$ \\  
    \midrule
    Random Prefix & $(d_{cat}+1) \cdot 50,000$  & $1$ \\  
    \midrule
    Random Halfspaces & $d_{cat} \cdot 50,000$  & $1$ \\  
    \bottomrule
\end{tabular}
\label{tab:queries}
\end{table}

% \subsection{Evaluation metrics} 
% %
% We evaluate the performance of synthetic data algorithms by measuring the approximation error of each statistic. We use two metrics to evaluate the performance: the average and maximum approximation errors. Furthermore, we report the approximation error over various privacy levels, determined by the privacy parameter $\varepsilon$, to examine the trade-off between privacy and accuracy for each method.
% by varying the privacy parameter, allowing us to determine the optimal privacy level for a given application.

\subsection{Baselines}

\paragraph{\rappp.}

We compare our mechanism \privGA{} against the mechanism \rappp{} by \citet{vietri2022private}. The \rappp{} algorithm uses a first-order optimization algorithm called {\em Sigmoid Temperature Annealing} (pseudocode can be found in Appendix \ref{appx:rappp}). Recall that \rappp{} replaces the prefix queries with a differentiable surrogate query by using Sigmoid functions. Moreover, to control the degree by which the Sigmoid functions approximate the prefix functions, it uses the {\em inverse Sigmoid temperature parameter} $\invtemp$. The algorithm starts with a small inverse temperature $\invtemp$ and runs a gradient-based minimizer (SGD or Adam) on the induced optimization objective with learning rate \LR, and then repeats the process for a different choice of inverse temperature. 

% The inverse temperature parameters used in our experiments are $\invtemp\in \{2, 4, 8, 16, 32, 64, 128, 256, 512, 1024, 2048\}$. 

% \rappp{} is also sensitive to its learning rate (\LR) parameter, which controls the speed of the gradient-descent algorithm. Thus, we run \rappp{} multiple times, each time with a different learning rate $\LR \in \{0.0005, 0.001, 0.002, 0.005, 0.01\}$. 

% We run \rappp{} for 5000 iterations and \privGA{} for 3000 iterations, and both get synthetic data of size 100. For \rappp{} baseline, each time we try all lr values in $[0.0005, 0.001, 0.002, 0.005, 0.01]$ and choose the synthetic data that get lowest in-sample error to be the final result. For \privGA{}, we set the population size $N$ to be 8000.
% \gv{Add more} \jt{not sure what to add}\gv{This is good for now.}

\paragraph{\rap/\gem.}

We also compare our method to \rap{} \citep{aydore2021differentially} and \gem{} \citep{liu2021iterative}, two gradient-based optimization algorithms for generating private synthetic data that belong to discrete data domains. In both algorithms, datasets are modeled as mixtures of product distributions $P$ over the attributes, with the main difference being the way in which such distributions are parameterized---in \gem{}, $P$ is parameterized by a neural network that given Gaussian noise, outputs a set of product distributions, while in \rap{}, $P$ is parameterized directly by the probabilities defining the distribution for each attribute. Because both methods are limited to discrete data, real-valued columns must be discretized first. Consequently, \rap{} and \gem{} can only optimize over $k$-way categorical and range marginals. In Appendix \ref{appx:rapgem}, we show how we modify these methods to optimize over range queries and also provide additional details about their optimization procedures. 

\paragraph{\pgmem.}

Lastly, we compare to a graphical model approach, \pgm{} \citep{mckenna2019graphical}, which like \rap{} and \gem{}, is also limited to discrete data domains. However, \pgm{} instead models data distributions using probabilistic graphical models. We run an adaptive version of \pgm{} that also uses the exponential mechanism. We refer to this variant as \pgmem{} and run it on $k$-way categorical marginals.
% , and compare it against \privGA{}, \rap{}, and \gem{} on $k$-way marginal queries.


% \subsection{Additional details on \privGA{}.} 
% %
% For the experiments in this section, we run the \privGA{} algorithm with a population size of $N=10000$. In addition, the elite set parameter is set to $T=2$. These values give consistent results for our experiments. However, at the cost of longer runtime, increasing $G$ and $N$ should improve the accuracy of the \privGA{} since it provides the algorithm with more rounds to find an accurate synthetic dataset.

% The remaining parameter is the mutation strength $\sigma$, which controls the magnitude of off-spring mutations from one generation to the next. For instance, setting mutation strength $\sigma=0$ equates to no modifications and would not produce any diversity for future generations. On the other hand, a higher value of $\sigma$ corresponds to more aggressive mutations, which could make the system unstable and not converge. In our work, we found that $\sigma=0.1$ provides a good trade-off between diversity and stability of each generation. However, in the following section, we compare the performance of \privGA{} over different choices of mutation strength $\sigma$ and demonstrate that any value between $0.1$ and $0.5$ also provides good performance. 




% \paragraph{Hyperparameter Sensitivity Evaluation.} 
% %
% How difficult it is to choose the correct parameter combination for a particular mechanism is paramount to its practicality. We say that a mechanism is sensitive to the choice of hyperparameters if it only works well under a narrow set of values. Therefore, in this section, we evaluate how sensitive \privGA{} and \rappp{} are to the choice of the mutation strength $\sigma$ and and learning rate \LR{} parameters respectively. We evaluate both algorithms over different choices of hyperparameters to approximate the set of prefix queries on the \acsreal{} dataset for New York. Moreover, we evaluate over two privacy levels $\varepsilon \in \{0.1, 1\}$. In Table \ref{tab:hyperparameters}, we observe that \rappp{} is very sensitive to the choice of \LR, only working for $\LR=0.02$. \privGA{}, however, is less sensitive to the choice of mutation strength $\sigma$. Setting $\sigma=0.1$ is the best value we found, but any value of $\sigma \in [0.05, 0.5]$ also serves as a good choice.


% \subsection{Experiment setup} We compare the performance of our proposed algorithm, \privGA{}, against the baseline mechanism in different settings over different differential privacy levels. A critical parameter that significantly influences the performance is the number of adaptive epochs $T$, as described in the adaptive framework algorithm \ref{alg:adaptive}.

% To evaluate the performance of the algorithms, we try different values of $T$ for each algorithm in our experiments and report the best error for each $\varepsilon$ value. To allow for a fair and accurate comparison of the algorithms, we provide a detailed description of how the results were computed, including specific settings or parameters, such as the different values of $T$ we tried.

% \begin{table}[h]
%     \centering
%     \begin{tabular}{c|c}
%          \privGA{} &  \\
%          \acsmobility & 25, 50, 75, 100 
%          Prefix
%     \end{tabular}
%     \caption{Number of adaptive epoch for each setting}
%     \label{tab:my_label}
% \end{table}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.99\linewidth]{images/acsreal_max_avg_error.png}
    \caption{Max and average error evaluated on \acsrealdata{CA} with non-differentiable queries---150K random halfspaces and 200K random prefixes. 
    \rap{} and \gem{} are trained with $3$-way range queries.
    We fix $\delta={1/N^2}$ and vary $\varepsilon\in\{0.07, 0.23, 0.52, 0.74, 1.0\}$. Results are averaged over 3 runs.}
    \label{fig:errors_acsreal}
\end{figure}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.99\linewidth]{images/mobility_max_avg_error.png}
    \caption{Max and average error evaluated on \acsmobdata{CA} with differentiable queries---3-way categorical and 2-way range marginal queries.
    We fix $\delta={1/N^2}$ and vary $\varepsilon\in\{0.07, 0.23, 0.52, 0.74, 1.0\}$. Results are averaged over 3 runs.
    }
    \label{fig:errors_acsmobility}
\end{figure}

\subsection{Results}
%
% Figure \ref{fig:income_prefix_errors} shows how our method offers significant improvement over both {\em average} and {\em max} error, especially over {\em max} error.
%
% Figure \ref{fig:income_prefix_errors} shows that while \rappp{} fails to optimize over {\em max} error, \privGA{} shows good performance on both {\em average} and {\em max} error. Moreover, \privGA{} offers a significant improvement for average error over all privacy parameter $\varepsilon$ and over the two datasets we tried.  

This section provides empirical evidence that \privGA{} is a better algorithm for generating real-valued synthetic data (i.e., when the statistical queries are non-differentiable). We fix $\delta=\frac{1}{N^2}$ and $\varepsilon\in\{0.07, 0.23, 0.52, 0.74, 1.0\}$ to examine the trade-off between privacy and accuracy. We run all algorithms using various choices of $T$ and report the best error (averaged over 3 runs) for each $\varepsilon$ value. In addition, we show that on discretized data (both categorical and mixed-type), the \privGA{} mechanism performs equally as well as prior work \rap{}, \gem{} and \pgmem. 

In Figure \ref{fig:errors_acsreal}, we show that when given the same set of queries $Q$, \privGA{} significantly outperforms \rappp{} with respect to max and average error. In particular, these experiments show that while \rappp{} can optimize over such queries, using a surrogate differentiable approximation in combination with temperature annealing leads to various problems. On prefix queries (Figure \ref{fig:errors_acsreal}, right panel), we see that while average error decreases as the privacy budget increases, the optimization of \rappp{} is unstable, causing the max error to unexpectedly increase. 

In addition, we run \rap{} and \gem{} on $3$-way range queries after discretizing \acsreal and evaluate their outputs on both halfspace and prefix queries in Figure \ref{fig:errors_acsreal}.\footnote{To convert discretized features back to real-valued attributes, we uniformly sample values within the bin.}
%
Given that that \rap{} and \gem{} are not optimized over halfspace and prefix queries, it is unsurprising that \privGA{} significantly outperforms both methods. However, we observe that with respect to average error, \rap{} and \gem{} still outperform \rappp{}, further highlighting its issues.

Finally, we present the performance of \privGA{} against \rap{}, \gem{} and \pgmem{} in Figure \ref{fig:errors_acsmobility}, where we plot errors on answering a large set of categorical marginal (left) and range marginal (right) queries on the \acsmob dataset. We note that answering categorical marginals has been the main focus of \rap{}, \gem{} and \pgm{}. Moreover, we discretize the data in such a way that the resulting bins align with the intervals comprising our range marginal queries, allowing us to also write differentiable forms of such queries for \rap{} and \gem{}.\footnote{See Appendix \ref{appx:rapgem} for more details.}
%
Nevertheless, we observe that \privGA{} is able to synthesize both categorical-only (for categorical marginals) and mixed-type (for range marginals) data that matches the performance of the three baseline algorithms. Moreover, unlike \rap{} and \gem{}, \privGA{} does not require that the numerical features be discretized first when optimizing over range marginal queries.



% \begin{figure}
% % % \textbf{title}
%     \centering
%     \includegraphics[width=0.5\textwidth]{icml/images/acsreal_.png}
%     \caption{Average error evaluating on 150K random halfspaces and and 200K random prefix  with $(\eps, \delta)$-differential privacy. . 
%      Input dataset is \acsreal for the state of California. We fix $\delta={1/n^2}$ for all experiment and use privacy budgets $\varepsilon\in\{0.07, 0.23, 0.52, 0.74, 1.0\}$. Results are averaged over 3 runs.}
%     \label{fig:acsreal}
% \end{figure}

% \begin{figure}
% % \textbf{title}
%     \centering
%     \includegraphics[width=0.5\textwidth]{icml/images/mobility_avg_error.png}
%     \caption{Average Error  evaluating on 3-way categorical and 2-way range marginal queries  with $(\eps, \delta)$-differential privacy. . 
%      Input dataset is \acsmob for the state of California. We fix $\delta={1/n^2}$ for all experiment and use privacy budgets $\varepsilon\in\{0.07, 0.23, 0.52, 0.74, 1.0\}$. Results are averaged over 3 runs.
%      }
%     \label{fig:mobility_avg_errors}
% \end{figure}










% \begin{table}[ht]
% \centering
% \caption{ML Accuracy after training with on $1$-DP synthetic data. Target variables include employment (ESR), income (ESR), and public coverage (PUBCOV)}
% \label{tab:ml_results}
% \begin{tabular}{l | l l l l}
%     \toprule
%     ML Task & Mechanism & LR  & RF & XGB\\
%     \midrule
%     \multirow{6}{*}{PUBCOV}
%     & \multirow{1}{*}{\gem}             &  0.2156 & 0.2011 & 0.2068 \\
%     & \multirow{1}{*}{\rap}             &  0.2142 & 0.1895 & 0.1908 \\
%     & \multirow{1}{*}{\rappp}           &  \textbf{0.2077} & 0.1816 & 0.1874 \\
%     & \multirow{1}{*}{\privGA(Pre)}  &  0.2119 & 0.1804 & \textbf{0.1823} \\
%      & \multirow{1}{*}{\privGA(HS)}     &  0.2121 & \textbf{0.1791} & 0.1874 \\ 
%      \cmidrule{2-5}
%     & \multirow{1}{*}{Original}         &  0.2095 & 0.1720 & 0.1581 \\
%     \midrule
    
%     \multirow{6}{*}{PINCP}
%     & \multirow{1}{*}{\gem}             & 0.0971        & 0.0815 & 0.0805\\
%     & \multirow{1}{*}{\rap}             & \textbf{0.0886} & 0.0745 & 0.0750\\
%     & \multirow{1}{*}{\rappp}           & 0.0923        & 0.0842 & 0.0876\\
%     & \multirow{1}{*}{\privGA(Pre)}  & 0.1184        & \textbf{0.0471} & \textbf{0.0558}\\
%      & \multirow{1}{*}{\privGA(HS)}     & 0.1174        & 0.0720 & 0.0882\\ 
%      \cmidrule{2-5}
%     & \multirow{1}{*}{Original}         & 0.0569        & 0.0369 & 0.0334\\
%     \midrule

%     \multirow{6}{*}{ESR}
%     & \multirow{1}{*}{\gem}             & 0.0865 &  0.0842   & 0.0892 \\
%     & \multirow{1}{*}{\rap}             & \textbf{0.0857} &  0.0818   & \textbf{0.0803} \\
%     & \multirow{1}{*}{\rappp}           & 0.0903 &  0.0825   & 0.0873 \\
%     & \multirow{1}{*}{\privGA(Pre)}     & 0.0903 &  0.0826   & 0.0852 \\
%     & \multirow{1}{*}{\privGA(HS)}      & 0.0907 &  \textbf{0.0784}   & 0.0829 \\
%      \cmidrule{2-5}
%     & \multirow{1}{*}{Original}         & 0.0768 &  0.0713   & 0.0648  \\

    
%     \bottomrule
% \end{tabular}
% \end{table}




% \begin{table}[ht]
% \centering
% \caption{ML Accuracy after training with on $(0.07)$-DP synthetic data. Target variables include employment (ESR), income (ESR), and public coverage (PUBCOV)}
% \label{tab:ml_results}
% \begin{tabular}{l | l l l l}
%     \toprule
%     ML Task & Mechanism & LR  & RF & XGB\\
%     \midrule
%     \multirow{6}{*}{PUBCOV}
%     & \multirow{1}{*}{\gem}             &  0.2168           & 0.2145            & 0.1989 \\
%     & \multirow{1}{*}{\rap}             &  0.2153           & 0.1967            & \textbf{0.1980} \\
%     & \multirow{1}{*}{\rappp}           &  \textbf{0.2105}  & 0.2143            & 0.2211 \\
%     & \multirow{1}{*}{\privGA(Pre)}     &  0.2138           & \textbf{0.1948}   & 0.2061 \\
%      & \multirow{1}{*}{\privGA(HS)}     &  0.2127           & 0.2013            & 0.2127 \\ 
%      \cmidrule{2-5}
%     & \multirow{1}{*}{Original}         &  0.2095 & 0.1720 & 0.1581 \\
%     \midrule
    
%     \multirow{6}{*}{PINCP}
%     & \multirow{1}{*}{\gem}             & 0.1078            & 0.0883            & 0.0953 \\
%     & \multirow{1}{*}{\rap}             & \textbf{0.1002}   & 0.0836            & 0.0829 \\
%     & \multirow{1}{*}{\rappp}           & 0.1112            & 0.1162            & 0.1237 \\
%     & \multirow{1}{*}{\privGA(Pre)}     & 0.1167            & \textbf{0.0694}   & \textbf{0.0770} \\
%      & \multirow{1}{*}{\privGA(HS)}     & 0.1236            & 0.1146            & 0.1207 \\ 
%      \cmidrule{2-5}
%     & \multirow{1}{*}{Original}         &  & 0.0369 & 0.0334\\
%     \midrule

%     \multirow{6}{*}{ESR}
%     & \multirow{1}{*}{\gem}             & 0.0878            & 0.0940            & 0.0884 \\
%     & \multirow{1}{*}{\rap}             & \textbf{0.0874}   & 0.0850            & 0.0839 \\
%     & \multirow{1}{*}{\rappp}           & 0.0923            & 0.0859            & 0.1083 \\
%     & \multirow{1}{*}{\privGA(Pre)}     & 0.0931            & 0.0832            & 0.0877 \\
%      & \multirow{1}{*}{\privGA(HS)}     & 0.0949            & \textbf{0.0791}   & \textbf{0.0831} \\ 
%      \cmidrule{2-5}
%     & \multirow{1}{*}{Original}         & 0.0768 &  0.0713   & 0.0648  \\

    
%     \bottomrule
% \end{tabular}
% \end{table}



==> icml/docs/experiment_details.tex <==
\section{Additional experiment details}

In this section we include additional details about our experiments, including information about datasets, queries, and hyperparameters.

%%%%% data attributes %%%%%
\paragraph{Data.} In Table \ref{tab:acs_data_attributes}, we list all attributes for each ACS task that are used in empirical results presented in either the main paper or this appendix.

\begin{table}[!htb]
\centering
\caption{We list the ACS data attributes used in our experiments.}
\label{tab:acs_data_attributes}
\begin{tabular}{l | l| l}
\toprule
Dataset & Categorical Attributes & Numeric Attributes \\
\midrule
\multirow{2}{*}{\acsmob} & MIL, DREM, CIT, DIS, COW, MAR, SCHL, MIG, NATIVITY & JWMNP, PINCP \\
& ANC, DEAR, DEYE, SEX, ESR, GCL, RAC1P, RELP & WKHP, AGEP \\
\midrule
\multirow{2}{*}{\acsreal} & \multirow{2}{*}{ESR, PINCP, PUBCOV} & AGEP, POVPIP, JWRIP, SEMP \\
& & WAGP, WKHP, INTP, JWMNP \\
\midrule
\multirow{1}{*}{\acsemp} & COW, OCCP, SCHL, MAR, SEX, PINCP, RAC1P, RELP, POBP & AGEP \\
\midrule
\multirow{2}{*}{\acscov} & MIL, FER, DREM, CIT, DIS, MAR, SCHL, PUBCOV & \multirow{2}{*}{PINCP, AGEP} \\
& MIG, NATIVITY, ANC, DEYE, SEX, ESR, RAC1P, DEAR, ESP & \\
\midrule
\multirow{1}{*}{\acsinc} & COW, OCCP, SCHL, MAR, SEX, PINCP, RAC1P, RELP, POBP & WKHP, AGEP \\
\midrule
\multirow{2}{*}{\acstra} & JWMNP, PUMA, CIT, DIS, OCCP, SCHL, JWTR, MAR & \multirow{2}{*}{AGEP, POVPIP} \\
& MIG, SEX, RAC1P, POWPUMA, RELP, ESP & \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!htb]
\centering
\caption{Number of workloads for categorical and range marginal queries.}
\label{tab:workloads}
\begin{tabular}{l | c c c c c c }
    \toprule
    & mobility & real \\
    \midrule
    $3$-way Cat. Marginals & 680 & - \\
    $2$-way Range Marginals & 68 & - \\
    $3$-way Range Marginals & - & 84 \\
    \bottomrule
\end{tabular}
\end{table}

% \begin{table}[!htb]
% \centering
% \caption{Number of workloads for each task}
% \label{tab:workloads}
% \begin{tabular}{l | c c c c c c }
%     \toprule
%     & employment & coverage & income & mobility & travel & real \\
%     \midrule
%     $3$-way Cat. Marginals & 560 & 680 & 84 & 680 & 364 & - \\
%     $2$-way Range Marginals  & 120 & 136 & 36 & 136 & 91 & - \\
%     $3$-way Range Marginals  & - & - & - & - & - & 84 \\
%     \bottomrule
% \end{tabular}
% \end{table}

\iffalse

%%%%% Runtime %%%%%
\paragraph{Runtime.} In Table \ref{tab:runtime}, we compare the runtime of \privGA{} and our 3 baselines on categorical experiments with $3$-way categorical marginal queries.

In terms of runtime of \privGA, The mutation and crossover steps are computationally straightforward. Therefore, the primary computational bottleneck is the evaluation of the objective score of each population in the dataset. In order to calculate the score of each dataset, we must evaluate the statistics on all synthetic datasets in a population of size $N$. Thus, the algorithm's runtime depends primarily on the speed of evaluating statistical queries. With our choice of hyperparameters, our algorithm attains reasonable runtime compared to the baselines, although our proposed update procedure for \rap{} and \gem{} still runs comparatively fast. 

Experiments for \privGA{} were run on a single GPU of NVIDIA TITAN V. All experiments for \rap{}, \gem{}, and \pgmem{} were run using a desktop computer with NVIDIA GeForce GTX 1080 Ti graphics card. Our implementation for \rap{} and \gem{} is derived from \url{https://github.com/terranceliu/dp-query-release}, while our implementation for \pgmem{} uses \url{https://github.com/ryan112358/private-pgm}.



\begin{table}[!htb]
\caption{We compare the runtime of all algorithms across various choices of $T$ when run on \acsmob, where $Q$ is all $3$-way categorical marginals and $\varepsilon = 1$. The runtime is measured in seconds.}
\label{tab:runtime}
\centering
\begin{tabular}{l | c c c c }
    \toprule
    & $T=25$ & $T=50$ & $T=75$ & $T=100$  \\
    \midrule
    \privGA & 860 & 1744 & 3231 & 5316  \\
    \rap  & 70 & 137 & 204 & 274 \\
    \gem  & 71 & 142 & 211 & 280 \\
    \pgmem & 397 & 2633 & 5693 & 8452 \\
    \bottomrule
\end{tabular}
\end{table}

\fi



%%%%% hyperparameters %%%%%
\paragraph{Hyperparameters.} In Table \ref{tab:hyperparameters}, we list the hyperparameters used for our algorithms.

\begin{table}[!htb]
\centering
\caption{Hyperparameters experiments (with adaptivity).}
\label{tab:hyperparameters}
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l l c c}
    \toprule
    Query Class & Method & Hyperparameter & Values \\
    \midrule
    \multirow{20}{*}{All Experiments} & 
    \multirow{5}{*}{\privGA{}}
    & \multirow{1}{*}{Data Size} & $2000$ \\
    & & \multirow{1}{*}{Population Size} & $1000$ \\
    & & \multirow{1}{*}{Elite Size} & $2$ \\
    & & \multirow{1}{*}{Mutation Rate} & $1$ \\
    & & \multirow{1}{*}{Crossover Rate} & $1$ \\
    & & \multirow{1}{*}{Max Generations} & $10000$ \\
    \cmidrule(lr){2-4}
    & \multirow{5}{*}{\rappp}
    & \multirow{1}{*}{Data Size ($N'$)} & $1000$ \\
    & & \multirow{1}{*}{Queries Sampled ($K$)} & $1000$ \\
    & & \multirow{1}{*}{Learning Rate} & $0.0005$, $0.001$, $0.002$, $0.005$, $0.01$ \\
    & & \multirow{2}{*}{Inverse Temp. ($\invtemp$)}
    & $2$, $4$, $8$, $16$, $32$, $64$, $128$ \\
    & & & $256$, $512$, $1024$, $2048$ \\
    \cmidrule(lr){2-4}
    & \multirow{4}{*}{\rap{} / \gem{}}
    & \multirow{1}{*}{\# Product Mixtures ($K$)} & $1000$ \\
    & & \multirow{1}{*}{Batch Size ($B$)} & $5000$ \\
    & & \multirow{1}{*}{Max Iterations ($M$)} & $1000$ \\
    & & \multirow{1}{*}{\# Samples} & $50000$ \\
    \cmidrule(lr){2-4}
    & \multirow{1}{*}{\rap} & \multirow{1}{*}{LR} & $0.03$ \\
    \cmidrule(lr){2-4}
    & \multirow{3}{*}{\gem{}}
    & \multirow{1}{*}{LR} & $0.0003$ \\
    & & \multirow{1}{*}{Hidden Layers} & $(128, 256)$ \\
    & & \multirow{1}{*}{Noise Dimension} & $16$ \\
    \cmidrule(lr){2-4}
    & \multirow{2}{*}{\pgmem}
    & \multirow{1}{*}{Max Iterations} & $250$ \\
    & & \multirow{1}{*}{\# Samples} & $N$ \\
    \midrule
    \multirow{2}{*}{Halfspace / Prefix} & 
    \multirow{1}{*}{\privGA{}} & \multirow{1}{*}{$T$} & $25$, $50$, $75$, $100$ \\
    \cmidrule(lr){2-4}
    & \multirow{1}{*}{\rappp} & \multirow{1}{*}{$T$} & $3$, $4$, $5$, $6$, $7$, $8$, $9$ \\
    \midrule
    \multirow{1}{*}{2-way Range} & 
    \multirow{1}{*}{\privGA{} / \rap{} / \gem{}} & \multirow{1}{*}{$T$} & $10$, $20$, $30$, $40$, $50$, $60$ \\
    \midrule
    \multirow{1}{*}{3-way Range} & 
    \multirow{1}{*}{\rap{} / \gem{}} & \multirow{1}{*}{$T$} & $10$, $20$, $40$, $60$, $80$ \\
    \midrule
    \multirow{1}{*}{3-way Categorical} & 
    \multirow{1}{*}{All algorithms} & \multirow{1}{*}{$T$} & $25$, $50$, $75$, $100$ \\
    \bottomrule
\end{tabular}
\end{table}


% \section{Additional results}

% In Tables \ref{tab:oneshot} we provide additional results on categorical marginals and with different ACS tasks as defined in Table \ref{tab:acs_data_attributes}. This brief experiment also shows that like in the adaptive setting, \privGA{} achieves similar performance to \rap{} on differentiable queries in the one-shot setting across many datasets. We use the same hyperparameters used in our adaptive experiments (Table \ref{tab:hyperparameters}), excluding ours choices for $T$, which are not applicable in the one shot setting.

% \begin{table}[!htb]
% \centering
% \caption{Max and average error of one-shot mechanism ($\varepsilon=1$) with $2$-way categorical marginal queries for all ACS tasks. We also list the number of workloads for each task.}
% \label{tab:oneshot}
%     \begin{tabular}{l c | c c | c c }
%     \toprule
%     & & \multicolumn{2}{c}{Max} & \multicolumn{2}{c}{Average}\\
%     & \# workloads & \rap{} & \privGA{} & \rap{} & \privGA{} \\
%     \midrule
%     \acsmob & 136 & 0.003005 & 0.004519 & 0.0004527 & 0.0005146 \\ 
%     \acsinc & 36 & 0.003048 & 0.001416 & 0.0000206 & 0.0000253 \\ 
%     \acsemp & 120 & 0.001288 & 0.001497 & 0.0001768 & 0.0001862 \\
%     \acstra & 91 & 0.004898 & 0.004251 & 0.0000318 & 0.00003724 \\ 
%     \acscov & 136 & 0.002156 & 0.002437 & 0.0003193 & 0.00034858 \\
%     \bottomrule
% \end{tabular}
% \end{table}

==> icml/docs/experiments_table.tex <==
\newcommand{\Cross}{$\mathbin{\tikz [x=1.4ex,y=1.4ex,line width=.2ex, red] \draw (0,0) -- (1,1) (0,1) -- (1,0);}$}%

\newcommand{\Checkmark}{$\color{green}\checkmark$}


\begin{table}[]
    \centering
    \begin{tabular}{p{0.40\linewidth}|c|c|c}
    & \pgm & \rap/\ \gem  & \rappp\\
    \hline
        Categorical data \&  3-way marginals &  \Checkmark & \Checkmark & \Cross \\
        \hline 
    Mixed data \& range queries &  \Checkmark & \Checkmark & \Cross  \\
         \hline 
    Mixed data \& halfspace queries &  \Cross & \Cross & \Checkmark  \\
    \end{tabular}
    \caption{Baselines}
    \label{tab:experiments}
\end{table}

==> icml/docs/intro.tex <==
\section{Introduction}

% \color{red}

% \subsection{Text TODO}

% \begin{itemize}

%     \item Reduce text about history of synthetic data:
%     \item   how the algorithm handles columns of different variance. Show how crossover handles this naturally.
%     \item  Add oracle theorem 
%     \item Describe in text time-based early stop.
% \end{itemize}

% \subsection{experiments TODO}
% TODO:
% \begin{enumerate}
%     \item Compare PrivGA vs GEM/RAP on mixed data. 
%     \item Implement RAP++ for range queries and prefix queries.
%     \item Estimate conditional halfspaces. Compare against RAP++.
%     \item Parameter analysis of PrivGA and RAP. Add a plot of error vs runtime.
%     \item Multi-task machine learning .
% \end{enumerate}

% \paragraph{Other ideas:} A list of other features we could include:
% \begin{enumerate}
%     \item Logistic regression queries: Answer a bunch of logistic regression queries with objective perturbation and project using PrivGA. 
%     \item Add fairness constraints. A model trained on synthetic data should be fair.
% \end{enumerate}


% \subsection{Main document plot list}
% \begin{enumerate}
%     \item Categorical-marginals plot for only one task (mobility). This plot includes PrivGA, RAP, GEM and PGM.
%     \item Range-marginals for 5 tasks. This plot includes PrivGA, RAP, GEM, PGM and RAP++.
%     \item 
% \end{enumerate}

% \color{black}
 
% In this work, we consider the problem of generating synthetic data under differential privacy \cite{dwork2006calibrating} with a focus on answering a large collection of statistical queries. 
% Some approaches to producing synthetic data follow the generative adversarial network (GAN) framework due to  \cite{goodfellow2014generative}. Private implementations of the GAN framework are based on private-stochastic gradient descent (DP-SDG)  (see \cite{}). However, these methods do not perform well in practice \gv{why?}. In this work, we consider a different paradigm that consists of allocating the privacy noise to answer a selected collection of statistical queries and then finding a synthetic dataset consistent with the query answers. 
%
% The problem of releasing statistics subject to privacy has been extensively studied \cite{MWEM}.

% Introduce the problem
Access to high-quality data is critical for decision-making and data analysis. However, the reliance on sensitive data can reveal private information about the individuals in the data, such as medical conditions or financial status. Therefore, privacy concerns impose legal and ethical constraints on what one can access for data analysis. \emph{Differential privacy} \citep{dwork2006calibrating} has become an increasingly popular framework  for protecting sensitive information by providing a formal privacy guarantee that allows one to calibrate the trade-off between privacy and accuracy. Moreover, differentially private synthetic data has become especially attractive, given that such data can be accessed repeatedly without added privacy costs. Consequently, we focus on the problem of generating synthetic data that approximates various properties of the underlying sensitive dataset while providing privacy guarantees. 

A standard approach to this problem is to find a synthetic dataset that matches a large family of statistics derived from the underlying dataset. In this work, we focus on statistics in the form of  \textit{statistical queries}, which count the fraction of examples that satisfy some specific properties. This approach is often framed as synthetic data for \textit{private query release}, where the goal is to release answers to an extensive collection of statistical queries by outputting a synthetic dataset from which answers are derived from. There exists a long line of research studying synthetic data for private query release \citep{BLR08, MWEM, dualquery, HDMM, FEM, mckenna2019graphical, aydore2021differentially, liu2021leveraging, liu2021iterative}. Moreover, when the set of statistical properties is sufficiently rich, this approach has been shown to outperform differentially private deep generative models (e.g., GANs) in both capturing various statistical properties and enabling downstream machine learning tasks \citep{tao2021benchmarking, vietri2022private}. 

% Recently, \citet{vietri2022private} has framed this type of method as a class of \textit{moment-matching} approaches.\footnote{In their framing, the process of optimizing synthetic data generators over statistical query answers is used for producing high-quality, multipurpose synthetic samples, rather than for simply releasing the raw statistical query answers themselves.} 
%
Even though the problem of generating synthetic data for private query release is shown to be computationally intractable in the worst case \cite{hardsynthetic, ullman2013answering},  there has been a line of work on practical algorithms that can perform well on real datasets \cite{dualquery, FEM, mckenna2019graphical, liu2021leveraging}. Before our work, the algorithms that achieve state-of-the-art performance all leverage gradient-based optimization \citep{aydore2021differentially, liu2021iterative, vietri2022private} to minimize the error for certain classes of statistical queries. However, these methods require differentiability, severely limiting the types of statistical properties one can optimize. For example, existing algorithms such as \rap{} \citep{aydore2021differentially} and \gem{} \citep{liu2021iterative} focus specifically on using first-order mechanisms for approximating marginal queries that apply to discrete data only, requiring real-valued attributes be discretized first. 

% In general, this discretization approach can be computationally expensive, particularly when a high resolution of the real-value features is required and the data contains many real-valued features. 
% For example, if $b$ bins are used to discretize $r$ real-valued columns, the resulting discretized dataset will have a dimension of $b \cdot r$. 
% Additionally, discretization is limited in terms of the types of queries one can optimize for. In this work, we focus on answering random halfspace and prefix queries, which would be impossible to discretize to such a fine granularity for.

Many natural classes of queries for data containing real-valued attributes are non-differentiable, such as prefixes (equivalently the CDF of an attribute), and their higher-dimensional extension, halfspaces. Moreover, these queries cannot be optimized directly by methods that operate over discrete data, even with the discretization of real-valued features. \citet{vietri2022private} circumvent discretization by approximating non-differentiable queries with differentiable surrogate functions. Thus, their approach, \rappp{}, can directly optimize over a large class of statistical queries. However, their method induces additional error due to the relaxation of the original minimization problem, which may not produce an optimal solution for the original one. \footnote{
In Appendix \ref{appx:rappp}, we show a simple example in which the continuous relaxation leads \rappp{} to a bad local minimum very far from the optimal solution---\emph{even} when absent of privacy constraints.}

% \footnote{A {\em marginal} query is a function that counts the fraction of rows in a dataset where a particular set of attributes matches specific values. For example, a marginal query is: "How many people in dataset $D$ are Asian and live in NYC."}

In light of these challenges, we propose a new synthetic data generation algorithm, \privGA{}, that is capable of outputting \textit{mixed}-type data (i.e., containing both discrete and real-valued attributes) without requiring differentiability in its optimization objective or discretization of real-valued attributes. \privGA{} is zeroth-order mechanism based on a genetic algorithm that avoids the limitations of first-order methods such as \rappp{}, which uses surrogate loss functions to ensure differentiability. Instead, \privGA{} can optimize the error objective directly. Inspired by the genetic algorithm $\simpleGA$ \citep{such2017deep}, our algorithm \privGA{} evolves a population of datasets over $G$ generations---starting from a population of $N'$ randomly chosen datasets, where on each generation, the algorithm maintains a set of elite synthetic datasets. Then, the algorithm uses this elite set to produce the population for the next round by crossing samples (i.e., combining parameters) and applying specific mutations (i.e., perturbing parameters). For the purpose of private synthetic data, we devise new strategies for crossing and mutating samples.

Given that our method only requires zeroth-order access to any objective function, we demonstrate that \privGA{} can directly optimize over a wide range of statistical queries that capture various statistical properties summarizing both discrete and real-valued data attributes. Specifically, we first conduct experiments in mixed-type data domains, evaluating on random (1) halfspace and (2) prefix queries. We then explore categorical-only data, in which we use (3) $k$-way categorical marginal queries. Lastly, we again evaluate \privGA{} on mixed-type data using (4) $k$-way range marginal queries. Note that (3) and (4) can be represented as differentiable functions, while (1) and (2) cannot.

We summarize our contributions as the following:
%
\begin{itemize}[noitemsep,topsep=0pt]
    \item We present \privGA{}, a versatile genetic algorithm that can generate synthetic data to approximate a wide range of statistical queries, regardless of their differentiability. To achieve this, we develop novel crossover and mutation functions that are crucial to the success of \privGA{} across various statistical queries. 
    \item We conduct an empirical evaluation on data derived from the American Community Survey. We note that our method is highly parallelizable, scaling to the high-dimensional data settings explored in our experiments.
    \item In the mixed-type data domain, we show that \privGA{} outperforms the state-of-the-art method, \rappp{}, on non-differentiable queries (i.e., halfspace and prefix queries). Furthermore, we show that \emph{even} for differentiable query classes (i.e., $k$-way categorical and range marginals), \privGA{} matches first-order optimization methods.\footnote{Our work is also the first to modify our baseline methods, \rap{} and \gem{}, to optimize over $k$-way range marginals for mixed type data, with the limitation being that real-valued attributes are discretized first.}
\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{images/acs_histplot2.png}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}
\paragraph{Additional related work.}
\iffalse
% Introduce early synthetic data mechanisms  
 \smallDB{} \citep{BLR08}, one of the first private synthetic data mechanisms, searches the space of small datasets consistent with the original data schema and selects the dataset that best matches the answers on the original dataset. However, \smallDB{} is computationally intractable as it needs to enumerate the search space of all possible small datasets, which is exponential in the data dimension. A more practical approach, proposed in \citet{MWEM}, is the Multiplicative-Weights-Exponential-Mechanism (\mwem) with optimal sample complexity for the query release problem. The \mwem{} algorithm is more practical than \smallDB{} but is still computationally intractable for data dimensions commonly found in real-world datasets. 
 % Describe the history of Oracle efficient mechanisms
 \dualquery{} \citep{gaboardi2014dual} and \fem{} \citep{Vietri2019NewOA} can be viewed as efficient versions of \mwem{}, where the computationally hard step is replaced by a practical optimization heuristic. Both \dualquery{} and \fem{} have worse sample complexity than \mwem{} but are more scalable for higher dimensional data.\fi

  % is the \smallDB{} algorithm by \citet{BLR08}.  \smallDB{} \citep{BLR08}, one of the first private synthetic data mechanisms, searches the space of small datasets consistent with the original data schema, then runs a differentially private mechanism to select the small dataset that best matches the answers on the original dataset. As a result, the \smallDB{} algorithm can accurately answer exponential in $n$ many statistical queries, whereas the Gaussian mechanism only answers $O(n^2)$ queries. However, the issue with \smallDB{} is that it is computationally intractable as it needs to enumerate the search space of all possible small datasets, which is exponential in the data dimension. A more practical approach, proposed in \citet{MWEM}, is the Multiplicative-Weights-Exponential-Mechanism (\mwem) with optimal sample complexity for the query release problem. The \mwem{} algorithm is more practical than  \smallDB, but it is still computationally intractable for high enough dimensional data. The reason is that \mwem{} must maintain a probability distribution over the data domain, which is exponentially large in the number of attributes in the data.

% PGM
In addition to algorithms \rap{}, \gem{}, and \rappp{} \cite{aydore2021differentially, liu2021iterative, vietri2022private}, another benchmark algorithm that uses first-order optimization is the PrivatePGM (\pgm{}) algorithm \citep{mckenna2019graphical} and its variations \citep{mckenna2022aim}.  Similar to \rap{} and \gem{}, \pgm{} does not directly does not support non-differentiable queries such as thresholds and half-spaces on real-valued data. While one can first discretize numerical features, \citet{vietri2022private} show that \rappp{} still performs better than \pgm{} on real-valued data for approximating prefix queries and downstream machine learning. Finally, there is a line of work \citep{XieLWWZ18, JordonYvdS18, gan2, gan3, vae, harder2021dp} that develops differentially private algorithms for training deep generative models (e.g., GANs, VAEs, etc.), but they generally have not shown promising results for enforcing consistency with simple classes of statistics when applied to tabular data \citep{tao2021benchmarking, vietri2022private}. As a result, we do not compare against these approaches.


\iffalse
\paragraph{Limitations of data discretization.}
Discretizing real-valued features and running a suitable method can produce high-quality results in specific scenarios. However, this approach has its limitations. Discretization can be computationally expensive, particularly when a high resolution of the real-value features is required and the data contains many real-valued features. 
% For example, if $b$ bins are used to discretize $r$ real-valued columns, the resulting discretized dataset will have a dimension of $b \cdot r$. 
Additionally, discretization is limited in terms of the types properties one can optimize for. In this work, we focus on answering a random halfspace and prefix queries, which would be impossible to discretize to such a fine granularity for.
% Another class of queries, halfspace queries, which capture linear properties of the real-valued features, cannot be directly encoded by discretization even with infinite granularity. 
% Therefore, discretization is a reasonable strategy for some settings but may not be the best solution for all types of queries and problems.


\paragraph{Limitations of a recent first-order approach for real-valued data.}
For data with real-valued features, a common task is to approximate prefix queries\footnote{An example of a prefix query is: "How many people in dataset $D$ have a salary less than $10K$".} under differential privacy. Recently, \citet{vietri2022private} introduces a first-order algorithm \rappp{} for preserving any threshold-based queries, including prefix queries, and operates over real-valued data by using a differentiable relaxation of the optimization problem. However, the relaxation step introduces a new source of error, potentially leading to catastrophic outcomes in which the the algorithm find a local minimum very far from the optimal solution.\footnote{We provide a simple example in Appendix \ref{appx:rappp}.}
\fi
% \input{docs/rap++_v2}

==> icml/docs/intro_old.tex <==
\section{Introduction}

% \color{red}

% \subsection{Text TODO}

% \begin{itemize}

%     \item Reduce text about history of synthetic data:
%     \item   how the algorithm handles columns of different variance. Show how crossover handles this naturally.
%     \item  Add oracle theorem 
%     \item Describe in text time-based early stop.
% \end{itemize}

% \subsection{experiments TODO}
% TODO:
% \begin{enumerate}
%     \item Compare PrivGA vs GEM/RAP on mixed data. 
%     \item Implement RAP++ for range queries and prefix queries.
%     \item Estimate conditional halfspaces. Compare against RAP++.
%     \item Parameter analysis of PrivGA and RAP. Add a plot of error vs runtime.
%     \item Multi-task machine learning .
% \end{enumerate}

% \paragraph{Other ideas:} A list of other features we could include:
% \begin{enumerate}
%     \item Logistic regression queries: Answer a bunch of logistic regression queries with objective perturbation and project using PrivGA. 
%     \item Add fairness constraints. A model trained on synthetic data should be fair.
% \end{enumerate}


% \subsection{Main document plot list}
% \begin{enumerate}
%     \item Categorical-marginals plot for only one task (mobility). This plot includes PrivGA, RAP, GEM and PGM.
%     \item Range-marginals for 5 tasks. This plot includes PrivGA, RAP, GEM, PGM and RAP++.
%     \item 
% \end{enumerate}

% \color{black}
 
% In this work, we consider the problem of generating synthetic data under differential privacy \cite{dwork2006calibrating} with a focus on answering a large collection of statistical queries. 
% Some approaches to producing synthetic data follow the generative adversarial network (GAN) framework due to  \cite{goodfellow2014generative}. Private implementations of the GAN framework are based on private-stochastic gradient descent (DP-SDG)  (see \cite{}). However, these methods do not perform well in practice \gv{why?}. In this work, we consider a different paradigm that consists of allocating the privacy noise to answer a selected collection of statistical queries and then finding a synthetic dataset consistent with the query answers. 
%
% The problem of releasing statistics subject to privacy has been extensively studied \cite{MWEM}.

% Introduce the problem
Access to high-quality data is critical for decision-making and data analysis. However, the use of sensitive data can reveal private information about the individuals in the data, such as medical conditions or financial status. Therefore, privacy concerns impose legal and ethical constraints on the kind of data one can access for data analysis. In this work, we consider the task of releasing an extensive collection of statistical queries that respect the privacy of individuals in the data. \swcomment{should talk about synthetic data instead} A {\em statistical} query (SQ) is a function that counts the number of individuals in a dataset that satisfy a specific property---releasing statistics forms a fundamental operation for a wide range of data analysis tasks. Furthermore, we consider approximating the statistical queries subject to the formal requirement of \emph{differential privacy} \cite{dwork2006calibrating} to preserve privacy. 



The most straightforward differential privacy mechanism is to add a small amount of perturbation to the answer to each query. However, this simple solution only scales when we are required to approximate many statistical questions. Therefore, in this work, we are interested in generating synthetic data under the constraint of differential privacy consistent with many statistical queries. To formulate the problem more formally, we introduce some notation. Let $D$ sensitive data, and let $Q(D)\in [0, 1]^m$ encode the answer to $m$ queries. Then, the goal is to find a synthetic dataset $\Dhat$ under differential privacy such that the distance between $Q(\Dhat)$ and $Q(D)$ is close.
\gvdelete{
A simple and differentially private mechanism for releasing
approximate statistics is the Gaussian mechanism, which
perturbs the answers of each query with independent Gaussian noise. However, the Gaussian mechanism's error grows fast with the number of queries we want to approximate. For instance, the Gaussian mechanism cannot approximate more than $m=O(n^2)$ statistical queries, where $n$ is the data size, and more generally, there exists no efficient mechanism for approximating exponentially many queries \citep{ullman2013answering}.}

The synthetic data approach provides several advantages. For example, \citet{BLR08} proved that releasing private synthetic data can approximate an exponential number of queries in the dataset size. In contrast, the mechanism that only perturbs the query answers can approximate $O(n^2)$ queries. In addition, synthetic data is reusable for additional analysis without degrading users' privacy. For example, synthetic data trained to preserve statistical queries be used as training data for machine learning or to augment existing datasets.

\gvdelete{
Today, there exist many differentially private mechanisms for generating synthetic data, but they often are limited to the types of data they can produce and the classes of queries they support. For example, recent work focuses on approximating marginal queries\footnote{A {\em marginal} query is a function that counts the fraction of rows in a dataset where a particular set of attributes matches specific values. For example, a marginal query is: "How many people in dataset $D$ are Asian and live in NYC."} 
%
for discrete datasets by leveraging first-order optimization techniques \cite{aydore2021differentially, liu2021iterative}. The central idea of these first-order methods is to solve an optimization problem for finding synthetic data to match the given statistics. }
Today, there exist many efficient differentially private mechanisms for generating synthetic data, but most have limitations. For example, recent work focuses on approximating marginal queries\footnote{A {\em marginal} query is a function that counts the fraction of rows in a dataset where a particular set of attributes matches specific values. For example, a marginal query is: "How many people in dataset $D$ are Asian and live in NYC."} for discrete datasets by leveraging first-order optimization techniques \cite{aydore2021differentially, liu2021iterative}. The first-order methods first access the query answers by perturbing the query answers to obtain a set of noisy measurements $\hat{a} = Q(D) + z$ that satisfy differential privacy. Then learn a synthetic dataset $\Dhat$ that minimizes the following objective:
%
\begin{align}\label{eq:objectiveI}
\| \hat{a } - Q(\Dhat) \|_2
\end{align}
%
%
\gvdelete{
The challenge is that the first-order methods require differentiability in the optimization objective. Nevertheless, when the objective is non-differentiable (as in learning synthetic data for matching statistics), it is still possible to design a differentiable surrogate function that approximates the original objective. 
Consequently, while prior work has shown that first-order methods are effective for approximating a broad class of marginal queries, the methods they propose are still limited only to matching marginals for discrete attributes.}
%
%
When the input data is discrete, and the queries are marginals, the objective \eqref{eq:objectiveI} is a discrete optimization problem. To address this challenge, \citet{aydore2021differentially, liu2021iterative} proposed a method for data domain relaxation into a continuous space and finding a differentiable surrogate function that approximates the original objective. 
This approach allows for applying efficient first-order optimization techniques to learn synthetic data in the relaxed space that approximates the queries. Finally, the synthetic data generated in the relaxed space can be reconstructed in the original data domain by sampling from a distribution defined by the relaxed dataset.

\swcomment{this narrative is pretty good. i think we should give a basic sense of what the optimization is for: given a set of (noisy) measurements, compute a synthetic data set that is consistent with the measurements.}\jtcomment{maybe we could move the part that introduces the projection mechanism here.}

% For data with real-valued features, a common task is to instead approximate prefix queries\footnote{An example of a prefix query is: "How many people in dataset $D$ have a salary less than $10K$".}
% %
% under differential privacy. 
% % The category of first-order methods may handle real-valued features by discretizing the values into $b$ discrete features, but more is needed. One issue is that discretization results in an explosion in the data dimension when there are many real-valued features. 
% Recent work by \citet{vietri2022private} introduces first-order approach to generate real-valued data to match prefix queries natively. However, their algorithm has some issues that arise from modifying the optimization objection. In the following, we describe the mechanism by \citet{vietri2022private} for approximating prefix queries and provide a simple example of where it fails. Then in the experiment section, we show how this bad case can happen for a real dataset.

% \paragraph{A First-Order Approach} 

In the scenario where the input data comprises contains real-valued features, there exist many natural classes of queries that involve using a threshold function. It is crucial to note that this threshold function is not differentiable. Some examples include range queries, prefix queries, and half-spaces. In light of this, the first-order technique proposed in \citet{aydore2021differentially, liu2021iterative} does not apply. Therefore, two approaches have been proposed in the literature to address the issue. The first approach involves discretizing the real-valued features, while the second involves relaxing the threshold queries by utilizing a soft threshold function, which preserves differentiability.

\paragraph{Limitations of data discretization}
The first approach of data discretization can be costly in terms of space and runtime if a high resolution of the real-value features is required.\gvcomment{More details...}
\input{docs/rap++_v2}



\subsection{Contributions} 
% Explain the projection mechanism since it underpins all other methods. Why gradient based methods overcame oracle-efficient methods.
\gvdelete{
Our approach falls under the framework of the projection mechanism by \citet{HT10}. The projection mechanism consists of two steps: First, it estimates the statistics using the Gaussian mechanism to get the approximate vector answers $\hat{a}\in\mathbb{R}^m$. Then, it projects $\hat{a}$ to the set of answer vectors consistent with some dataset to obtain a final vector $a'\in\mathbb{R}^m$. The projection mechanism obtains optimal average error for approximating statistical queries with differential privacy. Still, the projection step corresponds to solving a difficult discrete optimization problem intractable in the high dimensional setting. Therefore, the strategy used in this work is to approximate the projection step using efficient optimization heuristics. 
}
% RAP/GEM techniques rely on the query structure.
% Only work for categorical data. Limited to the types of queries.
% Recently proposed mechanisms approximate the projection step efficiently  \cite{aydore2021differentially, liu2021iterative, vietri2022private} via first-order optimization techniques. These first-order mechanisms use the marginal queries' structure to relax the projection step's discrete objective and obtain a differentiable loss function, which may be non-convex. Then, the algorithm runs off-the-shelf differential optimization algorithms to minimize the relaxed objective. While such gradient-based optimization algorithms are not guaranteed find an optimal solution, such approaches have been more effective and efficient for answering large classes of marginal queries than their oracle-efficient predecessors. However, despite their success, these first-order mechanisms have a fundamental limitation in which the need to modify the objective introduces an additional source of error that may sometimes result in catastrophic failures. Furthermore, the first-order mechanisms are limited to approximating queries that can be expressed in differentiable forms.




% Why we need new methods for real-valued data
% A fundamental limitation of mechanisms described so far is that they only operate over discrete data, which can be problematic when the data we are trying to approximate contains real-valued features. A simple but impractical way to handle real-valued features is by discretizing. The most typical strategy is discretizing the data into a finite number of categorical bins. However, discretizing data is impractical because choosing the correct parameters  (i.e., how many bins to use) is challenging. The recent work by \citet{vietri2022private} provides a mechanism $\rppp$ that follows from the same framework as  $\rp$ \cite{aydore2021differentially} but operates natively over real-valued data. \citet{vietri2022private} shows that $\rppp$ outperforms all other methods that rely on discretization for estimating real-value data. 

% Describe RP++ and how it fails 


% A approach for query answering is using synthetic data.
% The objective is to produce a synthetic dataset $\Dhat$ that has the same schema as $D$, consistent with $D$ on all queries $Q$.
%  To preserve privacy, we perturb the statistics $Q(D)$ using a simple Gaussian noise mechanism to obtain a vector of noisy statistics $\hat{a}$. Given the set of queries $Q$ and the noisy statistics $\hat{a}$, one can define an optimization problem as follows  
% \begin{align}\label{eq:dhaterror}
%   f_{Q, \hat{a}}(\Dhat) = \|\hat{a} - Q(\Dhat) \|
% \end{align}

% The focus of this paper is finding better solutions to \ref{eq:dhaterror} that are currently available. 

Our main contribution \privGA{} is a \emph{zeroth}-order optimization mechanism for the projection step. Our mechanism avoids limitations of first-order methods used in prior work \cite{vietri2022private} by avoiding data relaxation or using surrogates of the objective, which are an additional source of error.  
% Our methods have the following advantages: 
%
Our mechanism adapts from a simple genetic algorithm by \citet{such2017deep} that evolves a population of datasets over $G$ generations—starting from a population of  $N$ randomly chosen datasets—where on each generation, the algorithm keeps a small set of elite synthetic datasets. Then, the algorithm uses the elite set to produce the population for the next round by crossing elite members (or combining parameters) and applying specific mutations to the parameters. Our crucial innovation is a special rule for {\em crossing} and {\em mutating} elite synthetic datasets that produce quality candidates for subsequent generations.

    
Our algorithm only requires zeroth-order access to the objective function and outperforms the first-order methods when the query class contains prefix queries, and the data is real-valued data. Furthermore, the mechanism is highly parallelizable, as shown in \citet{such2017deep}, making it very scalable for high-dimensional data settings.
\jtcomment{We might keep it consistent when using words "our algorithm", "our mechanism" and "\privGA{}"}

% \begin{enumerate}
%     % \item An evolution mechanism outperforms the prior work \cite{vietri2022private} on real-valued data. Avoids the limitations of gradient-based methods. 
%     \item The zeroth-order optimization algorithm outperforms the first-order methods when the query class contains threshold based queries and the data is mixed type.
%     \item Because our zeroth-order approach does not need to compute gradients,  our methods make no modifications to the original objective, enabling us to to preserve a general class of queries outside of just statistical queries.
% \end{enumerate}



\paragraph{Additional related work.}

% Introduce early synthetic data mechanisms  
One of the first synthetic data mechanisms is the \smallDB{} algorithm by \citet{BLR08}.  \smallDB{} searches the space of small datasets consistent with the original data schema, then runs a differentially private mechanism to select the small dataset that best matches the answers on the original dataset. As a result, the \smallDB{} algorithm can accurately answer exponential in $n$ many statistical queries, whereas the Gaussian mechanism only answers $O(n^2)$ queries. However, the issue with \smallDB{} is that it is computationally intractable as it needs to enumerate the search space of all possible small datasets, which is exponential in the data dimension. A more practical approach, proposed in \citet{MWEM}, is the Multiplicative-Weights-Exponential-Mechanism (\mwem) with optimal sample complexity for the query release problem. The \mwem{} algorithm is more practical than  \smallDB, but it is still computationally intractable for high enough dimensional data. The reason is that \mwem{} must maintain a probability distribution over the data domain, which is exponentially large in the number of attributes in the data.


% Describe the history of Oracle efficient mechanisms
Unfortunately, the computational barrier is unavoidable, but, despite the negative results\jtcomment{do we need to mention the negative results here?}, recent techniques have focused on leveraging different optimization heuristics to overcome the computational obstacle. For example, the mechanism \dualquery{} and \fem{} by \citet{gaboardi2014dual} and \citet{Vietri2019NewOA} respectively can be seen as efficient versions of \mwem, where the computational hard step in \mwem{} is replaced by a practical optimization heuristic such as an integer solver. Both  \dualquery{} and \fem{} have worse sample complexity than \mwem{} but are more scalable for higher dimensional data.


A  line of work that competes with the first-order approaches is the PrivatePGM algorithm by \cite{mckenna2019graphical}, and its variations \cite{mckenna2022aim}. This mechanism solves a high-dimensional convex optimization problem to find a distribution over a discrete data domain that best matches noisy answers to marginal queries. 
Since  PrivatePGM uses the structure of marginal queries and categorical data, it does not support real-valued data. To handle real-valued data with PrivatePGM, one can always discretize the data. However, then,  \citet{vietri2022private}  showed that   \rppp{} performs better than a variation of PrivatePGM (that discretizes real-valued features) on real-valued data for approximating prefix queries. Therefore, in this work, we primarily compare our method against \rppp{}.

% \gv{This is copy paste for now: } 
Finally, there is a line of work that has taken modern techniques for distribution learning (GANs, VAEs, etc.) but generally has not shown promising results for enforcing consistency with simple classes of statistics like marginal queries. As a result, we do not compare to approaches from this line of work.

==> icml/docs/prelims.tex <==


\section{Preliminaries}



\subsection{Datasets and Queries }
% \paragraph{}


% {Notation}
We use $\cX$ to denote a data domain where $d$ denotes the number of features in $\cX$, and $x\in \cX$ denotes an element from the data domain. 
% Let $d_i = |\cX_i|$ be the cardinality of the $i$-th feature.
For $x\in \cX$, we use $x_i$ to denote the $i$-th feature of $x$.
A dataset $D\in\cX^*$ is a multiset of values from a data domain $\cX$. In this work, we consider mixed-valued datasets with a bounded domain. The focus of this work is on answering statistical queries. A statistical query is a bounded function  $q:\cX^* \rightarrow [0,1]$ that maps a dataset to a bounded real value. The formal definition is 
\begin{definition}[Statistical Query \citep{kearns1998efficient}]
    A \emph{statistical query} is defined by a predicate function $\phi:\cX\rightarrow\{0,1\}$. Given a dataset $D\in \cX^n$, the corresponding statistical query $q_\phi$ is defined as : $q_\phi(D) = \frac{1}{n}\sum_{x\in D} \phi(x)$. 
\end{definition}



We use $Q=\{q_i, \ldots, q_m\}$ to represent a set of $m$ statistical queries and for a given dataset $D$, we use
$Q(D) = [q_1(D),\ldots, q_m(D)] \in [0,1]^m$ to denote the answers of all $m$ statistical queries on $D$.


In this work, we are interested in answering different types of statistical queries that capture different statistical properties. The first type is the class of categorical marginals, which has been the primary focus of most prior works. The \emph{$k$-way categorical marginal} queries count the fraction of rows in a dataset that matches a combination of values.

% capture the relationship between categorical features. 

% \begin{definition}[Categorical marginals ]
% \end{definition}
\begin{definition}[Categorical Marginal Queries]\label{def:cat_marginals}
A $k$-way \textit{categorical marginal} query is defined by a set of categorical features $S$ of cardinality $|S|=k$, together with a particular element $c\in \prod_{i\in S} \cX_i$ in the domain of $S$.  Given such a pair  $(S, c)$, let $\cX(S, c)=\{x \in \cX : x_S = c \}$ denote the set of points that match $c$. The corresponding statistical query $q_{S, c}$ is defined as $q_{S,c}(D) = \sum_{x\in D}\mathbbm{1}\{x\in \cX(S, c)\}$, 
% \begin{align*}
%     q_{S,c}(x) = \mathbbm{1}\{x\in \cX(S, c)\}.
% \end{align*}
where $\mathbbm{1}$ is the indicator function.
\end{definition}

For real-values features, we define the class of \emph{range} queries or \emph{$k$-way range-marginals} that capture the $k$.  A $1$-way range query is defined by an attribute $A$ and two real-values $a, b\in [0,1]$ and counts the number of rows where real-valued attribute $A$ lies in $[a, b]$.

% \begin{definition}[ Range marginals ]
% \end{definition}
\begin{definition}[Range Marginal Queries]\label{def:range_marginals}
 A $k$-way \textit{range marginal} query is defined by a set of categorical features $C$, an element $y\in \cX_C$, a set of numerical features $R$ and a set of intervals $\tau=\{[\tau_{j,0}, \tau_{j,1}]\}_{j\in R}$, with $|C| + |R| = k$ and $|R| = |\tau|$.
Let $\cX(C, y)$ be as in \cref{def:cat_marginals} and let $\cR(R, \tau) =\{x\in\cX : \tau_{j, 0} \leq x_j \leq \tau_{j, 1} \quad \forall_{j\in R}\}$ denote the set of points where each feature $j\in R$ fall below its corresponding threshold value $\tau_j$.
% and $\cX(R, \tau)$ be as in \cref{def:prefix}.
Then the statistical query $q_{C, y, R, \tau}$ is defined as $$    q_{C, y, R, \tau}(D) =\sum_{x\in D} 
   \mathbbm{1}\{x\in \cX(C, y) \} \cdot   \mathbbm{1}\{x\in \cR(R, \tau) \} .$$ 
% The corresponding statistical query is defined by a component-wise product of a marginal vector $\mu_{C, x} $ (defined in \cref{def:marginals}) and a prefix marginal query: 
% \begin{align*}
%     q_{C, y, R, \tau}(x) = 
%   \mathbbm{1}\{x\in \cX(C, y) \} \cdot   \mathbbm{1}\{x\in \cX(R, \tau) \} .
%     % \mu_{C, x} \cdot   \prod_{i\in R}\mathbbm{1}\{ x_i \leq \tau(i) \}
% \end{align*}
\end{definition}

We note that while range marginal queries are useful for capturing statistical properties of real-valued data, they can also be applicable to discretized data. For example, one can discretize a real-valued column into the bins that are a superset of the intervals $\tau$ defined in Definition \ref{def:range_marginals}.\footnote{In Section \ref{sec:experiments} and the appendix, we will discuss how range marginal queries are still applicable to \gem{} and \rap{}, which handle real-valued attributes by discretizing them first.}

We define a \emph{workload} as the set of marginal queries defined by some set of features (i.e., $S$ for categorical marginals and $C \cup R$ for range marginals).

Next, we present two additional queries---halfspace and prefix queries---that are also useful in summarizing real-valued features. We emphasize that such queries are the focus of our work, since they cannot be directly optimized by existing methods using first-order optimization. These queries can in some ways be thought of as higher-dimensional generalizations of CDF functions. Moreover, synthetic data matching statistical properties defined by these queries have been shown to do well on downstream tasks like machine learning classification \citep{vietri2022private}.

\begin{definition}[Halfspace Query]\label{def:halfspace}
% For a numerical data domain $\cX = \mathbb{R}^d$.
A \textit{halfspace} query is defined by a categorical feature $i$,
 a target value  $y\in\cX_i$,
a set of numerical features $R$,  a vector $\theta\in\mathbb{R}^{|R|}$ and a threshold $\tau\in \mathbb{R}$ as $    q_{i, y, R, \theta, \tau}(D) =\sum_{x\in D}  \mathbbm{1}\{\dotp{\theta, x_R} \leq \tau \text{ and } x_i = y\} .$
% \begin{align*}
%     q_{i, y, R, \theta, \tau}(x) =  \mathbbm{1}\{\dotp{\theta, x_R} \leq \tau \text{ and } x_i = y\} .
% \end{align*} 
\end{definition}

\begin{definition}[$k$-way prefix queries]\label{def:prefix}
A $k$-way prefix query is defined by a set of real-valued features $C\subseteq [d]$ ($|C|=k$) and a set of threshold $\tau=\{\tau_i \in [0,1]: i\in C\}$. Let $\cX(C, \tau) =\{x\in\cX : x_i\leq \tau_i \quad \forall i\in C\}$ be the set of points, that has each feature $i\in C$ fall below the corresponding threshold $\tau_i$. Then the prefix query $q_{C, \tau}$ is given by $q_{C, \tau}(D) = \sum_{x\in D} \mathbb{I}\{x\in \cX(C, \tau)\}$.
\end{definition}

% Finally, our goal is to accurately estimate statistical queries according to $\ell_{\infty}$, $\ell_2$ and $\ell_1$ error:
% \begin{definition}
% Let $D\in \cX^n$ be a dataset and $Q$ be a set of statistical queries. Then the $\ell_p$-error of a synthetic dataset $\Dhat^{n'}$ is $\|Q(D) - Q(D')\|_p$.
% \end{definition}

\subsection{Differential Privacy} 
% The fundamental problem we address in this paper is releasing the statistics $Q(D)\in [0,1]^m$ when the dataset $D$ may contain sensitive information.  
To protect user privacy, we estimate $Q(D)$ under the constraint of differential privacy \cite{dwork2006calibrating}, which is a widely accepted notion of privacy protection at the user level. 
% Differential privacy allows one to control the trade-off between how much one can learn about a population and how much data leakage is acceptable on the user level. 
For example, the US Census Bureau has begun using differential privacy to protect the privacy of individuals when releasing census data. Differential privacy is used to add noise to the census data in order to obscure the data of any one individual, while still providing accurate statistical information about the population as a whole.

To define differential privacy, we say that two datasets are neighboring if they are different in at most one data point. We give the formal definition here:
\begin{definition}[Differential Privacy (DP) \cite{dwork2006calibrating}]\label{def:dp}
A randomized algorithm $\mathcal{M}:\cX^n\rightarrow \cR$ satisfies $(\varepsilon, \delta)$-differential privacy if 
for all neighboring datasets $D, D'$ and for all outcomes $S\subseteq \cR$ we have
%
\begin{align*}
    \pr{\mathcal{M}(D) \in S} \leq e^{\varepsilon} \pr{\mathcal{M}(D') \in S}+\delta
\end{align*}
\end{definition}

A related notion we use is {\em zero-Concentrated Differential Privacy} (zCDP) \cite{DworkR16, BunS16}, which has a simpler privacy composition.

\begin{definition}[zCDP \cite{bun2016concentrated}]\label{def:zcdp}A randomized algorithm $\mathcal{M}:\cX^n\rightarrow \cR$ satisfies $\rho$-zero differential privacy ($\rho$-zCDP) if 
for all neighboring datasets $D, D'$ and for all $\alpha\in(1,\infty)$ we have: $\mathbb{D}_{\alpha}(\mathcal{M}(D),\mathcal{M}(D'))\leq\rho\alpha$, where $\mathbb{D}_{\alpha}(\mathcal{M}(D),\mathcal{M}(D'))$ is $\alpha$-Renyi divergence between the distributions $\mathcal{M}(D)$ and $\mathcal{M}(D')$.
\end{definition}

The composition property is given by the following result:
\begin{lemma}[zCDP Composition, \cite{bun2016concentrated}]\label{lemma:comp} Let $\mathcal{A}_1:\mathcal{X}^n\rightarrow R_1$ be $\rho_1$-zCDP. Let $\mathcal{A}_2:\mathcal{X}^n\times R_1 \rightarrow R_2$ be such that $\mathcal{A}_2(\cdot,r)$ is $\rho_2$-zCDP for every $r\in R_1$. Then the algorithm $\mathcal{A}(D)$ that computes $r_1=\mathcal{A}_1(D), r_2=\mathcal{A}_2(D,r_1)$ and outputs $(r_1,r_2)$ satisfies  $(\rho_1+\rho_2)$-zCDP.
\end{lemma}

Any mechanism that satisfies zCDP also satisfies DP.
\begin{theorem}[zCDP to DP]
    If $M$ provides $\rho$-zCDP, then $M$ is $(\rho+2\sqrt{\rho\log(1/\delta)},\delta)$-differentially private for any $\delta>0$.
\end{theorem}



We will use the post-procession properties of zCDP in our analysis. Essentially, there is no loss of privacy  when doing an operation on the output of a zCDP mechanism. 
\begin{lemma}[Post-processing]\label{lemma:post} Let $M:\mathcal{X}^n\rightarrow\mathcal{Y}$ and $f:\mathcal{Y}\rightarrow\mathcal{Z}$ be randomized algorithms. Suppose $M$ satisfies $\rho$-zCDP. Define $M':\mathcal{X}^n\rightarrow\mathcal{Z}$ by $M'(X)=f(M(X))$. Then $M'$ satisfies $\rho$-zCDP.
\end{lemma}

% Finally, a related notion of privacy is called concentrated differential privacy (zCDP) \cite{DworkR16,BunS16}, which enables cleaner composition analyses for privacy. 
%
%
%%%%%%%%%%%%%%%%%
%% Def 
%%%%%%%%%%%%%%%%%
% \begin{definition}[Concentrated DP,  \cite{DworkR16,BunS16}]\label{def:zCDP}
%  A randomized mechanism $\cM:\cX^n \rightarrow \cR$ is ${\rho}$-CDP, if for all neighboring datasets $P, P'$ (i.e., differing on a single person), and for all $\alpha\in(1,\infty)$,
%  \begin{align*}
%      \rendiver{\alpha}{\cM(P)\parallel\cM(P')} \leq \rho\alpha
%  \end{align*}
%  where $\rendiver{\alpha}{\cM(P)\parallel\cM(P')}$ is the R\'{e}nyi divergence between the distributions $\cM(P)$ and $\cM(P')$.
% \end{definition}


% Our synthetic data algorithm uses two  primitive  functions for privately selecting and answering low sensitive queries the exponential mechanism and the Gaussian mechanism. 
We use the Gaussian mechanism for privately estimating a subset of statistical queries, which perturbs the statistics with Gaussian noise scaled by the queries' sensitivity. A query of the data has low sensitivity if a small change in the data produces a small change in the output. Formally, let $\Delta(Q)$ denote the $\ell_2$-sensitivity  of vector-valued query $Q$, where $ \Delta(Q) = \max_{\text{neighboring } D,D'} \| Q(D) - Q(D')\|_2$. 

\begin{definition}[Gaussian Mechanism]\label{def:gaussian}
Let $Q:\cX^n \rightarrow \mathbb{R}^m$ be a function of the dataset. The Gaussian mechanism on input $D\in \cX^n$ , $Q$, and $\rho>0$, outputs $Q(D) + \cN\pp{0, \tfrac{\Delta(Q)^2}{2\rho}\cdot \mathbb{I}}$. 
%
And the Gaussian mechanism satisfies $\rho$-zCDP \cite{bun2016concentrated}.
\end{definition}


We will also use the private selection algorithm \emph{report noisy max} \cite{durfee2019practical} with Gumbel perturbation noise, whose output distribution is identical to that of the exponential mechanism \cite{mcsherry2007mechanism}.

\begin{definition}[Report Noisy Max With Gumbel Noise]\label{def:rnm} The Report Noisy Max mechanism $RNM(D,q,a,\rho)$ takes as input a dataset $D\in\mathcal{X}^n$, a vector of $m$ statistical queries $q$, a vector of $m$ query answers $a$, and a zCDP parameter $\rho$. It outputs the index of the query with highest noisy error estimate, $i^*=\arg\max_{i\in[m]}(|q_i(D)-a_i|+Z_i)$ where each $Z_i\sim{\rm Gumbel}(1/\sqrt{2\rho}n)$. $RNM(\cdot,q,a,\rho)$ satisfies $\rho$-zCDP.
\end{definition}

% \begin{lemma}[\citet{dong2020optimal}]
%     For any vector of statistical queries $q$, vector of conjectured answers $a$, and zCDP parameter $\rho$, $RNM(\cdot,q,a,\rho)$ satisfies $\rho$-zCDP.
% \end{lemma}

% \paragraph{ML Queries}  Our algorithm takes as input a finite collection of statistical queries and a dataset $D$. Prior work on efficient private-synthetic-data generation required queries to be either marginal queries \cite{mckenna2019graphical, mckenna2022aim} or that the queries are differentiable in the data domain \cite{vietri2022private, aydore2021differentially, liu2021iterative}. In contrast, our mechanism can operate over a general class of statistical queries and is efficient for high-dimensional data domains. 

% We choose a class of queries consisting of random binary tree classifiers for our experiments. We denote it by $Q_{\text{tree}}$. Any query $q\in Q_{\text{tree}}$ maps a rows of data $x\in \cX$ to a random binary label $\{0,1\}$. By choosing a large set of queries, many will likely be good discriminators of real and synthetic data. Even though we choose specifically binary tree classifiers, our mechanism operates over any class.




% \paragraph{Downstream Applications:}
% A central tenet machine learning task is the ability learn models that generalize. However, in practice training machine learning models is an iterative process that that involves reusing the same dataset multiple times. Therefore, to validate the generalization properties of a machine learning algorithm, the typical practice is to separate a fraction of the dataset for evaluation. 
% Given a synthetic dataset we 
% We define a machine learning task by a triple $(\Dtrain ,\Dtest, \cH)$, where $\cH$ is a hypothesis space.. Then, the training is as follows: On each round $\in [T]$ a




% \paragraph{Techniques} Our techniques include a synthetic data algorithm that efficiently optimizes over a general class of statistical queries. Prior work in synthetic data generation can only answer either marginal queries or queries that can be expressed in a differentiable form, see \cite{aydore2021differentially, liu2021iterative, mckenna2019graphical, mckenna2022aim, Vietri2019NewOA, gaboardi2014dual}.

% Furthermore, we implement our mechanism to satisfy differential privacy and take advantage of the \emph{transfer theorem} due to \cite{jung2019new} to preserve generalization. We use the Gaussian mechanism with the sparse vector technique for the privacy implementation.




==> icml/docs/query_release_problem.tex <==
\section{Private Query Release via Synthetic Data} 

For the problem of estimating statistics $Q(D)$ subject to differential privacy, we follow the framework of the projection mechanism \cite{NKL, DworkNT15}. Suppose we are given $m$ statistical queries, represented by $Q$, and a dataset $D$, then the first step consists of independently perturbing every coordinate of $Q(D)$ to obtain a private estimate, denoted by $\hat{a}$. Given a privacy parameter $\rho$, the noisy answer vector is computed as follows:
\begin{align}\label{eq:gaussianmech}
    \hat{a} \leftarrow Q(D) + \cN\pp{0, \tfrac{\Delta(Q)}{2\rho}\cdot \mathbb{I}}
\end{align}


Then, the \emph{project} step involves finding a synthetic dataset $\Dhat$ that best explains the estimate $\hat{a}$. Finally, to represent the projection step, we define a loss minimization problem, where the loss function is defined by $\hat{a}$ and $Q$ as follows:
\begin{align}\label{eq:obj}
 L_{\hat{a}, Q} (\Dhat) =   \|\hat{a} - Q(\Dhat) \|_2^2
\end{align}


By the properties of the Gaussian mechanism and the post-processing property (Theorem \ref{lemma:post}), the projection mechanism framework satisfies  $\rho$-zCDP regardless of the optimization procedure used to solve \eqref{eq:obj}.

\input{icml/algorithms/privga.tex}

\paragraph{Adaptive Selection Framework.} In practice, when the number of queries $m$ is very large, the objective \eqref{eq:obj} becomes extremely noisy for any practical optimization routine. Therefore, we follow the Adaptive Selection Framework of \citet{liu2021iterative} that, over $K$ rounds, chooses high error queries adaptively using  the report noisy max mechanism (alternatively the exponential mechanism of \cref{def:exponential}). Algorithm \ref{alg:adaptive} of Appendix \ref{appx:adaptive} shows the details of this framework, which we note satisfies the following theorem:


\begin{theorem}\label{thm:privacy} For any $K$, $\rho>0$, dataset $D$, query set $Q$ and any procedure used to solve objective \eqref{eq:obj},  the adaptive framework  strategy satisfies $\rho$-zCDP. By extension, it also satisfies $(\varepsilon, \delta)$-differential privacy for: $\varepsilon = \rho+2\sqrt{\rho\cdot \log(1/\delta)}$.
\end{theorem}
We provide a proof sketch to Theorem \ref{thm:privacy} below.
\begin{proof}
In the adaptive selection framework, the report noisy max (RNM, \cref{def:rnm}) and Gaussian mechanism (GM, \cref{def:gaussian}) are both called $K$ times, each with a privacy budget of $\rho' = \rho / (2\cdot K)$. As shown in \cref{def:gaussian} and the work of \citet{durfee2019practical}, each individual call to RNM or GM satisfies $({\rho'})$-zCDP. Thus, by the composition properties outlined in \citet{bun2016concentrated}(see \cref{lemma:comp} ), the combination of $2\cdot K$ $\rho'$-zCDP mechanisms satisfies $\rho$-zCDP.\end{proof}
% \subsection{The Adaptive Selection Framework }

% \citet{HT10} shows that the projection mechanism is optimal for minimizing $\ell_2$ loss, as in objective \eqref{eq:obj}. However, in practice, when the number of queries $m$ is very large the objective \eqref{eq:obj} becomes extremely noisy for any practical optimization routine. Therefore, we follow a iterative strategy that chooses high error queries adaptively using the exponential mechanism or the report noisy max mechanism. Algorithm \ref{alg:adaptive} of Appendix \ref{appx:adaptive} shows the details of the adaptive framework.

==> icml/docs/rap++.tex <==
\subsection{Limitations of a recent first-order approach for real-valued data.}

% \subsection{First-Order Approach for Real-Valued Data}

% We first explain the solution first-order method by \cite{vietri2022private} that was tailored to approximate real-valued data. Furthermore, we give a example of how the algorithm can fail.

For data with real-valued features, a common task is to instead approximate prefix queries\footnote{An example of a prefix query is: "How many people in dataset $D$ have a salary less than $10K$".}
%
under differential privacy.
Recently, \citet{vietri2022private} introduced a first-order algorithm \rappp{} for preserving any threshold-based queries, including prefix queries, and operates over real-valued data. However, in modifying the optimization objective to derive an approximate loss function for such queries, various issues arise.

% The recent work by \citet{vietri2022private} gives a first-order algorithm \rppp{} for preserving any threshold-based queries, including prefix queries, and operates over real-valued data. 
% Recall, that the objective function is given by \eqref{eq:obj}. this section describes how \rppp{} works and gives an example of how it can fail to solve $\eqref{eq:obj}$.
To showcase such issues, consider a $1$-dimensional real-valued data domain $\cX = [0,1]$, and suppose that the goal is to approximate a single prefix query with a threshold of $0.5$. Let $f_{0.5}(x) = \mathbb{I}\{x \leq 0.5\}$ be the prefix function, then for a dataset $D$ with $n$ rows the corresponding statistical query is $Q(D) = \frac{1}{n}\sum_{x\in D} f_{0.5}(x)$. 
%
Ignoring, privacy constraints, our objective is to find a synthetic data $\Dhat$ that minimizes a loss function defined by the input data $D$ and the statistical query $Q$:
 \begin{align*}
     L_{D, Q}(\Dhat) = |Q(D) - Q(\Dhat)|
 \end{align*}
 %
 Since this loss function $  L_{D, Q}(\cdot )$ is not differentiable for such queries, the \rppp{} mechanism instead optimizes a differentiable relaxation of  $L_{D, Q}$. To achieve this, \rppp{} replaces the prefix query $f_{0.5}$, with a Sigmoid function, which have well-behaved gradients with adjustable magnitudes via the inverse temperature parameter. A {\em Sigmoid} function   with threshold $\tau$ and {\em inverse temperature parameter} $\invtemp$ is given by
\begin{align*}
    f_\tau^{[\invtemp]}(x)=\pp{{1+\exp(-\invtemp\cdot (x-\tau))}}^{-1}
\end{align*}
Finally, the prefix Sigmoid approximation is given by
$\widetilde{Q}_\invtemp(D) = \frac{1}{n}\sum_{x\in D} f_{0.5}^{[\invtemp]}(x)$. Ignoring privacy constraints, the \rppp{} algorithm's differentiable loss function becomes
%
\begin{align*}
    \widetilde{L}_{ D, Q,\invtemp}(\Dhat) = |Q(D) - \widetilde{Q}_\invtemp(\Dhat)|
\end{align*}
for a fixed inverse temperature parameter $\invtemp>0$ for  synthetic dataset $\Dhat\in [0,1]^{n'}$

% Since $Q$ consists of prefix queries (or any other threshold-based), the function $Q(\cdot)$ is not continuous everywhere and is not differentiable, thus not suitable for first-order optimization. Therefore, the fundamental idea behind the \rppp{} mechanism is to give a differentiable relaxation for the class of threshold-based statistical queries. The problem relaxation is achieved by replacing the function $Q(\cdot)$ by a differentiable approximation that we denote by $\tilde{Q}(\cdot )$. Then, \rppp{} uses the surrogate loss function given by $L_\invtemp (\Dhat) = \|\hat{a} -\widetilde{Q}(\Dhat) \|_2^2$, which is differentiable in $\Dhat$ by the chain rule.
%
% For example, a $1$-way prefix query  with threshold $\tau$ is defined by $q_{\tau}(D) =\frac{1}{n}\sum_{x\in D} f_\tau(x)$, where $D$ has $n$ rows and $f_\tau(x)= \mathbb{I}\{x \leq \tau\}$ is the prefix function. Then, the corresponding Sigmoid approximation with inverse temperature parameter $\invtemp$ is given by 
% \begin{align*}
%     \widetilde{q}_\tau^{[\invtemp]}(D) = \frac{1}{n}\sum_{x\in D} f_\tau^{[\invtemp]}(x)
% \end{align*}

% \paragraph{Optimization Failure Example}
% To showcase how the Sigmoid approximation leads to optimization issues, consider a $1$-dimensional real-valued data domain $\cX = [0,1]$. And suppose that the query set $Q$ consists of a single prefix query with a threshold of $0.5$. Let $f_{0.5}(x) = \mathbb{I}\{x \leq 0.5\}$ by the prefix function, and the corresponding statistical query be $Q(D) = \frac{1}{n}\sum_{x\in D} f_{0.5}(x)$. Finally,  the Sigmoid approximation is given by
% $\widetilde{Q}_\invtemp(D) = \frac{1}{n}\sum_{x\in D} f_{0.5}^{[\invtemp]}(x)$. Then, ignoring privacy constraints, the \rppp{} algorithm's loss function for a fixed inverse temperature parameter $\invtemp>0$ for  synthetic dataset $\Dhat\in [0,1]^{n'}$ is given by
% $$L_{Q, D,\invtemp}(\Dhat) = |Q(D) - \widetilde{Q}_\invtemp(\Dhat)|$$

Now, using a simple example, we show that \rppp{} can get stuck in a bad local minimum of the differentiable loss function. Suppose that the input data $D$ consist of $n/2$ entries with value equal to $0$ and $n/2$ entries with value equal to $1$, that is $D=\{0, \ldots, 0, 1, \ldots, 1\}\in [0,1]^n$. Then the input dataset $D$, evaluates to $Q(D) = 0.5$ on the prefix query (half the data points are bellow the $0.5$ threshold).
%
Next, consider the synthetic data point $\Dhat=\{0.5, \ldots, 0.5\}$, which evaluates to $\widetilde{Q}(\Dhat) = 0.5$  on the Sigmoid prefix function, then,  $\Dhat$ is a local minimum of the loss function $\widetilde{L}_{D, Q, \invtemp}$ ($\widetilde{L}_{D, Q, \invtemp}(\Dhat) = 0$).
%
% \begin{align*}
%     \widetilde{L}_{D, Q, \invtemp}(\Dhat) = |Q(D) - \widetilde{Q}_\invtemp(\Dhat)| 
%     = |0.5 - 0.5| = 0
% \end{align*}
%
However, when evaluated on the actual prefix query, the synthetic data point $\Dhat$ evaluates to $Q(\Dhat) = 1$. Therefore, the error on the original loss function is $L_{D, Q}(\Dhat)=0.5$.
% \begin{align*}
%   L_{D, Q}(\Dhat) =  |Q(D) - {Q}_\invtemp(\Dhat)| = |0.5 - 1| = 0.5
% \end{align*}

This simple example shows how the first-order optimization procedure by \citet{vietri2022private} can get stuck in a bad local minimum, resulting in a poor approximation of the statistical queries. Furthermore, in the experiment section, we will show that the \rppp{} algorithm fails in practice.

==> icml_ready/algorithms/gsd.tex <==

% \newcommand{\elite}{\mathcal{E}}

% \begin{algorithm}[!htb]
% \caption{Private Genetic Algorithm for Synthetic Data ($\GSD$) \label{alg:GSD}}
% \begin{algorithmic}[1]
% \STATE \textbf{Require:} The search space $\cX^{N'}$ of mixed-type synthetic datasets with $N'$ rows and $d$ features, number of generations $G$, population size $P$, elite  set size $E$.
% \STATE \textbf{Input:} A set of $m$ queries $Q:\cX^n \rightarrow [0,1]^m$, (noisy) query answers $\hat{a}\in [0, 1]^m$.

% \STATE Set the objective function for the synthetic datasets:
% \begin{align*}
%     L(\Dhat) = \| \hat{a} - Q(\Dhat)\|_2
% \end{align*}

% \STATE Initialize elite set $\elite_1 \leftarrow \{\Dbar_{1, i} \in \cX^{N'}: i \in [E]\}$ of synthetic datasets with $N'$ rows.
% \FOR{$g = 1, \ldots, G$}
    
%     \STATE Set $\Dhat^\star_{g} \leftarrow \argmin_{\Dhat \in \elite_{g}} L(\Dhat)$.

%     \STATE  Define a population of $P+E$ synthetic datasets:
%     $$\cP_g = \{\Dtil_{g, 1},\ldots, \Dtil_{g, P}\}\cup \elite_g$$
%     where each $\Dtil_{g, j}$ is generated as follows:
    
%     \FOR{$p=1, \ldots, P$}
    
%         \STATE \textbf{Mutate:} Sample a row $i\sim U([N'])$, feature $j\sim U([d])$ and set $\Dtil_{g, p}$ as 
% \begin{align*}
% \forall_{r\in [N'/2], c\in [d]}\quad 
% \Dtil_{g, p}(r, c) = 
%         \begin{cases} 
%          v \sim U\pp{\cX_j} & \text{ if } r = i \text{ and } c = j \\ 
%       \Dhat^\star_g(r, c) & \text{otherwise}
%     \end{cases}  
% \end{align*}

%         \STATE \textbf{Cross:} Sample two rows  $i_1, i_2\sim U([N'])$,  a feature $j\sim U([d])$, and elite member $\Dbar \sim U(\elite_g)$  and set $\Dtil_{g, p}$: 
%         \begin{align*}
% % \quad \text{such that}\quad 
% \forall_{r\in [N']\backslash [N'/2], c\in [d]} \quad 
% \Dtil_{g, p}(r, c) = 
%         \begin{cases}  \Dbar(i_2, c) & \text{ if } r = i_1 \text{ and } c = j \\ 
%       \Dhat^\star_g(r, c) & \text{otherwise}
%     \end{cases}  
% \end{align*}
%     \ENDFOR
%     \STATE Set $\elite_{g+1}$ as top $E$ members from population $\cP_g$  with respect to \emph{minimizing} objective $L(\cdot)$.
% \ENDFOR
% \STATE \textbf{return } $\Dhat_G^\star$
% \end{algorithmic}
% \end{algorithm}





% \begin{algorithm}[!htb]
% \caption{Private Genetic Algorithm for Synthetic Data ($\GSD$) \label{alg:GSD}}
% \begin{algorithmic}[1]
% \STATE \textbf{Require:} The search space $\cX^{N'}$ of mixed-type synthetic datasets with $N'$ rows and $d$ features, number of generations $G$, population size $P$, elite  set size $E$.
% \STATE \textbf{Input:} A set of $m$ queries $Q:\cX^* \rightarrow [0,1]^m$, (noisy) query answers $\hat{a}\in [0, 1]^m$.

% \STATE Set the objective function for the synthetic datasets:
% \begin{align*}
%     L(\Dhat) = \| \hat{a} - Q(\Dhat)\|_2
% \end{align*}

% \STATE Initialize elite set $\elite_1 \leftarrow \{\Dbar_{1, i} \in \cX^{N'}: i \in [E]\}$ of synthetic datasets with $N'$ rows.
% \FOR{$g = 1, \ldots, G$}
    
%     \STATE Set $\Dhat^\star_{g} \leftarrow \argmin_{\Dhat \in \elite_{g}} L(\Dhat)$.

%     \STATE  Define a population of $P+E$ synthetic datasets:
%     $$\cP_g = \{\Dtil_{g, 1},\ldots, \Dtil_{g, P}\}\cup \elite_g$$
%     where each member of $ \{\Dtil_{g, 1},\ldots, \Dtil_{g, P}\}$ is generated as follows:
    
%     \FOR{$p=1, \ldots, P / 2$}
    
%         \STATE \textbf{Mutate:} 
%         Initialize $\Dtil_{g, p}$ equal to $\Dhat_g^\star$. Then, sample a row $i\sim U([N'])$, feature $j\sim U([d])$ and value  $v \sim U\pp{\cX_j}$.  Update  $\Dtil_{g, p}$ as follows:
%         $$ \Dtil_{g, p}(i, j) \leftarrow v$$
%     % \begin{align*}
%     % \forall_{r\in [N'/2], c\in [d]}\quad 
%     % \Dtil_{g, p}(r, c) = 
%     %         \begin{cases} 
%     %          v \sim U\pp{\cX_j} & \text{ if } r = i \text{ and } c = j \\ 
%     %       \Dhat^\star_g(r, c) & \text{otherwise}
%     %     \end{cases}  
%     % \end{align*}


%     \ENDFOR
%     \FOR{$p=P/2+1, \ldots, P$}
%         \STATE \textbf{Cross:}Initialize $\Dtil_{g, p}$ equal to $\Dhat_g^\star$. Then, sample two rows  $i_1, i_2\sim U([N'])$,  a feature $j\sim U([d])$, and elite member $\Dbar \sim U(\elite_g)$ and update  $\Dtil_{g, p}$ as follows: 
%         $$\Dtil_{g, p}(i_1, j)  \leftarrow \Dbar(i_2, j) $$

        
% %         \begin{align*}
% % % \quad \text{such that}\quad 
% % \forall_{r\in [N']\backslash [N'/2], c\in [d]} \quad 
% % \Dtil_{g, p}(r, c) = 
% %         \begin{cases}  \Dbar(i_2, c) & \text{ if } r = i_1 \text{ and } c = j \\ 
% %       \Dhat^\star_g(r, c) & \text{otherwise}
% %     \end{cases}  
% % \end{align*}
%     \ENDFOR
%     \STATE Set $\elite_{g+1}$ as top $E$ members from population $\cP_g$  with respect to \emph{minimizing} objective $L(\cdot)$.
% \ENDFOR
% \STATE \textbf{return } $\Dhat_G^\star$
% \end{algorithmic}
% \end{algorithm}



\begin{algorithm}[!htb]
\caption{Private Genetic Algorithm for Synthetic Data ($\GSD$) \label{alg:GSD}}
\begin{algorithmic}[1]
\STATE \textbf{Require:} The search space $\cX^{N'}$ of mixed-type synthetic datasets with $N'$ rows and $d$ features, number of generations $G$, mutations population size $\Pmut$, crossover population size $\Pcross$ and elite  set size $E$.
\STATE \textbf{Input:} A set of $m$ queries $Q:\cX^* \rightarrow [0,1]^m$, (noisy) query answers $\hat{a}\in [0, 1]^m$.

\STATE Set the objective function for the synthetic datasets:
\begin{align*}
    L_{Q, \hat{a}}(\Dhat) = \| \hat{a} - Q(\Dhat)\|_2
\end{align*}

\STATE Initialize uniformly at random the elite set $\elite_1 \leftarrow \{\Dbar_{1, i} \sim U(\cX^{N'}): i \in [E]\}$ of synthetic datasets with $N'$ rows.
\FOR{$g = 1, \ldots, G$}
    
    \STATE Set $\Dhat^\star_{g} \leftarrow \argmin_{\Dhat \in \elite_{g}} L_{Q, \hat{a}}(\Dhat)$.

    \STATE Initialize candidate population set $\cP_g \leftarrow\elite_g$. 
    \STATE \textbf{Mutations: } Repeat $\Pmut$ times:  Initialize a synthetic data $\Dtil$ equal to $\Dhat_g^\star$. Then, sample a row $i\sim U([N'])$, feature $j\sim U([d])$ and value  $v \sim U\pp{\cX_j}$.  Update  $\Dtil$ as follows:
        $ \Dtil(i, j) \leftarrow v$ and add $ \Dtil$ to $\cP_g$.

    \STATE \textbf{Crossovers:} Repeat $\Pcross$ times: Initialize $\Dtil$ equal to $\Dhat_g^\star$. Then, sample two rows  $i_1, i_2\sim U([N'])$,  a feature $j\sim U([d])$, and elite member $\Dbar \sim U(\elite_g)$ and update  $\Dtil$ as follows:  $\Dtil(i_1, j)  \leftarrow \Dbar(i_2, j) $. Then add $\Dtil$ to $\cP_g$. 
        
    % \STATE  Define a population of $\Pmut + \Pcross + E$ synthetic datasets:
    % $$\cP_g = \{\Dtil_{g, 1},\ldots, \Dtil_{g, \Pmut}, \Dtil_{g, 1},\ldots, \Dtil_{g, \Pcross} \}\cup \elite_g$$
    % where each member of $ \{\Dtil_{g, 1},\ldots, \Dtil_{g, P}\}$ is generated as follows:
    
    % \FOR{$p=1, \ldots, P / 2$}
    
    %     \STATE \textbf{Mutate:} 
    %     Initialize $\Dtil_{g, p}$ equal to $\Dhat_g^\star$. Then, sample a row $i\sim U([N'])$, feature $j\sim U([d])$ and value  $v \sim U\pp{\cX_j}$.  Update  $\Dtil_{g, p}$ as follows:
    %     $$ \Dtil_{g, p}(i, j) \leftarrow v$$
    % \ENDFOR
    % \FOR{$p=P/2+1, \ldots, P$}
    %     \STATE \textbf{Cross:}Initialize $\Dtil_{g, p}$ equal to $\Dhat_g^\star$. Then, sample two rows  $i_1, i_2\sim U([N'])$,  a feature $j\sim U([d])$, and elite member $\Dbar \sim U(\elite_g)$ and update  $\Dtil_{g, p}$ as follows: 
    %     $$\Dtil_{g, p}(i_1, j)  \leftarrow \Dbar(i_2, j) $$
    % \ENDFOR
    \STATE \textbf{Update Elites:} Evaluate each member of $\cP_g$ on $L_{Q, \hat{a}}(\cdot)$. Then, set $\elite_{g+1}$ as top $E$ members from population $\cP_g$  with respect to \emph{minimizing} objective $L_{Q, \hat{a}}(\cdot)$.
\ENDFOR
\STATE \textbf{return } $\Dhat_G^\star$
\end{algorithmic}
\end{algorithm}

==> icml_ready/algorithms/gsd_efficient.tex <==


\newcommand{\elite}{\mathcal{E}}

\begin{algorithm}[!htb]
\caption{Private Genetic Algorithm for Synthetic Data ($\GSD$) \label{alg:GSD}}
\begin{algorithmic}[1]
\STATE \textbf{Require:} The search space $\cX^{N'}$ of mixed-type synthetic datasets with $N'$ rows and $d$ features, number of generations $G$, population size $P$, elite  set size $E$.
\STATE \textbf{Input:} A set of $m$ queries $Q:\cX^* \rightarrow [0,1]^m$, (noisy) query answers $\hat{a}\in [0, 1]^m$.

\STATE Set the objective function for the synthetic datasets:
\begin{align*}
    L(\Dhat) = \| \hat{a} - Q(\Dhat)\|_2
\end{align*}

\STATE Initialize elite set $\elite_1 \leftarrow \{\Dbar_{1, i} \in \cX^{N'}: i \in [E]\}$ of synthetic datasets with $N'$ rows.
\FOR{$g = 1, \ldots, G$}
    
    \STATE Set $\Dhat^\star_{g} \leftarrow \argmin_{\Dhat \in \elite_{g}} L(\Dhat)$.

    \STATE  Define a population of $P+E$ synthetic datasets:
    $$\cP_g = \{\Dtil_{g, 1},\ldots, \Dtil_{g, P}\}\cup \elite_g$$
    where each member of $ \{\Dtil_{g, 1},\ldots, \Dtil_{g, P}\}$ is generated as follows:
    
    \FOR{$p=1, \ldots, P / 2$}
    
        \STATE \textbf{Mutate:} 
        Initialize $\Dtil_{g, p}$ equal to $\Dhat_g^\star$. Then, sample a row $i\sim U([N'])$, feature $j\sim U([d])$ and value  $v \sim U\pp{\cX_j}$.  Update  $\Dtil_{g, p}$ as follows:
        $$ \Dtil_{g, p}(i, j) \leftarrow v$$
    % \begin{align*}
    % \forall_{r\in [N'/2], c\in [d]}\quad 
    % \Dtil_{g, p}(r, c) = 
    %         \begin{cases} 
    %          v \sim U\pp{\cX_j} & \text{ if } r = i \text{ and } c = j \\ 
    %       \Dhat^\star_g(r, c) & \text{otherwise}
    %     \end{cases}  
    % \end{align*}


    \ENDFOR
    \FOR{$p=P/2+1, \ldots, P$}
        \STATE \textbf{Cross:}Initialize $\Dtil_{g, p}$ equal to $\Dhat_g^\star$. Then, sample two rows  $i_1, i_2\sim U([N'])$,  a feature $j\sim U([d])$, and elite member $\Dbar \sim U(\elite_g)$ and update  $\Dtil_{g, p}$ as follows: 
        $$\Dtil_{g, p}(i_1, j)  \leftarrow \Dbar(i_2, j) $$

        
%         \begin{align*}
% % \quad \text{such that}\quad 
% \forall_{r\in [N']\backslash [N'/2], c\in [d]} \quad 
% \Dtil_{g, p}(r, c) = 
%         \begin{cases}  \Dbar(i_2, c) & \text{ if } r = i_1 \text{ and } c = j \\ 
%       \Dhat^\star_g(r, c) & \text{otherwise}
%     \end{cases}  
% \end{align*}
    \ENDFOR
    \STATE Set $\elite_{g+1}$ as top $E$ members from population $\cP_g$  with respect to \emph{minimizing} objective $L(\cdot)$.
\ENDFOR
\STATE \textbf{return } $\Dhat_G^\star$
\end{algorithmic}
\end{algorithm}

==> icml_ready/algorithms/privga.tex <==

\newcommand{\elite}{\mathcal{E}}

\begin{algorithm}[!htb]
\caption{Private Genetic Algorithm ($\privGA$) \label{alg:privGA}}
\begin{algorithmic}[1]
\STATE \textbf{Require:} The search space $\cX^n$ of mixed-type synthetic datasets with $n$ rows and $d$ features, number of generations $G$, population size $N$, elite  set size $E$.
% crossover function $\gamma:\cX^n\times\cX^n\rightarrow\cX^n$, mutation function $\psi:\cX^n\rightarrow\cX^n$.
% number of synthetic rows $n'$,
% privacy parameter $\rho>0$. \\
% \STATE\textbf{Input:} Dataset $D$, $m$ statistical queries $Q$.

% \STATE Privatize statistics $\hat{a} \leftarrow Q(D) + \cN\pp{0, \frac{m}{2\rho}}$ and set objective function:
% \begin{align*}
%   f_{Q, \hat{a}}(\Dhat) = \|\hat{a} - Q(\Dhat) \|
% \end{align*}
\STATE \textbf{Input:} A set of $m$ queries $Q:\cX^n \rightarrow [0,1]^m$, (noisy) query answers $\hat{a}\in [0, 1]^m$.

\STATE Set the objective function for the synthetic datasets:
\begin{align*}
    L(\Dhat) = \| \hat{a} - Q(\Dhat)\|_2
\end{align*}

{{\color{blue}\# Define sparse-mutation and row-crossover functions. }}
\FUNCTION{ Sparse Mutation $\psi(\Dhat)$:}
\item Uniformly sample a row $r\in[n]$, a column $c\in[d]$  and a value $v \sim \cX_c$ from the domain of feature $c$.
\item \textbf{Output} $\Dhat_{\text{muta}}$ where the value of its $r$-th row and $c$-th column is $v$ and everywhere else is equal to $\Dhat$.
\ENDFUNCTION

\FUNCTION{ Row Crossover $\gamma(\Dhat_a, \Dhat_b)$:}
\item Uniformly sample two rows $r_a, r_b\in[n]$.
\item \textbf{Output} $\Dhat_{\text{cross}}$ having all rows from $\Dhat_a$, except row $r_a$ is placed by row $r_b$ from $\Dhat_b$ .
\ENDFUNCTION
% \STATE \textbf{function} $\psi_\sigma(\Dhat)$: \\   
% % On input $\Dhat\in \Theta$ 
%     \hspace{2mm}  Randomly select a row $r\in[n']$, a column $c\in[d]$  and  $z \sim \cN(0, \sigma^2)$.
%       \textbf{output} $\Dtil$ where its $i$-th row and $j$-th column is given by
%     \begin{align*}
%     \Dtil_{i,j} =
%     \begin{cases}
%     \Dhat_{i,j} + z & \text{if } i = r \text{ and } j = c \\
%     \Dhat_{i,j} & \text{otherwise } \\
%     \end{cases}
%     \end{align*}


{{\color{blue}\# Run genetic algorithm with $\psi$ and $\gamma$. }}
\STATE Initialize elite set $\elite_1 \leftarrow \{\Dhat_{1, i} \in \cX^n: i \in [E]\}$.
\FOR{$g = 1, \ldots, G$}
    
    %  \STATE {{\color{blue}\# Mutate each elite parameter}}
    % \FOR{$\theta_{elite} \in \elite $}
    %     \STATE Add mutation $\psi(\theta_{elite})$ to next generation $ \cP^{g}$.
    
    % \FOR{$j=1,\ldots N$}
        
    %     \STATE Randomly sample two elite members $a,b\in [E]$. 
    %     % two parents $\Dhat_{g}^a, \Dhat_{g}^b\in \elite_g$
    %     % \STATE Randomly select two parents $\Dhat_{g}^a, \Dhat_{g}^b\in \elite_g$
    %     \STATE Apply crossover and and then mutate result:
    %     $$\Dhat_{g, j}^{\text{cross}} \leftarrow \psi\pp{\gamma\pp{\Dhat_{g, a}, \Dhat_{g, b}}}$$
    %      % \STATE Add $\Dhat_{g}^{\text{cross}}$ to $ \cP_{g}$.
    % \ENDFOR
    \STATE  Define a population of $N+E$ synthetic datasets:
    $$\cP_g = \{\Dhat_{g, 1}^{\text{cross}},\ldots, \Dhat_{g, N}^{\text{cross}}\}\cup \elite_g$$
    where each $\Dhat_{g, j}^{\text{cross}}$ is constructed by sampling two elite members  $a,b\in [E]$ and then applying crossover and and then mutating:
    %
    $$\Dhat_{g, j}^{\text{cross}} \leftarrow \psi\pp{\gamma\pp{\Dhat_{g, a}, \Dhat_{g, b}}}$$
    \STATE Set $\elite_{g+1}$ as top $E$ members from population $\cP_g$ that \emph{minimize} objective $L(\cdot)$.

   % \STATE {{\color{blue}\#  Find parameter from  $\cP^{g-1}$ that minimizes $L$}}
   %  \STATE Set elite $\Dhat^g_\star\leftarrow \argmin_{\theta\in \cP^{g-1}} L(\theta)$
   %  \STATE Add $\theta^g_\star$ to next generation $\cP^{g}$.
   %  \STATE {{\color{blue}\#  Choose best $T$ from $\cP^{g-1}$ to define the {\em elite} set.}}


    
    % \STATE Add $\Dhat^g_\star$ to $\cP^{g}$.
    % \STATE {{\color{blue}/\ /\ The next generation includes the $N-T-1$ off-spring, the  and the elite parameter }}
    % \STATE Set $\cP^g \leftarrow \{\theta_1,\ldots \theta_{N-T-1}\}\uplus \text{Elite}_{g} \uplus\{\theta^g_\star\}$.
\ENDFOR
\STATE \textbf{return} $\Dhat_\star\leftarrow \argmin_{\Dhat\in \elite_{g+1}} L(\Dhat)${{\color{blue}\# best from $\elite_{g+1}$.}}
\end{algorithmic}
\end{algorithm}

==> icml_ready/algorithms/rap++.tex <==
\newcommand{\qtil}{\tilde{q}}
\begin{algorithm}[t]
\small
\begin{algorithmic}[1]
\caption{Relaxed Projection with Sigmoid Temperature Annealing}\label{alg:rappp}
% \Require   
% Let $\widetilde{\cX}\subseteq [0,1]^d$ be a relaxed data domain with dimension $d$.  
% For any query $q:\cX\rightarrow \{0,1\}^{*}$, let $\qtil: \widetilde{\cX} \times \mathbb{Z}^{+}\rightarrow [0,1]^{*}$ be its continuous \textit{Sigmoid approximation}.
\STATE \textbf{Input: } A set of $m$ sigmoid differentiable queries $\{\tilde{q}^{[\cdot]}_i\}_{i\in [m]}$, a set of $m$ target answers $\hat{a}=\{\hat{a}_i \}_{i\in [m]}$, initial inverse temperature $\sigma_1\in\mathbb{R}^+$, stopping condition $\gamma>0$, and initial dataset $\widehat{D}_1$.


% \State Initialize the loss function $L:\widetilde{\cX}^{n'}\times \mathbb{Z}^{+} \rightarrow[0,1]$:
    % $\Loss_Q(D', \sigma) = \frac{1}{|Q|} \sum_{q\in Q} \|q(D) - \qtil(D', \sigma) \|_2$ \ar{This should be defined in terms of $\hat a$ not $q(D)$ right?} \gv{Yes. will fix it.}

% \State Initialize $\widehat{D}_1 \in \mathbb{R}^{\hat{n}}$.

\FOR{$j=1$ \textbf{ to } $J$}
% \State Compute gradient: $g_t \leftarrow \nabla \Loss_2(D_{t-1}^{'},  \sigma_0 \cdot 2^{k})$ 
% \State Update: $D_{t}^{'} \leftarrow \sparsemax\pp{D_{t-1}^{'} - \alpha \cdot g_t}$ \ar{What is this? I thought we were using the ADAM optimizer?}  \gv{Yes. will fix it.}
% \State SparseMax and clip.
\STATE Set inverse temperature $\sigma_j = \sigma_1 \cdot 2^{j-1}$.
\STATE Define the sigmoid differentiable loss function: 
%
$    \Loss_j(\widehat{D}) = \sum_{i \in [m]} \left( \qtil^{[\sigma_j]}_i(\widehat{D}) - \hat{a}_i \right)^2$
%
\STATE  Starting with $\widehat{D}\leftarrow \widehat{D}_j$.
% update $\widehat{D}$ using 
Run  gradient descent on $L_j({\widehat{D}})$ until    $\|\nabla \Loss_j(\widehat{D})\| \leq \gamma$.
%
Set $\widehat{D}_{j+1} \leftarrow \widehat{D}$.
\ENDFOR
\STATE \textbf{Output} $\widehat{D}_{J+1}$
\end{algorithmic}
\end{algorithm}

==> icml_ready/docs/PrivGA_2.tex <==
\section{Private Genetic Algorithm (\privGA)}\label{sec:GSDdesc}

The generation of high-quality synthetic data through the projection mechanism framework, as described in \cref{sec:projmech}, presents a challenging task that necessitates the solution of an NP-hard optimization problem \citep{HT10}.  Therefore, we propose the \privGA{} algorithm, which solves the projection step in the projection mechanism using a genetic algorithm (GA). 

\subsection{Background on genetic algorithms}
\label{sec:gabackground}

Genetic Algorithms (GA) are a class of optimization algorithms inspired by natural selection and genetic recombination. Introduced by \citet{holland1992genetic}, GAs provide a heuristic search technique to solve complex optimization problems by evolving a population of candidate solutions towards an optimal or near-optimal solution. Crucially, GAs do not require differentiability in the optimization objective.


% GAs offer several benefits for optimization problems; however, GAs do not represent a one-fit-all solution since they require a suitable problem representation (i.e., encoding) and choice of genetic operators to work effectively. For instance, the choice of problem representation can significantly affect the GA's computational efficiency because they typically require multiple iterations and evaluations of the objective function, which can be time-consuming. Furthermore, failure to choose suitable genetic operators can lead to poor candidates or a lack of diversity in the population, making the GA suffer from slow convergence or convergence to the local minimum.






\subsection{Private-GSD}
%

This section presents a genetic algorithm named  Private Genetic Synthetic Data (\GSD), developed specifically for synthetic data generation.
\GSD{} applies two genetic operators known as `mutations' and `crossover' in the GA literature (\citep{such2017deep}). 
In contrast to prior genetic algorithms, the mutation and crossover operator applied by \GSD{} are specifically designed for searching the space of synthetic datasets and optimizing the projection step  described in \cref{sec:projmech}. 
These operators, aimed at generating incremental improvements in synthetic datasets across multiple generations, have been designed for computational efficiency and quick convergence.  We begin by unpacking the core elements and structure of \GSD{} and then dive into the specifics of these genetic operators.

The \GSD{} algorithm operates on a set of statistical queries, denoted as $Q$, and their respective target private responses, $\hat{a}$. It formulates an optimization problem via the objective function $L_{Q,\hat{a}}:\cX^{N'}\rightarrow [0,1]$. A proposed solution to $L_{Q,\hat{a}}$ is a synthetic dataset comprising a user-specified number of rows, $N'$. Thus, \GSD's ultimate objective is to identify a synthetic dataset within $\mathcal{X}^{N'}$ that minimizes $L_{Q,\hat{a}}$. \GSD{} also incorporates other parameters such as the maximum number of generations, $G$, over which it will operate, as well as $\Pmut$ and $\Pcross$, which respectively represent the quantity of proposed solutions generated using mutation and crossover strategies. Lastly, the $E$ parameter determines the number of candidates that will be selected to parent the succeeding generation.

The genetic process unfolds across $G$ generations. For each generation, denoted as $g\in [G]$, \GSD{} maintains a set of elite $E$ candidate solutions, symbolized as $\elite_g$. These represent the optimal $E$ candidate solutions discovered thus far. The initial elite set, $\elite_1$, is chosen at random from the set $\cX^{N'}$. Within each generation, \GSD{} generates $(\Pmut+\Pcross)$ new candidate solutions. These are obtained by introducing minor random variations to the best synthetic data identified up to generation $g$, denoted as $\Dhat^\star_g$. To achieve this, \GSD{} applies a random genetic modification—either mutation or crossover—to $\Dhat^\star_g$, yielding a new synthetic data candidate, $\Dtil$. This process allows for inheriting traits from the elite synthetic dataset and adds diversity, paving the way for potentially superior solutions.

The group of candidate synthetic datasets in generation $g\in[G]$, denoted as $\cP_g$, comprises the $\Pmut+\Pcross$ new candidates and the elite candidates $\elite_g$. \GSD{} assigns a score to each candidate in $\cP_g$ based on their alignment with the objective function $L_{Q, \hat{a}}$. It then ranks all $\Pmut+\Pcross+E$ individual candidates according to their scores, and the top $E$ candidates with the highest fitness scores are chosen as the next generation of elite candidates. This iterative procedure continues until a predetermined termination criterion—such as reaching the maximum number of generations, achieving a satisfactory fitness level, or meeting a predefined condition—is satisfied.


Now, we delve into the specifics of the `mutation' and `crossover' genetic operators, which play a significant role in \GSD's performance. These operators are only applied to the optimal dataset $\Dhat_g^\star$, with the goal of incremental improvements over many generations. Moreover, both operators only modify a single value of $\Dhat_g^\star$. Empirically, we find that having sparse genetic updates is crucial to the success of \GSD, as shown in \cref{tab:parameters} where altering numerous values simultaneously performs noticeably worse.

\paragraph{Mutation.}
The mutation process is a vital part of a genetic algorithm. It introduces minor random perturbations to the most optimal solution to create novel candidate solutions. Controlled by parameter $\Pmut$, the mutation strategy of the \GSD{} algorithm determines the number of candidate synthetic datasets produced in each generation.
During the mutation phase, a row $i \in [N']$ and column $j \in [d]$ are randomly selected. The entry in $\Dhat^\star_g$ corresponding to the selected row $i$ and column $j$ is then replaced by a value sampled uniformly from the range of acceptable values for column $j$. This modified dataset, which differs from $\Dhat^\star_g$ by a single entry,\footnote{While we could adjust the number of mutated rows at each step, our empirical data shows that in our settings, mutating a single row often yields the best performance (see Table 1).} is subsequently added to the pool of candidate solutions.

\paragraph{Crossover.}
Taking inspiration from genetic recombination, the crossover operator merges the parameters of two parent candidates to generate a new offspring. Parameter $\Pcross$ determines the number of candidate synthetic datasets produced in each \GSD{} generation via the crossover strategy.
To sample a new candidate synthetic dataset, the \GSD's crossover operation selects an elite dataset $\Dbar$ from the elite set $\elite_g$. It then combines the parameters of $\Dbar$ with those of the optimal dataset $\Dhat^\star_g$ to produce a new dataset $\Dtil$. This synthetic dataset, differing from $\Dhat^\star_g$ by a single entry, is subsequently added to the candidate solutions population, $\cP_g$.
The crossover operation combines the parameters of $\Dhat^\star_g$ and $\Dbar$ by selecting two rows $i_1, i_2\in[N']$, and a feature $j\in[d]$. The new dataset $\Dtil$ then has its $(i_1, j)$ entry set to match the value of $\Dbar$ at row $i_2$ and feature $j$ (i.e., $\Dtil(i_1, j) = \Dbar(i_2, j)$), while all other entries of $\Dtil$ mirror the corresponding values at $\Dhat^\star_g$.

The crossover operator plays an integral role in improving the convergence rate of \GSD. \cref{fig:convergence} shows the convergence of the \GSD{} algorithm with and without the crossover operator. By encouraging the replication of significant values (with respect to the fitness function) in subsequent generations, \GSD{} with the crossover step converges exponentially faster compared to an algorithm reliant solely on mutations.

\input{Figures/convergence}




\subsection{Privacy And Accuracy}


Below, we state the formal privacy guarantee of \privGA{}, which directly follows from \cref{thm:privacy}.

\begin{corollary}\label{thm:privgaguarantee} 
% For any quer
For any $\rho>0$, dataset $D$, and query set $Q$.
Running \privGA{} (\cref{alg:GSD}) under the adaptive framework satisfies $\rho$-zCDP and  $(\varepsilon, \delta)$-differential privacy for: $\varepsilon = \rho+2\sqrt{\rho\cdot \log(1/\delta)}$.
\end{corollary}
Given that \GSD{} falls within the `projection mechanism' framework proposed by \citet{NKL}, an accuracy analysis can be performed under several assumptions: (1) the input data are discrete, (2) the number of queries is finite, and (3) the optimization step invariably finds the optimal solution of the objective. This kind of analysis assumes access to a perfect optimization oracle and is often referred to as `oracle-efficient' accuracy analysis. It follows a similar approach to previous studies by \citet{gaboardi2014dual, vietri2022private, aydore2021differentially}.

The accuracy statement for \GSD{} is presented in \cref{thm:accurayAppendix}, with a detailed proof provided in the Appendix. Our analysis of \GSD's accuracy is similar to the accuracy analysis of the \RAP{} mechanism \citep{aydore2021differentially}, which also uses the projection mechanism framework and adopts the `oracle-efficient' assumption. However, unlike \RAP, which implements a relaxation step in the data domain to maintain objective differentiability, \GSD{} does not perform such a step. Consequently, our accuracy theorem applies to a general class of queries, whereas the one for \RAP{} is limited to $k$-way marginal queries.
% Since \privGA{} falls under the framework of the projection mechanism of \citet{NKL}, the accuracy analysis can be carried out under the following assumptions: (1) the input data is discrete, (2) the number of queries is finite, and (3) the optimization step is guaranteed to find the optimal solution of the objective. This type of analysis, which assumes access to a perfect optimization oracle, is referred to as "oracle-efficient" accuracy analysis and follows the same style of prior work by \citet{gaboardi2014dual, vietri2022private, aydore2021differentially}.
% The accuracy statement of \GSD{}, is given in \cref{thm:accurayAppendix} in the appendix. Our accuracy analysis of \privGA{} is similar to the accuracy analysis of the \rap{} mechanism \citep{aydore2021differentially}, which also falls under the projection mechanism framework and uses the `oracle-efficient' assumption. However, \privGA{} does not perform a relaxation step in the data domain, unlike the \rap{} mechanism, which performs such a step to maintain the differentiability of the objective. Thus, our accuracy theorem applies to a general class of queries, whereas the one for \rap{} only applies to $k$-way marginal queries.

 % \begin{align*}
     
 % \end{align*}
 % We state the formal guarantee in the Theorem \ref{thm:accurayAppendix} of the appendix. 



% \begin{theorem}\label{thm:accuray}
% For a discrete data domain $\cX$ and any dataset $D\in\cX^N$ with $N$ rows.
% Fix privacy parameters  $\epsilon, \delta>0$, the synthetic dataset size $N'$, and any set of $m$ queries $Q:\cX^*\rightarrow[0,1]^m$. If the one-shot \privGA{} mechanism solves the minimization in the projection step exactly, then 
% the one-shot \privGA{} mechanism outputs a synthetic data $\Dhat$ with
%  average error bounded as
% \begin{align*}
%   \sqrt{\tfrac{1}{m} \| Q(D) - Q(\Dhat) \|_2^2} \leq \\
%    O\pp{
%    \frac{
%     \pp{(\pp{\log(|\cX|) + \log(1/\beta)}\ln(1/\delta)}^{1/4}
%    }{\sqrt{\epsilon\cdot N }}
%    + \frac{\sqrt{\log(m)}   }{\sqrt{N'}}
%    }
% \end{align*}
% \end{theorem}


\begin{remark}
\cref{thm:accurayAppendix} only applies if the underlying optimization algorithm in \cref{alg:GSD} is successful in minimizing the objective in \cref{eq:obj}. Therefore, we accompany the accuracy theorem with empirical evidence that validates the performance of \privGA{} across various datasets (\cref{sec:experiments}; \cref{fig:oneshot_2way_cat}).    
\end{remark}

==> icml_ready/docs/ablation_study.tex <==

\subsection{Ablation study on \GSD{} parameters}\label{sec:ablationstudy}
This sections analyzes different configurations and parameters of \GSD{} and their effect on the final approximation error and runtime. As described in \cref{alg:GSD}, the relevant parameters are the number of generations $G$, the number of mutations $\Pmut$, the number of crossovers $\Pcross$ and the elite size $E$. 

\paragraph{Population size} In this section, we delve into the investigation of parameters $\Pmut$ and $\Pcross$, which guide the generation of candidate synthetic datasets in each iteration. $\Pmut$ and $\Pcross$ represent the count of candidates created via the mutation and crossover strategies respectively. Consequently, these population size parameters correspond to the exploration rate of the \GSD{} method; larger population sizes correspond to a broader array of potential solution candidates at each generation.

Nonetheless, a trade-off exists: larger population sizes incur higher computational costs since \GSD{} to computes the objective function for synthetic dataset candidate. If we denote the quantity of queries as $m$ and the population size as $P$, the computational cost of \GSD{} for each iteration equals $O(P\cdot m)$. Conversely, a reduced population size $P=\Pmut+\Pcross$ may result in slower convergence.

To identify the optimal population size, we conduct an experiment where we adjust the population size and observed its impact on the final error and computation time. We run \GSD{} that outputs a synthetic dataset matching all $2$-way marginal queries on five separate ACS datasets. For each dataset, we initiate \GSD{} with different $\Pmut$ and $\Pcross$ values, maintaining $\Pmut \leq \Pcross$ and keeping other parameters constant. The privacy parameter $\epsilon$ is set to $1$, synthetic data rows to $N'=1000$, and the number of iterations to $G=300,000$ with early stopping.

We present our experimental findings in figures \cref{tab:ablationsummary} and \cref{fig:ablation_runtime}. \cref{tab:ablationsummary} offers insights into the impact of the population size parameters on the final error and runtime. Notably, while the population size parameters only moderately affect the final error, they substantially influence the computational time. Given the stability of the \GSD{} error across different parameters, we next visualized the effect of these parameters on computational time in \cref{fig:ablation_runtime}.

The heatmap in \cref{fig:ablation_runtime} presents total computational time for each parameter combination, where darker hues indicate longer computational times. From this visualization, it is evident that the optimal population size is contingent on the dataset in question. For instance, while the \acscovdata{CA}, \acsempdata{CA}, and \acsmobdata{CA} datasets benefited from larger population sizes, the \acsincdata{CA} and \acstradata{CA} datasets performed better with smaller ones. However, we find that a robust parameter configuration that yields consistently good performance across all tasks was found to be $\Pmut=100$ and $\Pcross=100$.


\input{tables/ablation_summary}

\input{Figures/ablation_runtime}


\paragraph{Genetic Operators Rate}
In this section, we investigate an alternate approach to the \GSD{} algorithm that formulates new candidates by modifying multiple rows of synthetic data via either mutation or crossover operations. Typically, as detailed in \cref{sec:GSDdesc}, the \GSD{} method generates a new candidate synthetic data by adjusting a single entry of the optimal synthetic dataset, $\Dhat_g^\star$. However, by applying genetic operators to multiple rows of $\Dhat_g^\star$, we can potentially accelerate the convergence rate. We hence introduce `mutation rate' and `crossover rate' to denote the number of rows altered in each operation. For example, if the mutation rate is $k$, each candidate solution generated using the mutation strategy will differ from $\Dhat_g^\star$ at $k$ locations.

We conduct an experiment to understand the influence of these rates, in which we vary both the mutation rate and the crossover rate. We run \GSD{} on \acsmobdata{CA} and with all 2-way marginal statistics. The privacy parameter is set to $\epsilon=1$, the maximum number of generations capped at $100,000$, the population size constrained to $100$, and the size of the synthetic data set at $1,000$.

\cref{tab:parameters} depicts the final average error and the corresponding runtime in seconds for each combination of mutation rate and crossover rate. Our findings indicate that both the mutation rate and the crossover rate have a significant impact on error and run time. Interestingly, a mutation rate and crossover rate of $1$ yielded the best average error and run time across all combinations, establishing it as a consistently dependable choice in our experiment. This result emphasizes the importance of selecting these rates carefully for optimal algorithm performance. It further provides evidence that amplifying the level of perturbation in the candidate generation step can destabilize \GSD{} and lead to suboptimal performance.


% In this section we consider a version of \GSD{} that produces new candidates by perturbing multiple rows of synthetic data--using either the mutation or crossover operators.  For example, as described in \cref{sec:GSDdesc}, the \GSD{} method generates a new candidate synthetic data by perturbing a single entry of the optimal synthetic dataset $\Dhat_g^\star$.  However, in principle we could apply the genetic operators to multiple rows of $\Dhat_g^\star$ with the aim of speeding up the rate of convergence.   We refer to the number of rows that get modified--using mutation or crossover--as the 'mutation rate' and 'crossover rate', respectively. For example, if the mutation rate is $k_{mut}$ then each candidate solution generated using the mutation strategy will differ from $\Dhat_g^\star$ in $k_{mut}$ entries.

% Therefore, in this section  we conduct an experiment that varies the the mutation rate and the crossover rate. For this experiment, we used the \acsmobdata{CA} dataset and optimized over the set of 2-way marginal statistics. The privacy parameter was set to $\epsilon=1$, the maximum number of generations was set to $100,000$, the population size was set to $100$, and the synthetic data size was set to $1,000$. The results of the experiment are presented in Table \ref{tab:parameters}. For each mutation rate and crossover rate combination, the table displays the final average error, along with the corresponding run time in seconds in parentheses. Our findings demonstrate that the choice of  mutation rate and crossover rate has a significant impact on both the error and run time. However, we observed that setting the mutation rate and crossover rate to $1$ achieves the best average error and run time, and is therefore a stable choice.

\input{tables/mutation_cross}


==> icml_ready/docs/accuracy.tex <==
\section{Accuracy Analysis of \privGA{}}

Our mechanism inherits similar oracle accuracy guarantees of the (non-adaptive) \rap{} mechanism, which were proven in \citet{aydore2021differentially}. 
% In the adaptive selection framework, the report noisy max (\cref{def:rnm}) and Gaussian mechanism (GM, \cref{def:gaussian}) are both called $K$ times, each with a privacy budget of $\rho' = \rho / (2\cdot K)$. As shown in \cref{def:gaussian} and the work of \citet{durfee2019practical}, each individual call to EM or GM satisfies $(\tfrac{\rho'}{2})$-zCDP. Thus, by the composition properties outlined in \citet{bun2016concentrated}, the combination of $2\cdot K$ $\rho'$-zCDP mechanisms satisfies $\rho$-zCDP.



\begin{theorem}\label{thm:accurayAppendix}
For a discrete data domain $\cX$ and any dataset $D\in\cX^N$ with $N$ rows.
Fix privacy parameters  $\epsilon, \delta>0$, the synthetic dataset size $N'$, and any set of $m$ queries $Q:\cX^*\rightarrow[0,1]^m$. If the one-shot \privGA{} mechanism solves the minimization in the projection step exactly, then 
the one-shot \privGA{} mechanism outputs a synthetic data $\Dhat$ with
 average error bounded as
\begin{align*}
  \sqrt{\tfrac{1}{m} \| Q(D) - Q(\Dhat) \|_2^2} \leq 
   O\pp{
   \frac{
    \pp{(\log(|\cX|/\beta)\ln(1/\delta)}^{1/4}
   }{\sqrt{\epsilon\cdot N }}
   + \frac{\sqrt{\log(m)}}{\sqrt{N'}}
   }
\end{align*}
\end{theorem}
\begin{proof}

We begin with the projection mechanism, which has the following guarantee proven by \citet{NKL}: Given the discrete data domain $\cX$, let $\cX^*$ be the set of datasets of arbitrary size with rows from the domain $\cX$.

The projection mechanism by \citet{NKL}, perturbs the answers of $Q$ on dataset $D$ using the Gaussian mechanism to obtain a vector $\hat{a}$, and then finds a synthetic dataset $\Dhat^*\in \cX^*$ by solving the following objective
% %
\begin{align*}
    \Dhat^* \leftarrow \argmin_{\Dhat \in \cX^*} \|\hat{a} - Q(\Dhat)\|
\end{align*}
% %
with the following accuracy guarantee:
\begin{align*}
    \sqrt{ \tfrac{1}{m}\| Q(D) - Q(\Dhat^*) \|_2^2} \leq \alpha  = O\pp{\frac{\pp{\ln(|\cX| /\beta)\ln(1/\delta)}^{1/4}}{\sqrt{\epsilon\cdot N}}} 
\end{align*}

Next, let $m$ be the number of queries in $Q$. By a simple sampling argument, proven in Lemma 3.7 of \citet{BLR08}, there exists a dataset $\Dhat$ of size $N'$ that satisfies the following:
\begin{align*}
     \|Q(\Dhat) - Q(\Dhat^*)\|_{\infty} \leq \sqrt{\frac{\log(m)}{N'}}
\end{align*}

Finally, suppose that the output of \privGA{} is $\Dhat\in\cX^{N'}$, which is generated by solving an optimization problem exactly as follows:
%
\begin{align*}
    \Dhat \leftarrow \argmin_{\Dhat \in \cX^{N'}} \|\hat{a} - Q(\Dhat)\|
\end{align*}

Then, by triangle inequality:
\begin{align*}
    \sqrt{ \tfrac{1}{m}\| Q(D) - Q(\Dhat) \|_2^2}
    &= \sqrt{ \tfrac{1}{m}\| Q(D) - Q(\Dhat^*) + Q(\Dhat^*) - Q(\Dhat) \|_2^2} \\
    %
    &\leq  \sqrt{ \tfrac{1}{m}\| Q(D) - Q(\Dhat^*) \|_2^2} + \sqrt{ \tfrac{1}{m}\|  Q(\Dhat^*) - Q(\Dhat) \|_2^2} && (\text{Triangle inequality})\\
    &\leq \sqrt{ \tfrac{1}{m}\| Q(D) - Q(\Dhat^*) \|_2^2} + \|Q(\Dhat) - Q(\Dhat^*)\|_{\infty} \\
    %
    &\leq O\pp{\frac{\pp{\ln(|\cX| /\beta)\ln(1/\delta)}^{1/4}}{\sqrt{\epsilon\cdot N}}}  + \sqrt{\frac{\log(m)}{N'}} \\
    % &\leq \sqrt{ \|\tfrac{1}{m} Q(D) - Q(\Dhat^*) \|_2^2}
    % + \|Q(\Dhat) - Q(\Dhat^*)\|_{\infty} 
\end{align*}
\end{proof}


Despite the bounds in \cref{thm:accurayAppendix} matching from the bounds in \citet{aydore2021differentially}, there is no guarantee about the performance \privGA{}'s optimization. Therefore, we empirically show that \privGA{} has comparable performance to \rap{} on matching marginal statistics over many different datasets.
In \cref{fig:oneshot_2way_cat}, we provide results on categorical marginals and with different ACS tasks as defined in Table \ref{tab:acs_data_attributes}. This brief experiment also shows that, like in the adaptive setting, \privGA{} achieves similar performance to \rap{} on differentiable queries in the one-shot setting across many datasets. We use the same hyperparameters used in our adaptive experiments (Table \ref{tab:hyperparameters}), excluding our choices for $T$, which are not applicable in the one-shot setting.



==> icml_ready/docs/algorithm_details.tex <==
\section{Additional algorithm details}

\subsection{Privacy Theorem details}\label{appx:privacyproof}

We first provide additional preliminaries.

The composition property of zCDP differential privacy is given by the following result:

\begin{lemma}[zCDP Composition, \citep{bun2016concentrated}]\label{lemma:comp} Let $\mathcal{A}_1:\mathcal{X}^N\rightarrow R_1$ be $\rho_1$-zCDP. Let $\mathcal{A}_2:\mathcal{X}^n\times R_1 \rightarrow R_2$ be such that $\mathcal{A}_2(\cdot,r)$ is $\rho_2$-zCDP for every $r\in R_1$. Then the algorithm $\mathcal{A}(D)$ that computes $r_1=\mathcal{A}_1(D), r_2=\mathcal{A}_2(D,r_1)$ and outputs $(r_1,r_2)$ satisfies  $(\rho_1+\rho_2)$-zCDP.
\end{lemma}

Any mechanism that satisfies zCDP also satisfies DP.
\begin{theorem}[zCDP to DP]
    If $M$ provides $\rho$-zCDP, then $M$ is $(\rho+2\sqrt{\rho\log(1/\delta)},\delta)$-differentially private for any $\delta>0$.
\end{theorem}



We will use the post-procession properties of zCDP in our analysis. Essentially, there is no loss of privacy  when doing an operation on the output of a zCDP mechanism. 
\begin{lemma}[Post-processing]\label{lemma:post} Let $M:\mathcal{X}^N\rightarrow\mathcal{Y}$ and $f:\mathcal{Y}\rightarrow\mathcal{Z}$ be randomized algorithms. Suppose $M$ satisfies $\rho$-zCDP. Define $M':\mathcal{X}^N\rightarrow\mathcal{Z}$ by $M'(X)=f(M(X))$. Then $M'$ satisfies $\rho$-zCDP.
\end{lemma}

% Finally, a related notion of privacy is called concentrated differential privacy (zCDP) \citep{DworkR16,BunS16}, which enables cleaner composition analyses for privacy. 
%
%
%%%%%%%%%%%%%%%%%
%% Def 
%%%%%%%%%%%%%%%%%
% \begin{definition}[Concentrated DP,  \citep{DworkR16,BunS16}]\label{def:zCDP}
%  A randomized mechanism $\cM:\cX^n \rightarrow \cR$ is ${\rho}$-CDP, if for all neighboring datasets $P, P'$ (i.e., differing on a single person), and for all $\alpha\in(1,\infty)$,
%  \begin{align*}
%      \rendiver{\alpha}{\cM(P)\parallel\cM(P')} \leq \rho\alpha
%  \end{align*}
%  where $\rendiver{\alpha}{\cM(P)\parallel\cM(P')}$ is the R\'{e}nyi divergence between the distributions $\cM(P)$ and $\cM(P')$.
% \end{definition}


% Our synthetic data algorithm uses two  primitive  functions for privately selecting and answering low sensitive queries the exponential mechanism and the Gaussian mechanism. 
We use the Gaussian mechanism for privately estimating a subset of statistical queries, which perturbs the statistics with Gaussian noise scaled by the queries' sensitivity. A query of the data has low sensitivity if a small change in the data produces a small change in the output. Formally, let $\Delta(Q)$ denote the $\ell_2$-sensitivity  of vector-valued query $Q$, where $ \Delta(Q) = \max_{\text{neighboring } D,D'} \| Q(D) - Q(D')\|_2$. 

\begin{definition}[Gaussian Mechanism]\label{def:gaussian}
Let $Q:\cX^N \rightarrow \mathbb{R}^m$ be a function of the dataset. The Gaussian mechanism on input $D\in \cX^N$ , $Q$, and $\rho>0$, outputs $Q(D) + \cN\pp{0, \tfrac{\Delta(Q)^2}{2\rho}\cdot \mathbb{I}}$. 
%
And the Gaussian mechanism satisfies $\rho$-zCDP \citep{bun2016concentrated}.
\end{definition}


We will also use the private selection algorithm \emph{report noisy max} \citep{durfee2019practical} with Gumbel perturbation noise, whose output distribution is identical to that of the exponential mechanism \citep{mcsherry2007mechanism}.

\begin{definition}[Exponential Mechanism]\label{def:exponential}
Given some dataset $D\in \cX^*$, arbitrary range $\mathcal{R}$, and score function $S: \mathcal{X}^*\times\mathcal{R}\rightarrow\mathbb{R}$, the exponential mechanism $\mathcal{M}_E(D,S,\mathcal{R},\varepsilon)$ selects and outputs an element $r\in\mathcal{R}$ with probability proportional to $\exp\pp{\frac{\varepsilon S(D,r)}{2\Delta_S}},$ where $\Delta_S$
 is the sensitivity of $S$.
 \end{definition}

\begin{definition}[Report Noisy Max With Gumbel Noise]\label{def:rnm} The Report Noisy Max mechanism $RNM(D,q,a,\rho)$ takes as input a dataset $D\in\mathcal{X}^N$, a vector of $m$ statistical queries $q$, a vector of $m$ query answers $a$, and a zCDP parameter $\rho$. It outputs the index of the query with highest noisy error estimate, $i^*=\arg\max_{i\in[m]}(|q_i(D)-a_i|+Z_i)$ where each $Z_i\sim{\rm Gumbel}(1/\sqrt{2\rho}N)$. $RNM(\cdot,q,a,\rho)$ satisfies $\rho$-zCDP.
\end{definition}

We now provide a proof sketch to \cref{thm:privacy}.

\begin{proof}
In the adaptive selection framework, the report noisy max (RNM, Definition \ref{def:rnm}) and Gaussian mechanism (GM, Definition \ref{def:gaussian}) are both called $K\cdot S$ times, each with a privacy budget of $\rho' = \rho / (2\cdot K\cdot S)$. As shown in Definition \ref{def:gaussian} and the work of \citet{durfee2019practical}, each individual call to RNM or GM satisfies $({\rho'})$-zCDP. Thus, by the composition properties outlined in \citet{bun2016concentrated}(see Lemma \ref{lemma:comp} ), the combination of $2\cdot K\cdot S$ $\rho'$-zCDP mechanisms satisfies $\rho$-zCDP.\end{proof}

\subsection{Adaptive Selection}\label{appx:adaptive}

We present the Adaptive Selection framework in Algorithm \ref{alg:adaptive}, and also provide its privacy proof below.

\input{icml/algorithms/adaptive_framework.tex}

% We provide a proof sketch to Theorem \ref{thm:privacy} below.
% \begin{proof}
% \gvcomment{complete}
% \end{proof}

\subsection{\rappp{} and its limitations}\label{appx:rappp}
\input{icml/docs/rap++_v2.tex}

\subsection{Modifications to \rp{} / \gn{}}\label{appx:rapgem}

Suppose we have a data domain $\gX = \gX_1 \times \ldots \times \gX_d$ contains $d$ discrete attributes. Then both \rp{} and \gn{} (both the one-shot and adaptive variants) model such features as a mixture of $K$ product distributions over attributes $\gX_i$ (and possible values they can take on). We denote each product distribution as $P_i = \prod_{j=1}^d P_{ij}$, where $P_{ij}$ is a distribution over the discrete values of $\gX_j$. The difference between \rp{} and \gn{} then is how each distribution $P_{ij}$ is parametrized. In \rp, the parameters $\theta$ are exactly the values $P_{ij}$. Meanwhile, \gn{} instead outputs the values $P_{ij}$ using a neural network $F_{\theta}$, which takes in as input Gaussian noise $\mathbf{z} \sim \mathcal{N}\left(0, I_K \right)$.

In either case, query answers for $k$-way categorical queries can be calculated as a product over various columns in $P_i$. For example (relaxing notation), suppose $P_{i, \textrm{COLOR}=\textrm{red}}$ and $P_{i, \textrm{SHAPE}=\textrm{circle}}$ correspond to the probabilities that attributes $\textrm{COLOR}=\textrm{red}$ and $\textrm{SHAPE}=\textrm{circle}$. Then the 2-way marginal query counting the proportion of samples that are red circles can be written down as the product query $\frac{1}{K} \sum_{i=1}^{K} P_{i, \textrm{COLOR}=\textrm{red}} \times P_{i, \textrm{SHAPE}=\textrm{circle}}$.

Now suppose we have some numerical column that has been discretized into bins. Then a $k$-way range marginal query can be simple written down as a sum of product queries. For example, suppose we have an attribute QUANTITY that has been discretized into bins of size 10. Then the $2$-way range query for proportion of samples that are red and have quantity between 1 and 20 can be written down as $\frac{1}{K} \sum_{i=1}^{K} P_{i, \textrm{COLOR}=\textrm{red}} \times \left[ P_{i, \textrm{QTY}=\textrm{1-10}} + P_{i, \textrm{QTY}=\textrm{11-20}} \right]$. Therefore, we are able to still optimize over such queries, since they are simply sums over (differentiable) product queries that the algorithms were originally designed for.

Finally, while \citet{liu2021iterative} and \citet{aydore2021differentially} propose different optimization strategies for their algorithms at each round, we introduce a simpler update procedure that we find performs well across our experiments. We present this procedure in Algorithm \ref{alg:rapgem_update}.

\begin{algorithm}[!tbh]
\caption{\rp{} / \gn{} Update}
\label{alg:rapgem_update}
\begin{algorithmic}
\STATE {\bfseries Input:} $\rp{}/\gn{}_\theta$, queries (sampled via the exponential mechanism) $Q = \anglebrack{q_1, \ldots, q_t}$, noisy answers (measured via the Gaussian mechanism) $A = \anglebrack{a_1, \ldots, a_t}$, max iterations $M$, batch size $B$ \\

\FOR{$m = 1 $ {\bfseries to} $2M$}
    \STATE Let synthetic answers $\hat{A} = \rap{}/\gem{}_\theta(Q)$
    \STATE Let errors $P = |A - \hat{A}|$
    \IF{${m \bmod 2} = 0$}
        \STATE Sample a set of query indices $S$ of size $B$ uniformly
    \ELSE
        \STATE Sample a set of query indices $S$ of size $B$ proportional to errors $P$
    \ENDIF
    \STATE Update $\theta$ via stochastic gradient decent according to $\norm{P_S}_1$
\ENDFOR
\end{algorithmic}
\end{algorithm}

==> icml_ready/docs/conclusion.tex <==
\section{Conclusion}
We present \privGA{}, a versatile genetic algorithm that can generate synthetic data to approximate a wide range of statistical queries, regardless of their differentiability. 
% \privGA{} uses a novel crossover and mutation routine crucial to its success. 
Our empirical evaluation of the \privGA{} mechanism on mixed-type data demonstrates that \privGA{} outperforms the state-of-the-art method, \rappp{}, on non-differentiable queries and matches first-order optimization methods for differentiable ones. Overall, genetic algorithms present a promising solution for generating mixed-type synthetic data, and we hope our work will inspire further exploration of such approaches in privacy research.The \GSD{} source code is publicly available at \url{https://github.com/giusevtr/private_gsd}.

==> icml_ready/docs/dp.tex <==
\section{Additional preliminaries}
\begin{definition}[Exponential Mechanism]\label{def:exponential}
Given some dataset $D\in \cX^*$, arbitrary range $\mathcal{R}$, and score function $S: \mathcal{X}^*\times\mathcal{R}\rightarrow\mathbb{R}$, the exponential mechanism $\mathcal{M}_E(D,S,\mathcal{R},\varepsilon)$ selects and outputs an element $r\in\mathcal{R}$ with probability proportional to $\exp\pp{\frac{\varepsilon S(D,r)}{2\Delta_S}},$ where $\Delta_S$
 is the sensitivity of $S$.
 \end{definition}
 


==> icml_ready/docs/experiment_details.tex <==
\section{Additional experiment details}

In this section we include additional details about our experiments, including information about datasets, queries, and hyperparameters.

%%%%% data attributes %%%%%
\paragraph{Data.} In Table \ref{tab:acs_data_attributes}, we list all attributes for each ACS task that are used in empirical results presented in either the main paper or this appendix.

\begin{table}[!htb]
\centering
\caption{We list the ACS data attributes used in our experiments.}
\label{tab:acs_data_attributes}
\begin{tabular}{l | l| l}
\toprule
Dataset & Categorical Attributes & Numeric Attributes \\
\midrule
\multirow{2}{*}{\acsmob} & MIL, DREM, CIT, DIS, COW, MAR, SCHL, MIG, NATIVITY & JWMNP, PINCP \\
& ANC, DEAR, DEYE, SEX, ESR, GCL, RAC1P, RELP & WKHP, AGEP \\
\midrule
% \multirow{2}{*}{\acsreal} & \multirow{2}{*}{ESR, PINCP, PUBCOV} & AGEP, POVPIP, JWRIP, SEMP \\
% & & WAGP, WKHP, INTP, JWMNP \\
% \midrule
\multirow{1}{*}{\acsemp} & COW, OCCP, SCHL, MAR, SEX, PINCP, RAC1P, RELP, POBP & AGEP \\
\midrule
\multirow{2}{*}{\acscov} & MIL, FER, DREM, CIT, DIS, MAR, SCHL, PUBCOV & \multirow{2}{*}{PINCP, AGEP} \\
& MIG, NATIVITY, ANC, DEYE, SEX, ESR, RAC1P, DEAR, ESP & \\
\midrule
\multirow{1}{*}{\acsinc} & COW, OCCP, SCHL, MAR, SEX, PINCP, RAC1P, RELP, POBP & WKHP, AGEP \\
\midrule
\multirow{2}{*}{\acstra} & JWMNP, PUMA, CIT, DIS, OCCP, SCHL, JWTR, MAR & \multirow{2}{*}{AGEP, POVPIP} \\
& MIG, SEX, RAC1P, POWPUMA, RELP, ESP & \\
\midrule
\multirow{4}{*}{\acsmultitask} & OCCP, MIG, CIT, ESP, ANC, PUMA, FER, DEAR, DEYE & INTP, WAGP \\
&  ESR, FOCCP, JWTR, WAOB, JWMNP\_bin, DREM, GCL & SEMP, POVPIP \\ & MIL, SCHL, RELP, MAR, NATIVITY, POWPUMA & WKHP, JWRIP \\ & RAC1P, DIS, COW, PUBCOV, SEX, PINCP & AGEP \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!htb]
\centering
\caption{Number of workloads for categorical and range marginal queries used in our experiments.}
\label{tab:workloads}
\begin{tabular}{l | c c c c c }
    \toprule
    & mobility & coverage & employment & income & travel \\
    \midrule
    $2$-way Cat. Marginals & 136 & 136 & 120 & 36 & 91 \\
    $3$-way Cat. Marginals & 680 & 680 & 560 & 84 & 364 \\
    $2$-way BT Marginals & 68 & 34 & 16 & 18 & 28 \\
    % $3$-way BT Marginals & - & 84 & - & - & - & - \\
    \bottomrule
\end{tabular}
\end{table}





\iffalse

%%%%% Runtime %%%%%
\paragraph{Runtime.} In Table \ref{tab:runtime}, we compare the runtime of \privGA{} and our 3 baselines on categorical experiments with $3$-way categorical marginal queries.

In terms of runtime of \privGA, The mutation and crossover steps are computationally straightforward. Therefore, the primary computational bottleneck is the evaluation of the objective score of each population in the dataset. In order to calculate the score of each dataset, we must evaluate the statistics on all synthetic datasets in a population of size $N$. Thus, the algorithm's runtime depends primarily on the speed of evaluating statistical queries. With our choice of hyperparameters, our algorithm attains reasonable runtime compared to the baselines, although our proposed update procedure for \rap{} and \gem{} still runs comparatively fast. 

Experiments for \privGA{} were run on a single GPU of NVIDIA TITAN V. All experiments for \rap{}, \gem{}, and \pgmem{} were run using a desktop computer with NVIDIA GeForce GTX 1080 Ti graphics card. Our implementation for \rap{} and \gem{} is derived from \url{https://github.com/terranceliu/dp-query-release}, while our implementation for \pgmem{} uses \url{https://github.com/ryan112358/private-pgm}.



\begin{table}[!htb]
\caption{We compare the runtime of all algorithms across various choices of $T$ when run on \acsmob, where $Q$ is all $3$-way categorical marginals and $\varepsilon = 1$. The runtime is measured in seconds.}
\label{tab:runtime}
\centering
\begin{tabular}{l | c c c c }
    \toprule
    & $T=25$ & $T=50$ & $T=75$ & $T=100$  \\
    \midrule
    \privGA & 860 & 1744 & 3231 & 5316  \\
    \rap  & 70 & 137 & 204 & 274 \\
    \gem  & 71 & 142 & 211 & 280 \\
    \pgmem & 397 & 2633 & 5693 & 8452 \\
    \bottomrule
\end{tabular}
\end{table}

\fi



%%%%% hyperparameters %%%%%
\paragraph{Hyperparameters.} In Table \ref{tab:hyperparameters}, we list the hyperparameters used for our algorithms.

\input{tables/hyperparameters}

% \section{Additional results}

% In Tables \ref{tab:oneshot} we provide additional results on categorical marginals and with different ACS tasks as defined in Table \ref{tab:acs_data_attributes}. This brief experiment also shows that like in the adaptive setting, \privGA{} achieves similar performance to \rap{} on differentiable queries in the one-shot setting across many datasets. We use the same hyperparameters used in our adaptive experiments (Table \ref{tab:hyperparameters}), excluding ours choices for $T$, which are not applicable in the one shot setting.

% \begin{table}[!htb]
% \centering
% \caption{Max and average error of one-shot mechanism ($\varepsilon=1$) with $2$-way categorical marginal queries for all ACS tasks. We also list the number of workloads for each task.}
% \label{tab:oneshot}
%     \begin{tabular}{l c | c c | c c }
%     \toprule
%     & & \multicolumn{2}{c}{Max} & \multicolumn{2}{c}{Average}\\
%     & \# workloads & \rap{} & \privGA{} & \rap{} & \privGA{} \\
%     \midrule
%     \acsmob & 136 & 0.003005 & 0.004519 & 0.0004527 & 0.0005146 \\ 
%     \acsinc & 36 & 0.003048 & 0.001416 & 0.0000206 & 0.0000253 \\ 
%     \acsemp & 120 & 0.001288 & 0.001497 & 0.0001768 & 0.0001862 \\
%     \acstra & 91 & 0.004898 & 0.004251 & 0.0000318 & 0.00003724 \\ 
%     \acscov & 136 & 0.002156 & 0.002437 & 0.0003193 & 0.00034858 \\
%     \bottomrule
% \end{tabular}
% \end{table}



\subsection{Early Stop} \label{sec:earlystopAppendix}
In all experiments, \GSD{} operates over a maximum of $G$ generations. However, we employ an early-stop rule if the algorithm has reached a satisfactory level of convergence in optimizing its objective. This not only aids in achieving the desired result more swiftly but also conserves computational resources.

To determine the convergence of the algorithm, we utilize a time-window approach. We define a window size, $w$ (where $w < G$), for assessing the early-stop condition. The algorithm is halted if the percent change in loss between the current generation, $g$, and the generation $g-w$ is less than a predetermined threshold. In all cases in this paper, the threshold is set to $0.0001$. If the change in loss between the two generations within the window falls below this threshold, the algorithm is halted prematurely. This allows us to conclude that the algorithm has sufficiently converged and further iterations would not significantly contribute to the optimization of the objective. Additionally, the size of the time-window, $w$, is set to match the size of the synthetic dataset, $N'$. The proportionality of the window size to the dataset size ensures that our early-stop condition is adapted to the scale of the problem at hand.

==> icml_ready/docs/experiments.tex <==


\section{Experiments}\label{sec:experiments}


We conduct experiments to compare the performance of \privGA{} against baseline mechanisms in various settings. In particular, we evaluate the performance of various synthetic data mechanisms on mixed-typed data, which contain both categorical and numerical attributes. Our results demonstrate that in this setting, \privGA{} is strong mechanism in approximating various types of statistical queries, outperforming \rappp{}, the state-of-the-art method for generating synthetic data with real-valued columns. In addition, we demonstrate that \privGA{} achieves performance comparable to that of mechanisms specifically designed for---and restricted to---handling differentiable query functions for discrete data.

% In this study, we conduct experiments to compare the performance of \privGA{} against different baseline mechanisms in various settings. The primary focus of our evaluation is to assess the ability of the algorithm to approximate categorical features using publicly available data from the US census.

% The results of the categorical data type experiments indicate that \privGA{} exhibits comparable performance to mechanisms specifically designed for handling discrete data. However, the main objective of this section is to evaluate the performance of various synthetic data mechanisms when the input data contains numeric or real-valued features.

% We systematically varied the settings of the experiments, such as the type and size of the dataset, and the level of privacy required, to evaluate the performance of the algorithm. The main performance metric is the max error over the statistical queries. The results of the experiments were analyzed using various visualizations.

% The results of our experiments demonstrate that \privGA{} is a promising mechanism for approximating various types of statistical queries and mixed-type datasets. We finalize the section by showing that using the synthetic data as training data for machine learning models, and show that the models trained on synthetic data achieve test accuracy comparable to models trained on real data.  

\subsection{Data}\label{sec:data}

For our empirical evaluation, we use datasets derived from the Folktables package \citep{ding2021retiring}, which defines datasets using samples from the American Community Survey (ACS). The ACS is collected annually by the U.S. Census Bureau to capture the demographic and economic characteristics of individuals and households in the country. In particular, Folktables provides an array of classification tasks, which are defined by a target column, a collection of mixed-type features, and some filter that specifies what samples to include.\footnote{For example, a task can be defined to include only rows with individuals over the age of 18.}
%
\iffalse
While our work is primarily focused on outputting private synthetic data that contain real-valued attributes, the tasks predefined by \citet{ding2021retiring} are dominated by categorical features.\footnote{Each has has at most 4 real-valued features.}
%
Therefore, we focus our attention to the mobility task, which contains the most real-valued features (4 in total) among all tasks. We refer to this data domain as \acsmob. Moreover, to evaluate on a dataset that is comprised primarily of real-valued attributes, we construct a new data domain called \acsreal, which contains 8 real-valued and 3 categorical attributes.
\fi
%
The experiments in this section use samples from California and the five ACS tasks listed in \cref{tab:data_stats}. Finally, each dataset is normalized by linearly scaling real-valued columns to lie in $[0,1]$.

% We use a collection of datasets from the U.S. Census introduced in \citep{ding2021retiring}. These datasets include five pre-defined prediction tasks, each with a target column and a set of mix-type features. Each task consists of a subset of columns from the American Community Survey (ACS) corpus. The ACS is collected annually by the U.S. Census Bureau to capture the demographic and economic characteristics of individuals and households in the country.

% The ACS tasks defined originally in \citep{ding2021retiring} mostly contain categorical features (each has between 1 to 4 numeric features). Therefore, we use the original ACS tasks for our first experimental phase, where we test the synthetic data algorithms for categorical data and marginal queries. Next, we introduce a dataset of real-valued, continuous columns derived from the American Community Survey (ACS) for the second experiment phase. Specifically, we use the Folktables \citep{ding2021retiring} package to extract all the ACS real-valued columns (see Table \ref{tab:data_attributes}). We denote our newly constructed data domain as \acsreal and conduct experiments using records from various states. The \acsreal{} task contains three categorical features and nine real-valued features. We use data from California and New York, which contain 144725 and 58041 rows. We normalize the data by linearly scaling the values of each column to lie in $[0,1]$

\begin{table}[ht]
\centering
\begin{tabular}{l | c c c }
    \toprule
    Dataset & N & \# Real & \# Cat. \\
    \midrule
    \acsmobdata{CA} & 64263 & 4 & 17 \\
    \acsempdata{CA} & 303054 & 1 & 16 \\
    \acsincdata{CA} & 156532 & 2 & 9 \\
    \acscovdata{CA} & 110843 & 2 & 17 \\
    \acstradata{CA} & 138006 & 2 & 14 \\
    \bottomrule
\end{tabular}
\caption{For each dataset, we list the number of rows $N$, as well as the number of real and categorical features.}
\label{tab:data_stats}
\end{table}

% Mobility - 3-way marginals, 84 workloads, 9415563 queries
% Mobility - 2-way range, 68 workloads, 25296 queries
% Real - 3-way range (2 num), 84 workloads, 1076320 queries

% Mobility: Domain(DEYE: 2, COW: 10, ESR: 6, RELP: 17, ANC: 5, MIG: 2, SEX: 2, MIL: 4, DREM: 2, NATIVITY: 2, DEAR: 2, RAC1P: 9, MAR: 5, GCL: 3, CIT: 5, DIS: 2, SCHL: 24, PINCP: 32, AGEP: 32, WKHP: 32, JWMNP: 32)
% Real: Domain(ESR: 6, PINCP: 2, PUBCOV: 2, AGEP: 32, POVPIP: 32, JWRIP: 32, SEMP: 32, WAGP: 32, WKHP: 32, INTP: 32, JWMNP: 32)


\subsection{Statistical queries} 

Statistical queries are essential for data analysis and decision-making, as they allow us to extract meaningful insights from large and complex datasets. In this section, we describe how we define the four sets of statistical queries that we use in our experiments. We summarize these queries in \cref{tab:queries}  and describe them in more detail below:

%

\paragraph{Random Prefixes:} 
The first query class we consider is a random set of $50,000$ prefix queries, as in \cref{def:prefix}.
To generate a random prefix query, we randomly sample a categorical column $c$ and two numeric columns $a, b$. Then, uniformly sample a target value $v$ for column $c$ and the two thresholds $\tau_a,\tau_b\in[0,1]$ for the numeric columns $a$ and $b$, respectively. The corresponding prefix query $q_{\text{prefix}}$ is defined as follows:
%
\begin{align}
    q_{\text{prefix}}(x) = \mathbb{I}\{x_c = v \text{ and } x_{a}< \tau_a \text{ and } x_b < \tau_b\}
\end{align}
%
% To create the query set for the prefix class, we sample $50,000$ random prefix by repeating the process from above. 

\paragraph{Random Halfspaces}
Next, we sample $m=200,000$ random halfspace queries as in \cref{def:halfspace}. Each sample is generated as follows:  
Let $d'$ be the dimension of the one-hot encoding of $\cX$.
First, sample a random vector ${\theta}\in \mathbb{R}^{d'}$, where the value of each coordinate $i\in [d']$ is an i.i.d sample drawn from the normal distribution with variance $\tfrac{1}{d}$ (i.e., ${\theta}_i \sim \cN(0, \tfrac{1}{d})$). Then, sample a threshold value $\tau$ from the standard normal distribution, i.e., $\tau\sim \cN(0,1)$. Finally, add the query  $q_{\theta, \tau}$ to the set $Q_{\text{HS}}$.



% The $\ell_2$ sensitivity of a single halfspace query is $\Delta(q_{\theta, \tau})=1$.




\paragraph{$k$-way Categorical Marginals:}
Using categorical columns only, we select all $2$-way marginals in the one-shot setting and all $3$-way marginal queries in the  adaptive setting. Since the query answers in a workload sum up to $1$, each workload has $\ell_2$-sensitivity $\Delta_2 = \sqrt{2}$.

\paragraph{$k$-way Binary-Tree Marginals:}
In this work we introduce a class of queries, which we coined \emph{Binary-Tree Marginals}. The Binary-Tree marginals consists of a collection of range queries, as in \cref{def:range_marginals}) defined over various levels. We construct range queries using one categorical attribute and $k-1$ real-valued attribute. Recall that real-valued features lie in the domain $[0,1]$. Thus, we define a workload of range queries by the set of intervals of width $\frac{1}{2^j}$ for $j \in \{1, 2, \ldots, 5\}$.
Now consider the set
\begin{align*}
    I = \{ \pp{\tfrac{i}{2^j}, \tfrac{i + 1}{2^j}}| 0\leq i< 2^j , j \in \{1, 2, \ldots, 5\} \}
\end{align*}
%
Using the same notation from definition \ref{def:range_marginals}, for real-valued feature $c$, the corresponding range workload  $Q_{c, I} =\{ q_{c, (a,b)}\}_{(a, b) \in I}$ is the set of range queries defined by intervals in $I$. This construction simulates the binary mechanism of \citet{chan2011private} for releasing sum prefixes privately.

Note that a single data point only appears in one interval of size $1/2^j$ for each $0< j \leq 5$. Therefore, adding a new data point only affects the counts of $5$ range queries in the workload $Q_{c, I}$.
By the same logic, replacing a data point affects $10$ range queries in  $Q_{c, I}$. Therefore, we say that the workload  $Q_{c,I}$ has $\ell_2$-sensitivity $\sqrt{10}$.
% \begin{align}
%     % 
% \end{align}

% is a vector where each coordinate is the answer of range query $ q_{c, (a, b)}(x)$ for an interval in $(a,b)\in I$
% \begin{align*}
%    Q_{c, I}(x) = \pp{ q_{(a, b)}(x),  } _{(a, b)\in I}
% \end{align*}

\begin{table}[!htb]
\centering
\begin{tabular}{l |c c}
    \toprule
    Query class & Query set size & $\Delta_2$ \\
    \midrule
    2-way Categorical & ${\binom{d}{2}}$ & $\sqrt{2}$ \\  
    \midrule 
    3-way Categorical & ${\binom{d}{3}}$ & $\sqrt{2}$ \\  
    \midrule 
    2-way Binary-Tree & $d_{cat} \cdot d_{num}$ & $\sqrt{10}$ \\  
    \midrule
    % 3-way Binary-Tree & $d_{cat} \cdot {\binom{d_{num}}{2}}$ & $\sqrt{10}$ \\  
    % \midrule
    Random Prefix & $200000$  & $1$ \\  
    \midrule
    Random Halfspaces & $200000$  & $1$ \\  
    \bottomrule
\end{tabular}
\caption{The total number of queries depends on the input data total number of features, which we denote by $d$ and  the number of categorical and numerical features, $d_{cat}$ and $d_{num}$ respectively. In addition, we list the $\ell_2$-sensitivity $\Delta_2$ of each query class (the sensitivity for categorical and binary-tree marginals is written with respect to an entire workload of queries). In our experiments, the number of categorical attributes binary-tree marginals is set to $1$.}
\label{tab:queries}
\end{table}

% \subsection{Evaluation metrics} 
% %
% We evaluate the performance of synthetic data algorithms by measuring the approximation error of each statistic. We use two metrics to evaluate the performance: the average and maximum approximation errors. Furthermore, we report the approximation error over various privacy levels, determined by the privacy parameter $\varepsilon$, to examine the trade-off between privacy and accuracy for each method.
% by varying the privacy parameter, allowing us to determine the optimal privacy level for a given application.

\subsection{Baselines}

\paragraph{\rappp.}

We compare our mechanism \privGA{} against the mechanism \rappp{} by \citet{vietri2022private}. The \rappp{} algorithm uses a first-order optimization algorithm called {\em Sigmoid Temperature Annealing} (pseudocode can be found in Appendix \ref{appx:rappp}). Recall that \rappp{} replaces the prefix queries with a differentiable surrogate query by using Sigmoid functions. To control the degree by which the Sigmoid functions approximate the prefix functions, it uses the {\em inverse Sigmoid temperature parameter} $\invtemp$. The algorithm starts with a small inverse temperature $\invtemp$ and runs a gradient-based minimizer on the induced optimization objective with learning rate \LR, and then repeats the process for a different choice of inverse temperature. 

% The inverse temperature parameters used in our experiments are $\invtemp\in \{2, 4, 8, 16, 32, 64, 128, 256, 512, 1024, 2048\}$. 

% \rappp{} is also sensitive to its learning rate (\LR) parameter, which controls the speed of the gradient-descent algorithm. Thus, we run \rappp{} multiple times, each time with a different learning rate $\LR \in \{0.0005, 0.001, 0.002, 0.005, 0.01\}$. 

% We run \rappp{} for 5000 iterations and \privGA{} for 3000 iterations, and both get synthetic data of size 100. For \rappp{} baseline, each time we try all lr values in $[0.0005, 0.001, 0.002, 0.005, 0.01]$ and choose the synthetic data that get lowest in-sample error to be the final result. For \privGA{}, we set the population size $N$ to be 8000.
% \gv{Add more} \jt{not sure what to add}\gv{This is good for now.}

\paragraph{\rp{} / \gn{}.}

We also compare our method to \rap\footnote{We use the softmax variant proposed by \citet{liu2021iterative}, which has been shown to perform much better that the versions originally proposed in \citet{aydore2021differentially}. We note in \citet{vietri2022private}, references to \rap{} also refer to this softmax version.} \citep{liu2021iterative, aydore2021differentially} and \gem{} \citep{liu2021iterative}, two gradient-based optimization algorithms for generating private synthetic data that belong to discrete data domains. In both algorithms, datasets are modeled as mixtures of product distributions $P$ over the attributes, with the main difference being the way in which such distributions are parameterized---in \gem{}, $P$ is parameterized by a neural network that given Gaussian noise, outputs a set of product distributions, while in \rap{}, $P$ is parameterized directly by the probabilities defining the distribution for each attribute. Because both methods are limited to discrete data, real-valued columns must be discretized first. Consequently, \rap{} and \gem{} can only optimize over $k$-way categorical and binary-tree marginals. In \cref{appx:rapgem}, we show how we modify these methods to optimize over binary-tree queries and also provide additional details about their optimization procedures. Going forward, we denote the one-shot version of \rap{} and \gem{} by \rp{} (RelaxedProjection) and \gn{} (GenerativeNetwork) respectively.

\paragraph{\pgmem.}

Lastly, we compare to a graphical model approach, \pgm{} \citep{mckenna2019graphical}, which like \rap{} and \gem{}, is also limited to discrete data domains. However, \pgm{} instead models data distributions using probabilistic graphical models. We run an adaptive version of \pgm{} that also uses the exponential mechanism. We refer to this variant as \pgmem{} and run it on $k$-way categorical marginals.
% , and compare it against \privGA{}, \rap{}, and \gem{} on $k$-way marginal queries.


% \subsection{Additional details on \privGA{}.} 
% %
% For the experiments in this section, we run the \privGA{} algorithm with a population size of $N=10000$. In addition, the elite set parameter is set to $T=2$. These values give consistent results for our experiments. However, at the cost of longer runtime, increasing $G$ and $N$ should improve the accuracy of the \privGA{} since it provides the algorithm with more rounds to find an accurate synthetic dataset.

% The remaining parameter is the mutation strength $\sigma$, which controls the magnitude of off-spring mutations from one generation to the next. For instance, setting mutation strength $\sigma=0$ equates to no modifications and would not produce any diversity for future generations. On the other hand, a higher value of $\sigma$ corresponds to more aggressive mutations, which could make the system unstable and not converge. In our work, we found that $\sigma=0.1$ provides a good trade-off between diversity and stability of each generation. However, in the following section, we compare the performance of \privGA{} over different choices of mutation strength $\sigma$ and demonstrate that any value between $0.1$ and $0.5$ also provides good performance. 




% \paragraph{Hyperparameter Sensitivity Evaluation.} 
% %
% How difficult it is to choose the correct parameter combination for a particular mechanism is paramount to its practicality. We say that a mechanism is sensitive to the choice of hyperparameters if it only works well under a narrow set of values. Therefore, in this section, we evaluate how sensitive \privGA{} and \rappp{} are to the choice of the mutation strength $\sigma$ and and learning rate \LR{} parameters respectively. We evaluate both algorithms over different choices of hyperparameters to approximate the set of prefix queries on the \acsreal{} dataset for New York. Moreover, we evaluate over two privacy levels $\varepsilon \in \{0.1, 1\}$. In Table \ref{tab:hyperparameters}, we observe that \rappp{} is very sensitive to the choice of \LR, only working for $\LR=0.02$. \privGA{}, however, is less sensitive to the choice of mutation strength $\sigma$. Setting $\sigma=0.1$ is the best value we found, but any value of $\sigma \in [0.05, 0.5]$ also serves as a good choice.


% \subsection{Experiment setup} We compare the performance of our proposed algorithm, \privGA{}, against the baseline mechanism in different settings over different differential privacy levels. A critical parameter that significantly influences the performance is the number of adaptive epochs $T$, as described in the adaptive framework algorithm \ref{alg:adaptive}.

% To evaluate the performance of the algorithms, we try different values of $T$ for each algorithm in our experiments and report the best error for each $\varepsilon$ value. To allow for a fair and accurate comparison of the algorithms, we provide a detailed description of how the results were computed, including specific settings or parameters, such as the different values of $T$ we tried.

% \begin{table}[h]
%     \centering
%     \begin{tabular}{c|c}
%          \privGA{} &  \\
%          \acsmobility & 25, 50, 75, 100 
%          Prefix
%     \end{tabular}
%     \caption{Number of adaptive epoch for each setting}
%     \label{tab:my_label}
% \end{table}

% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=0.7\linewidth]{images/acsreal_max_avg_error.png}
%     \caption{Max and average error evaluated on \acsrealdata{CA} with non-differentiable queries---150K random halfspaces and 200K random prefixes. 
%     \rap{} and \gem{} are trained with $3$-way range queries.
%     We fix $\delta={1/N^2}$ and vary $\varepsilon\in\{0.07, 0.23, 0.52, 0.74, 1.0\}$. Results are averaged over 3 runs.}
%     \label{fig:errors_acsreal}
% \end{figure}

\input{Figures/prefix}
\input{Figures/halfspace}


\subsection{Early Stop} \label{sec:earlystopMain}
In all experiments, \GSD{} is set to operate over a maximum of $G$ generations but uses an early-stop rule if convergence in optimizing the objective is achieved. This procedure saves computational time and the details  are found in   \cref{sec:earlystopAppendix}.


\subsection{Results}
%
% Figure \ref{fig:income_prefix_errors} shows how our method offers significant improvement over both {\em average} and {\em max} error, especially over {\em max} error.
%
% Figure \ref{fig:income_prefix_errors} shows that while \rappp{} fails to optimize over {\em max} error, \privGA{} shows good performance on both {\em average} and {\em max} error. Moreover, \privGA{} offers a significant improvement for average error over all privacy parameter $\varepsilon$ and over the two datasets we tried.  

We now present empirical results comparing \privGA{} to various baseline methods. For our experiments, we fix $\delta=\frac{1}{N^2}$ and $\varepsilon\in\{0.07, 0.23, 0.52, 0.74, 1.0\}$ to examine the trade-off between privacy and accuracy. For adaptive algorithms, we run using adaptive epochs $T \in \{25, 50, 75, 100\}$ and report the best error (averaged over 3 runs) for each $\varepsilon$ value.

First, we provide empirical evidence that \privGA{} is a better algorithm for generating real-valued synthetic data (i.e., when the statistical queries are non-differentiable). As originally shown in \citet{vietri2022private}, Figures \ref{fig:errors_prefix} and \ref{fig:errors_halfspace} demonstrate that \rappp{}, the previous state-of-the-art method, can optimize over prefix and halfspace queries using a surrogate differentiable approximation in combination with temperature annealing. However, by directly optimizing over such objectives using zeroth order optimization, \privGA{} significantly outperforms \rappp{} with respect to max and average error. 

Next, we show that on discretized data (both categorical and mixed-type), \privGA{} mechanism performs equally as well as prior work \rp{}, \gn{} and \pgmem. In Figures \ref{fig:oneshot_2way_cat} and \ref{fig:ada_3way_cat}, we evaluate on categorical marginals, which are one of the primary focuses of \rp{}, \gn{} and \pgm{}.\footnote{We note that \pgm{} cannot be run with the one-shot mechanism since the size of graphical model becomes to large.} In addition, we evaluate on binary-tree queries in Figure \ref{fig:oneshot_2way_bt}. We note that for \rp{} and \gn{}, we discretize the data in such a way that the resulting bins align with the intervals comprising our binary-tree marginal queries, allowing us to also write differentiable forms of such queries for \rp{} and \gn{}.
%
Nevertheless, we observe that \privGA{} is able to synthesize both categorical-only (for categorical marginals) and mixed-type (for binary-tree marginals) data that matches the performance of the three baseline algorithms. Moreover, unlike the baseline methods, \privGA{} does not require that the numerical features be discretized first when optimizing over binary-tree marginal queries.


\input{Figures/oneshot_categorical}

\input{Figures/oneshot_ranges}

\input{Figures/adaptive_3way_categorical}


==> icml_ready/docs/intro.tex <==
\section{Introduction}

% \color{red}

% \subsection{Text TODO}

% \begin{itemize}

%     \item Reduce text about history of synthetic data:
%     \item   how the algorithm handles columns of different variance. Show how crossover handles this naturally.
%     \item  Add oracle theorem 
%     \item Describe in text time-based early stop.
% \end{itemize}

% \subsection{experiments TODO}
% TODO:
% \begin{enumerate}
%     \item Compare PrivGA vs GEM/RAP on mixed data. 
%     \item Implement RAP++ for range queries and prefix queries.
%     \item Estimate conditional halfspaces. Compare against RAP++.
%     \item Parameter analysis of PrivGA and RAP. Add a plot of error vs runtime.
%     \item Multi-task machine learning .
% \end{enumerate}

% \paragraph{Other ideas:} A list of other features we could include:
% \begin{enumerate}
%     \item Logistic regression queries: Answer a bunch of logistic regression queries with objective perturbation and project using PrivGA. 
%     \item Add fairness constraints. A model trained on synthetic data should be fair.
% \end{enumerate}


% \subsection{Main document plot list}
% \begin{enumerate}
%     \item Categorical-marginals plot for only one task (mobility). This plot includes PrivGA, RAP, GEM and PGM.
%     \item Range-marginals for 5 tasks. This plot includes PrivGA, RAP, GEM, PGM and RAP++.
%     \item 
% \end{enumerate}

% \color{black}
 
% In this work, we consider the problem of generating synthetic data under differential privacy \citep{dwork2006calibrating} with a focus on answering a large collection of statistical queries. 
% Some approaches to producing synthetic data follow the generative adversarial network (GAN) framework due to  \citep{goodfellow2014generative}. Private implementations of the GAN framework are based on private-stochastic gradient descent (DP-SDG)  (see \citep{}). However, these methods do not perform well in practice \gv{why?}. In this work, we consider a different paradigm that consists of allocating the privacy noise to answer a selected collection of statistical queries and then finding a synthetic dataset consistent with the query answers. 
%
% The problem of releasing statistics subject to privacy has been extensively studied \citep{MWEM}.

% Introduce the problem
Access to high-quality data is critical for decision-making and data analysis. However, the reliance on sensitive data can reveal private information about the individuals in the data, such as medical conditions or financial status. Therefore, privacy concerns impose legal and ethical constraints on what one can access for data analysis. \emph{Differential privacy} \citep{dwork2006calibrating} has become an increasingly popular framework  for protecting sensitive information by providing a formal privacy guarantee that allows one to calibrate the trade-off between privacy and accuracy. Moreover, differentially private synthetic data has become especially attractive, given that such data can be accessed repeatedly without added privacy costs. Consequently, we focus on the problem of generating synthetic data that approximates various properties of the underlying sensitive dataset while providing privacy guarantees. 

A standard approach to this problem is to find a synthetic dataset that matches a large family of statistics derived from the underlying dataset. In this work, we focus on statistics in the form of  \textit{statistical queries}, which count the fraction of examples that satisfy some specific properties. This approach is often framed as synthetic data for \textit{private query release}, where the goal is to release answers to an extensive collection of statistical queries by outputting a synthetic dataset from which answers are derived from. There exists a long line of research studying synthetic data for private query release \citep{BLR08, MWEM, dualquery, HDMM, FEM, mckenna2019graphical, aydore2021differentially, liu2021leveraging, liu2021iterative}. Moreover, when the set of statistical properties is sufficiently rich, this approach has been shown to outperform differentially private deep generative models (e.g., GANs) in both capturing various statistical properties and enabling downstream machine learning tasks \citep{tao2021benchmarking, vietri2022private}. 

% Recently, \citet{vietri2022private} has framed this type of method as a class of \textit{moment-matching} approaches.\footnote{In their framing, the process of optimizing synthetic data generators over statistical query answers is used for producing high-quality, multipurpose synthetic samples, rather than for simply releasing the raw statistical query answers themselves.} 
%
Even though the problem of generating synthetic data for private query release is shown to be computationally intractable in the worst case \citep{hardsynthetic, ullman2013answering},  there has been a line of work on practical algorithms that can perform well on real datasets \citep{dualquery, FEM, mckenna2019graphical, liu2021leveraging}. Before our work, the algorithms that achieve state-of-the-art performance all leverage gradient-based optimization \citep{liu2021iterative, vietri2022private} to minimize the error for certain classes of statistical queries. However, these methods require differentiability, severely limiting the types of statistical properties one can optimize. For example, existing algorithms such as \rap{} \citep{aydore2021differentially} and \gem{} \citep{liu2021iterative} focus specifically on using first-order mechanisms for approximating marginal queries that apply to discrete data only, requiring real-valued attributes be discretized first. 

% In general, this discretization approach can be computationally expensive, particularly when a high resolution of the real-value features is required and the data contains many real-valued features. 
% For example, if $b$ bins are used to discretize $r$ real-valued columns, the resulting discretized dataset will have a dimension of $b \cdot r$. 
% Additionally, discretization is limited in terms of the types of queries one can optimize for. In this work, we focus on answering random halfspace and prefix queries, which would be impossible to discretize to such a fine granularity for.

Many natural classes of queries for data containing real-valued attributes are non-differentiable, such as prefixes (equivalently the CDF of an attribute), and their higher-dimensional extension, halfspaces. Moreover, these queries cannot be optimized directly by methods that operate over discrete data, even with the discretization of real-valued features. \citet{vietri2022private} circumvent discretization by approximating non-differentiable queries with differentiable surrogate functions. Thus, their approach, \rappp{}, can directly optimize over a large class of statistical queries. However, their method induces additional error due to the relaxation of the original minimization problem, which may not produce an optimal solution for the original one. \footnote{
In Appendix \ref{appx:rappp}, we show a simple example in which the continuous relaxation leads \rappp{} to a bad local minimum very far from the optimal solution}
\footnote{\cref{fig:badexample} gives a simple example where \rappp{} fails to optimize a set of $3$ prefix queries on $1$-dimensional real-valued data.}

% \footnote{A {\em marginal} query is a function that counts the fraction of rows in a dataset where a particular set of attributes matches specific values. For example, a marginal query is: "How many people in dataset $D$ are Asian and live in NYC."}

In light of these challenges, we propose a new synthetic data generation algorithm, \privGA{}, that is capable of outputting \textit{mixed}-type data (i.e., containing both discrete and real-valued attributes) without requiring differentiability in its optimization objective or discretization of real-valued attributes. \privGA{} is a zeroth-order mechanism based on a genetic algorithm that avoids the limitations of first-order methods such as \rappp{}, which uses surrogate loss functions to ensure differentiability. Instead, \privGA{} can optimize the error objective directly. Inspired by the genetic algorithm $\simpleGA$ \citep{such2017deep}, our algorithm \privGA{} evolves a population of datasets over $G$ generations---starting from a population of $E$ randomly chosen datasets, where on each generation, the algorithm maintains a set of elite synthetic datasets. Then, the algorithm uses this elite set to produce the population for the next round by crossing samples (i.e., combining parameters) and applying specific mutations (i.e., perturbing parameters). For the purpose of private synthetic data, we devise new strategies for crossing and mutating samples.  To illustrate the limitations of the first-order approach \rappp{} and how \GSD{} overcomes them, we provide a simple example in \cref{fig:badexample}, where both algorithms try to approximate a target distribution over real values.

\input{Figures/rap++_bad_example}

Moreover, given that our method only requires zeroth-order access to any objective function, we demonstrate that \privGA{} can directly optimize over a wide range of statistical queries that capture various statistical properties summarizing both discrete and real-valued data attributes. Specifically, we first conduct experiments in mixed-type data domains, evaluating on random (1) halfspace and (2) prefix queries. We then explore categorical-only data, in which we use (3) $k$-way categorical marginal queries. Lastly, we again evaluate \privGA{} on mixed-type data using (4) $k$-way \emph{binary-tree marginal} queries (defined in \cref{sec:experiments}). Note that (3) and (4) can be represented as differentiable functions, while (1) and (2) cannot.

We summarize our contributions\footnote{While not the primary focus of our work, we provide ML evaluation experiments in \cref{appx:mleval}} as the following:
%
\begin{itemize}
    \setlength{\itemsep}{0pt}
    \setlength{\parskip}{0pt}
    \item We present \privGA{}, a versatile genetic algorithm that can generate synthetic data to approximate a wide range of statistical queries, regardless of their differentiability. To achieve this, we develop novel crossover and mutation functions that are crucial to the efficacy of \privGA{}.
    \item We conduct an empirical evaluation on data derived from the American Community Survey. We note that our method is highly parallelizable, scaling to the high-dimensional data settings explored in our experiments.
    \item In the mixed-type data domain, we show that \privGA{} outperforms the state-of-the-art method, \rappp{}, on non-differentiable queries (i.e., halfspace and prefix queries). Furthermore, we show that \emph{even} for differentiable query classes (i.e., $k$-way categorical and binary-tree marginals), \privGA{} matches first-order optimization methods.\footnote{Our work is also the first to modify our baseline methods, \rap{} and \gem{}, to optimize over $k$-way binary-tree marginals for mixed type data, with the limitation being that real-valued attributes are discretized first.}
\end{itemize}

\paragraph{Additional related work.}
\iffalse
% Introduce early synthetic data mechanisms  
 \smallDB{} \citep{BLR08}, one of the first private synthetic data mechanisms, searches the space of small datasets consistent with the original data schema and selects the dataset that best matches the answers on the original dataset. However, \smallDB{} is computationally intractable as it needs to enumerate the search space of all possible small datasets, which is exponential in the data dimension. A more practical approach, proposed in \citet{MWEM}, is the Multiplicative-Weights-Exponential-Mechanism (\mwem) with optimal sample complexity for the query release problem. The \mwem{} algorithm is more practical than \smallDB{} but is still computationally intractable for data dimensions commonly found in real-world datasets. 
 % Describe the history of Oracle efficient mechanisms
 \dualquery{} \citep{gaboardi2014dual} and \fem{} \citep{Vietri2019NewOA} can be viewed as efficient versions of \mwem{}, where the computationally hard step is replaced by a practical optimization heuristic. Both \dualquery{} and \fem{} have worse sample complexity than \mwem{} but are more scalable for higher dimensional data.\fi

  % is the \smallDB{} algorithm by \citet{BLR08}.  \smallDB{} \citep{BLR08}, one of the first private synthetic data mechanisms, searches the space of small datasets consistent with the original data schema, then runs a differentially private mechanism to select the small dataset that best matches the answers on the original dataset. As a result, the \smallDB{} algorithm can accurately answer exponential in $n$ many statistical queries, whereas the Gaussian mechanism only answers $O(n^2)$ queries. However, the issue with \smallDB{} is that it is computationally intractable as it needs to enumerate the search space of all possible small datasets, which is exponential in the data dimension. A more practical approach, proposed in \citet{MWEM}, is the Multiplicative-Weights-Exponential-Mechanism (\mwem) with optimal sample complexity for the query release problem. The \mwem{} algorithm is more practical than  \smallDB, but it is still computationally intractable for high enough dimensional data. The reason is that \mwem{} must maintain a probability distribution over the data domain, which is exponentially large in the number of attributes in the data.

% PGM
In addition to algorithms \rap{}, \gem{}, and \rappp{} \citep{aydore2021differentially, liu2021iterative, vietri2022private}, another benchmark algorithm that uses first-order optimization is the PrivatePGM (\pgm{}) algorithm \citep{mckenna2019graphical} and its variations \citep{mckenna2022aim}.  Similar to \rap{} and \gem{}, \pgm{} does not directly does not support non-differentiable queries such as thresholds and half-spaces on real-valued data. While one can first discretize numerical features, \citet{vietri2022private} show that \rappp{} still performs better than \pgm{} on real-valued data for approximating prefix queries and downstream machine learning. Finally, there is a line of work \citep{XieLWWZ18, JordonYvdS18, gan2, gan3, vae, harder2021dp} that develops differentially private algorithms for training deep generative models (e.g., GANs, VAEs, etc.), but they generally have not shown promising results for enforcing consistency with simple classes of statistics when applied to tabular data \citep{tao2021benchmarking, vietri2022private}.


\iffalse
\paragraph{Limitations of data discretization.}
Discretizing real-valued features and running a suitable method can produce high-quality results in specific scenarios. However, this approach has its limitations. Discretization can be computationally expensive, particularly when a high resolution of the real-value features is required and the data contains many real-valued features. 
% For example, if $b$ bins are used to discretize $r$ real-valued columns, the resulting discretized dataset will have a dimension of $b \cdot r$. 
Additionally, discretization is limited in terms of the types properties one can optimize for. In this work, we focus on answering a random halfspace and prefix queries, which would be impossible to discretize to such a fine granularity for.
% Another class of queries, halfspace queries, which capture linear properties of the real-valued features, cannot be directly encoded by discretization even with infinite granularity. 
% Therefore, discretization is a reasonable strategy for some settings but may not be the best solution for all types of queries and problems.


\paragraph{Limitations of a recent first-order approach for real-valued data.}
For data with real-valued features, a common task is to approximate prefix queries\footnote{An example of a prefix query is: "How many people in dataset $D$ have a salary less than $10K$".} under differential privacy. Recently, \citet{vietri2022private} introduces a first-order algorithm \rappp{} for preserving any threshold-based queries, including prefix queries, and operates over real-valued data by using a differentiable relaxation of the optimization problem. However, the relaxation step introduces a new source of error, potentially leading to catastrophic outcomes in which the the algorithm find a local minimum very far from the optimal solution.\footnote{We provide a simple example in Appendix \ref{appx:rappp}.}
\fi
% \input{docs/rap++_v2}





==> icml_ready/docs/ml_study.tex <==

\section{ML Evaluation}\label{appx:mleval}
This section critically assesses the utility of synthetic data in training machine learning models. We explore two main parameters in our investigation: the choice of mechanisms, such as \GSD{} or \rappp, and the selection of statistics to match, including categorical marginals, Binary Tree, or Halfspace queries.

We direct our attention toward datasets that encapsulate multiple classification tasks concurrently. To this end, we construct a multitask dataset that amalgamates all five predictive tasks outlined in \cref{fig:MLf1} by combining all feature and target columns. The learning challenge presented by a multitask dataset involves developing separate models, each predicting one of the target columns based on the feature columns. We exclude the employment task because its target is highly correlated with feature from another tasks, making the prediction problem trivial. Thus, the multitask dataset incorporates 25 categorical features, nine numerical features, and four binary target labels.

We initiate the experiment by dividing each dataset into a training and test set, using an 80/20 partition. The training set is subsequently processed by a private mechanism to produce a synthetic dataset that we use to train a logistic regression model. Lastly, the performance of the model is evaluated on the test data using the F1 metric. The F1 metric considers both precision and recall, providing a balanced assessment of model performance, particularly when dealing with imbalanced datasets. It is calculated as the harmonic mean of precision and recall, with a potential range from $0$ to $1$, wherein a higher score denotes superior model performance.

Our results are tabulated in Table ML and showcase the F1 score for predicting four target labels using logistic regression trained on various synthetic data methodologies alongside the F1 score of a logistic regression model trained on the original training data. The findings suggest that the \GSD{} mechanism coupled with Binary-Tree queries is a favorable choice among the other synthetic data baselines examined in this experiment. However, we note that the F1 scores of all private synthetic data methodologies are inferior to the model trained on the original data, even in a low privacy regime (i.e., $\epsilon=1$).

The question of why synthetic data does not get better performance in training ML models remains an open area of exploration. One conjecture is that we have yet to identify the right set of data properties (or statistical queries) that can be used to generate high-quality synthetic data for machine learning applications. However, we posit that the \GSD{} mechanism is well-equipped to tackle this challenge due to its inherent ability and flexibility in managing diverse queries. 

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.7\linewidth]{images/ML_f1.png}
    \caption{
    \textbf{Machine Learning Evaluation: } F1 test score of logistic regression trained on synthetic data. Each ACS dataset is partitioned into training and testing set, using an 80/20 split. The train set is used to train the synthetic data algorithm, and the F1 score is computed using the test set.
    Each algorithm is trained either on Binary Tree (BT) marginal queries or Halfspace (HS) queries.   We fix $\delta={1/N^2}$ and vary $\varepsilon\in\{0.07, 0.23, 0.52, 0.74, 1.0\}$. Results are averaged over 3 runs. }
    \label{fig:MLf1}
\end{figure}

% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=0.7\linewidth]{images/ML_acc.png}
%     \caption{
%     \textbf{Machine Learning Evaluation: } Accuracy test score of logistic regression trained on synthetic data. Each ACS dataset is partitioned into training and testing set. The train set is used to train the synthetic data algorithm, and the accuracy score is computed using the test set.
%     Each algorithm is trained either on Binary Tree (BT) marginal queries or Halfspace (HS) queries.   We fix $\delta={1/N^2}$ and vary $\varepsilon\in\{0.07, 0.23, 0.52, 0.74, 1.0\}$. Results are averaged over 3 runs. }
%     \label{fig:MLaccuracy}
% \end{figure}

==> icml_ready/docs/prelims.tex <==


\section{Preliminaries}\label{sec:prelims}



\subsection{Datasets and Queries }
Let's consider $\cX$ as a data domain of dimensionality $d$. Here, each element $x\in \cX$ is an observation within this data domain. For any given observation $x\in \cX$, we refer to its $i$-th feature as $x_i\in \cX_i$. The feature domain associated with this $i$-th feature is denoted by $\cX_i$. We define a dataset $D$ as a multiset of observations derived from the data domain $\cX$, where $D\subseteq \cX^*$. Often, to ensure a convenient representation of categorical features, we employ the one-hot encoding approach. In this context, one-hot encoding portrays a categorical value as a binary vector where all elements, barring the one corresponding to the category, are set to zero. We introduce $h_{oh}:\cX\rightarrow[0,1]^{d'}$ to denote the function that maps elements of $\cX$ to their one-hot encoding, with $d'$ representing the dimensionality of the one-hot encoded space. Finally, for any discrete set $S$, we define $U(S)$ as the uniform distribution over this set $S$. A random sample from $U(S)$ can be represented as $s\sim U(S)$. For any integer $i$, we use $[i]={1,\ldots,i}$ to represent the set of all integers from $1$ to $i$.

In this research, our focus lies on mixed-valued datasets within a bounded domain, with a particular emphasis on answering statistical queries. A statistical query is defined as a function $q:\cX^* \rightarrow [0,1]$ that maps a dataset to a value within the bounded interval [0,1]. The formal definition of a statistical query in this context is
\begin{definition}[Statistical Query \citep{kearns1998efficient}]
    A \emph{statistical query} is defined by a predicate function $\phi:\cX\rightarrow\{0,1\}$. Given a dataset $D\in \cX^N$, the corresponding statistical query $q_\phi$ is defined as : $q_\phi(D) = \frac{1}{N}\sum_{x\in D} \phi(x)$. 
\end{definition}



We use $Q=\{q_i, \ldots, q_m\}$ to represent a set of $m$ statistical queries and for a given dataset $D$.
Furthermore, for convenience,  we use
$Q(D) = [q_1(D),\ldots, q_m(D)] \in [0,1]^m$ to denote the answers of all $m$ statistical queries on $D$. 

In this work, we are interested in answering different types of statistical queries that capture different statistical properties. The first type is the class of categorical marginals, which has been the primary focus of most prior works. The \emph{$k$-way categorical marginal} queries count the fraction of rows in a dataset that matches a combination of values.

% capture the relationship between categorical features. 

% \begin{definition}[Categorical marginals ]
% \end{definition}
\begin{definition}[Categorical Marginal Queries]\label{def:cat_marginals}
A $k$-way \textit{categorical marginal} query is defined by a set of categorical features $S$ of cardinality $|S|=k$, together with a particular element $c\in \prod_{i\in S} \cX_i$ in the domain of $S$.  Given such a pair  $(S, c)$, let $\cX(S, c)=\{x \in \cX : x_S = c \}$ denote the set of points that match $c$. The corresponding statistical query $q_{S, c}$ is defined as $q_{S,c}(D) = \sum_{x\in D}\mathbbm{1}\{x\in \cX(S, c)\}$, 
% \begin{align*}
%     q_{S,c}(x) = \mathbbm{1}\{x\in \cX(S, c)\}.
% \end{align*}
where $\mathbbm{1}$ is the indicator function.
\end{definition}

For real-values features, we define the class of \emph{range} queries or \emph{$k$-way range-marginals} that capture the $k$.  A $1$-way range query is defined by an attribute $A$ and two real-values $a, b\in [0,1]$ and counts the number of rows where real-valued attribute $A$ lies in $[a, b]$.

% \begin{definition}[ Range marginals ]
% \end{definition}
\begin{definition}[Range Marginal Queries]\label{def:range_marginals}
 A $k$-way \textit{range marginal} query is defined by a set of categorical features $C$, an element $y\in \cX_C$, a set of numerical features $R$ and a set of intervals $\tau=\{[\tau_{j,0}, \tau_{j,1}]\}_{j\in R}$, with $|C| + |R| = k$ and $|R| = |\tau|$.
Let $\cX(C, y)$ be as in \cref{def:cat_marginals} and let $\cR(R, \tau) =\{x\in\cX : \tau_{j, 0} \leq x_j \leq \tau_{j, 1} \quad \forall_{j\in R}\}$ denote the set of points where each feature $j\in R$ fall below its corresponding threshold value $\tau_j$.
% and $\cX(R, \tau)$ be as in \cref{def:prefix}.
Then the statistical query $q_{C, y, R, \tau}$ is defined as $$    q_{C, y, R, \tau}(D) =\sum_{x\in D} 
   \mathbbm{1}\{x\in \cX(C, y) \} \cdot   \mathbbm{1}\{x\in \cR(R, \tau) \} .$$ 
% The corresponding statistical query is defined by a component-wise product of a marginal vector $\mu_{C, x} $ (defined in \cref{def:marginals}) and a prefix marginal query: 
% \begin{align*}
%     q_{C, y, R, \tau}(x) = 
%   \mathbbm{1}\{x\in \cX(C, y) \} \cdot   \mathbbm{1}\{x\in \cX(R, \tau) \} .
%     % \mu_{C, x} \cdot   \prod_{i\in R}\mathbbm{1}\{ x_i \leq \tau(i) \}
% \end{align*}
\end{definition}

We note that while range marginal queries are useful for capturing statistical properties of real-valued data, they can also be applicable to discretized data. For example, one can discretize a real-valued column into the bins that are a superset of the intervals $\tau$ defined in Definition \ref{def:range_marginals}.\footnote{In Section \ref{sec:experiments} and the appendix, we will discuss how range marginal queries are still applicable to \gem{} and \rap{}, which handle real-valued attributes by discretizing them first.}




Next, we present two additional queries---halfspace and prefix queries---that are also useful in summarizing real-valued features. We emphasize that such queries are the focus of our work, since they cannot be directly optimized by existing methods using first-order optimization. These queries can in some ways be thought of as higher-dimensional generalizations of CDF functions. Moreover, synthetic data matching statistical properties defined by these queries have been shown to do well on downstream tasks like machine learning classification \citep{vietri2022private}.

% \begin{definition}[Halfspace Query]\label{def:halfspace}
% A \textit{halfspace} query is defined by a categorical feature $i$,
%  a target value  $y\in\cX_i$,
% a set of numerical features $R$,  a vector $\theta\in\mathbb{R}^{|R|}$ and a threshold $\tau\in \mathbb{R}$ as $    q_{i, y, R, \theta, \tau}(D) =\sum_{x\in D}  \mathbbm{1}\{\dotp{\theta, x_R} \leq \tau \text{ and } x_i = y\} .$
% \end{definition}
\begin{definition}[Halfspace Query]\label{def:halfspace}
% Let $h_{oh}:\cX\rightarrow[0,1]^{d'}$ be a function that maps elements of $\cX$ to their one-hot encoding. 
A \textit{halfspace} query is defined by
a vector $\theta\in\mathbb{R}^{d'}$ and a threshold $\tau\in \mathbb{R}$. The \emph{halfspace} query is given by $q_{ \theta, \tau}(D) =\sum_{x\in D}  \mathbbm{1}\{\dotp{\theta, h_{oh}(x)} \leq \tau\}$, where 
$h_{oh}:\cX\rightarrow[0,1]^{d'}$ is the function that maps elements of $\cX$ to their one-hot encoding. 
\end{definition}


\begin{definition}[$k$-way prefix queries]\label{def:prefix}
A $k$-way prefix query is defined by a set of real-valued features $C\subseteq [d]$ ($|C|=k$) and a set of threshold $\tau=\{\tau_i \in [0,1]: i\in C\}$. Let $\cX(C, \tau) =\{x\in\cX : x_i\leq \tau_i \quad \forall i\in C\}$ be the set of points, that has each feature $i\in C$ fall below the corresponding threshold $\tau_i$. Then the prefix query $q_{C, \tau}$ is given by $q_{C, \tau}(D) = \sum_{x\in D} \mathbb{I}\{x\in \cX(C, \tau)\}$.
\end{definition}

% Finally, our goal is to accurately estimate statistical queries according to $\ell_{\infty}$, $\ell_2$ and $\ell_1$ error:
% \begin{definition}
% Let $D\in \cX^n$ be a dataset and $Q$ be a set of statistical queries. Then the $\ell_p$-error of a synthetic dataset $\Dhat^{n'}$ is $\|Q(D) - Q(D')\|_p$.
% \end{definition}






\subsection{Differential Privacy} 
% The fundamental problem we address in this paper is releasing the statistics $Q(D)\in [0,1]^m$ when the dataset $D$ may contain sensitive information.  
To protect user privacy, we estimate $Q(D)$ under the constraint of differential privacy \citep{dwork2006calibrating}, which is a widely accepted notion of privacy protection at the user level. 
% Differential privacy allows one to control the trade-off between how much one can learn about a population and how much data leakage is acceptable on the user level. 
For example, the US Census Bureau has begun using differential privacy to protect the privacy of individuals when releasing census data. Differential privacy is used to add noise to the census data in order to obscure the data of any one individual, while still providing accurate statistical information about the population as a whole.

To define differential privacy, we say that two datasets are neighboring if they are different in at most one data point. We give the formal definition here:
\begin{definition}[Differential Privacy (DP) \citep{dwork2006calibrating}]\label{def:dp}
A randomized algorithm $\mathcal{M}:\cX^N\rightarrow \cR$ satisfies $(\varepsilon, \delta)$-differential privacy if 
for all neighboring datasets $D, D'$ and for all outcomes $S\subseteq \cR$ we have
%
\begin{align*}
    \pr{\mathcal{M}(D) \in S} \leq e^{\varepsilon} \pr{\mathcal{M}(D') \in S}+\delta
\end{align*}
\end{definition}

A related notion we use is {\em zero-Concentrated Differential Privacy} (zCDP) \citep{DworkR16, BunS16}, which has a simpler privacy composition.

\begin{definition}[zCDP \citep{bun2016concentrated}]\label{def:zcdp}A randomized algorithm $\mathcal{M}:\cX^N\rightarrow \cR$ satisfies $\rho$-zero-Concentrated differential privacy ($\rho$-zCDP) if 
for all neighboring datasets $D, D'$ and for all $\alpha\in(1,\infty)$ we have: $\mathbb{D}_{\alpha}(\mathcal{M}(D),\mathcal{M}(D'))\leq\rho\alpha$, where $\mathbb{D}_{\alpha}(\mathcal{M}(D),\mathcal{M}(D'))$ is $\alpha$-Renyi divergence between the distributions $\mathcal{M}(D)$ and $\mathcal{M}(D')$.
\end{definition}


% \begin{lemma}[\citet{dong2020optimal}]
%     For any vector of statistical queries $q$, vector of conjectured answers $a$, and zCDP parameter $\rho$, $RNM(\cdot,q,a,\rho)$ satisfies $\rho$-zCDP.
% \end{lemma}

% \paragraph{ML Queries}  Our algorithm takes as input a finite collection of statistical queries and a dataset $D$. Prior work on efficient private-synthetic-data generation required queries to be either marginal queries \citep{mckenna2019graphical, mckenna2022aim} or that the queries are differentiable in the data domain \citep{vietri2022private, aydore2021differentially, liu2021iterative}. In contrast, our mechanism can operate over a general class of statistical queries and is efficient for high-dimensional data domains. 

% We choose a class of queries consisting of random binary tree classifiers for our experiments. We denote it by $Q_{\text{tree}}$. Any query $q\in Q_{\text{tree}}$ maps a rows of data $x\in \cX$ to a random binary label $\{0,1\}$. By choosing a large set of queries, many will likely be good discriminators of real and synthetic data. Even though we choose specifically binary tree classifiers, our mechanism operates over any class.




% \paragraph{Downstream Applications:}
% A central tenet machine learning task is the ability learn models that generalize. However, in practice training machine learning models is an iterative process that that involves reusing the same dataset multiple times. Therefore, to validate the generalization properties of a machine learning algorithm, the typical practice is to separate a fraction of the dataset for evaluation. 
% Given a synthetic dataset we 
% We define a machine learning task by a triple $(\Dtrain ,\Dtest, \cH)$, where $\cH$ is a hypothesis space.. Then, the training is as follows: On each round $\in [T]$ a




% \paragraph{Techniques} Our techniques include a synthetic data algorithm that efficiently optimizes over a general class of statistical queries. Prior work in synthetic data generation can only answer either marginal queries or queries that can be expressed in a differentiable form, see \citep{aydore2021differentially, liu2021iterative, mckenna2019graphical, mckenna2022aim, Vietri2019NewOA, gaboardi2014dual}.

% Furthermore, we implement our mechanism to satisfy differential privacy and take advantage of the \emph{transfer theorem} due to \citep{jung2019new} to preserve generalization. We use the Gaussian mechanism with the sparse vector technique for the privacy implementation.




==> icml_ready/docs/query_release_problem.tex <==
\section{Private Query Release via Synthetic Data} \label{sec:projmech}

For the problem of estimating statistics $Q(D)$ subject to differential privacy, we follow the framework of the projection mechanism \citep{NKL, DworkNT15}, which consists of perturbing the statistics with a differentially private mechanism followed by a \emph{projection step} that consists of finding a synthetic dataset that matches these perturbed statistics.

In this study, we consider two versions of the private projection mechanism. The first is the standard projection mechanism, referred to as the \emph{one-shot} version. The second is an \emph{adaptive} version of the projection mechanism, which proves useful in scenarios where a large number of queries are required. A comprehensive description of both frameworks is presented below.

\paragraph{One-shot projection mechanism:}
Suppose we are given $m$ statistical queries, represented by $Q$, and a dataset $D$. Then the first step consists of independently perturbing every coordinate of $Q(D)$ to obtain a private estimate, denoted by $\hat{a}$. Given a privacy parameter $\rho$, the noisy answer vector is computed as follows:
\begin{align}\label{eq:gaussianmech}
    \hat{a} \leftarrow Q(D) + \cN\pp{0, \tfrac{\Delta(Q)}{2\rho}\cdot \mathbb{I}}
\end{align}


Then, the \emph{project} step involves finding a synthetic dataset $\Dhat$ that best explains the estimate $\hat{a}$. To represent the projection step, we construct a loss minimization problem, where the loss function is defined by $\hat{a}$ and $Q$ as follows:
\begin{align}\label{eq:obj}
 L_{\hat{a}, Q} (\Dhat) =   \|\hat{a} - Q(\Dhat) \|_2^2
\end{align}


By the properties of the Gaussian mechanism and the post-processing property (Theorem \ref{lemma:post}), the projection mechanism framework satisfies  $\rho$-zCDP regardless of the optimization procedure used to solve \eqref{eq:obj}.

% \input{Arxiv/algorithms/privga.tex}



\paragraph{Adaptive selection framework:} In practice, when the number of queries $m$ is very large, the objective \eqref{eq:obj} becomes extremely noisy for any practical optimization routine. Therefore, we follow the Adaptive Selection Framework of \citet{liu2021iterative} that, over $K$ rounds, chooses high error queries adaptively using  the report noisy max mechanism (alternatively the exponential mechanism, as defined in Definition \ref{def:exponential}). Algorithm \ref{alg:adaptive} of Appendix \ref{appx:adaptive} shows the details of this framework, which we note satisfies the following theorem:


\begin{theorem}\label{thm:privacy} For any $K$, $\rho>0$, dataset $D$, query set $Q$ and any procedure used to solve objective \eqref{eq:obj},  the adaptive framework  strategy satisfies $\rho$-zCDP. By extension, it also satisfies $(\varepsilon, \delta)$-differential privacy for: $\varepsilon = \rho+2\sqrt{\rho\cdot \log(1/\delta)}$.
\end{theorem}

We provide a proof sketch to \cref{thm:privacy} below in \cref{appx:privacyproof}.

==> meeting_notes.tex <==
\section{Meeting notes:}


\paragraph{July 14:}

\begin{itemize}
     \item Find a setting such that the naive mechanism fails. How many rounds should we try? how many samples for train and test? What kind of discriminator should we use (Linear, Random Forest, Neural network)?
     \item We found out that a strategy that uses linear models to find queries is able to find high error queries in the interactive setting against a naive mechanism. 
     \item Once we have a strategy that defeats a naive mechanism, we should compare against online-MW. 
    \item Optimize runtime: We could optimize query manager by not re-initializing every round. 
\end{itemize}

==> tables/population_size.tex <==
% \begin{table}[]
%     \centering
%     \begin{tabular}{c c | c c c c c c c c c}
%     \toprule
%     & & \multicolumn{9}{c}{Run time in Seconds by Population Size} \\ 
%        \text{Dataset}  & \text{Queries} & \text {5}  & \text {10} &\text {20} &\text {40} &\text {80} &\text {160} &\text {320} &\text{640}&\text{1280} \\
%          \midrule 
%     \multirow{2}{*}{Travel} & \multirow{2}{*}{438594}  &  1887  &  1138  &  \textbf{654}  &  816  &  650  &  729  &  1164  &  1662  &  2920 \\
%   &   &  1887  &  1138  &  \textbf{654}  &  816  &  650  &  729  &  1164  &  1662  &  2920 \\
% Income & 274641  &  1129  &  800  &  424  &  \textbf{281}  &  435  &  451  &  540  &  521  &  999 \\
% Mobility & 38077  &  522  &  303  &  183  &  143  &  101  &  \textbf{99}  &  107  &  176  &  258 \\
% Coverage & 15894  &  1007  &  597  &  187  &  112  &  103  &  100  &  \textbf{97}  &  97  &  145 \\
% Employment & 10570  &  1690  &  618  &  198  &  210  &  86  &  89  &  \textbf{66}  &  69  &  116 \\
% \bottomrule
%     \end{tabular}
%     \caption{\textbf{Population size effect on run time:} The table represents the run time in seconds of \GSD{} initialized with population sizes in $\{5, 10, 20, 40, 80, 160, 320, 640, 1280\}$ for optimizing the class of 2-way Binary Tree queries.   The privacy parameter  $\epsilon$ was fixed to $1$, the number of synthetic data rows was $2000$ and the number of generations $200,000$.   }
%     \label{tab:my_label}
% \end{table}


 
% \begin{table}[]
%     \centering
%     \begin{tabular}{c c | c c c c c c c c c}
%     \toprule
%     & & \multicolumn{9}{c}{Run time in Seconds by Population Size} \\ 
%        \text{Dataset}  & \text{Queries} &   & \text {10} &\text {20} &\text {40} &\text {80} &\text {160} &\text {320} &\text{640}&\text{1280} \\
%          \midrule 
% \multirow{2}{*}{ travel } 	&\multirow{2}{*}{ 438594 } 	& Time  &  458  &  467  &  554  &  657  &  740  &  1173  &  1675  &  2934 \\
% 				&				&  Error*100  &  0.48  &  0.43  &  0.39  &  0.41  &  0.41  &  0.38  &  0.36  &  0.38 \\
% \multirow{2}{*}{ coverage } 	&\multirow{2}{*}{ 15894 } 	& Time  &  206  &  123  &  116  &  109  &  101  &  102  &  100  &  148 \\
% 				&				&  Error*100  &  0.43  &  0.44  &  0.46  &  0.44  &  0.49  &  0.44  &  0.47  &  0.49 \\
% \multirow{2}{*}{ employment } 	&\multirow{2}{*}{ 10570 } 	& Time  &  144  &  139  &  108  &  91  &  94  &  68  &  72  &  119 \\
% 				&				&  Error*100  &  0.54  &  0.34  &  0.34  &  0.26  &  0.27  &  0.29  &  0.25  &  0.25 \\
% \multirow{2}{*}{ income } 	&\multirow{2}{*}{ 274641 } 	& Time  &  312  &  283  &  270  &  445  &  457  &  551  &  523  &  998 \\
% 				&				&  Error*100  &  0.36  &  0.31  &  0.31  &  0.26  &  0.26  &  0.26  &  0.23  &  0.26 \\
% \multirow{2}{*}{ mobility } 	&\multirow{2}{*}{ 38077 } 	& Time  &  184  &  168  &  141  &  107  &  104  &  109  &  180  &  261 \\
% 				&				&  Error*100  &  0.92  &  0.97  &  0.97  &  0.82  &  0.87  &  0.92  &  0.92  &  0.87 \\

% \bottomrule
%     \end{tabular}
%     \caption{\textbf{Population size effect on run time:} The table represents the run time in seconds of \GSD{} initialized with population sizes in $\{5, 10, 20, 40, 80, 160, 320, 640, 1280\}$ for optimizing the class of 2-way Binary Tree queries.   The privacy parameter  $\epsilon$ was fixed to $1$, the number of synthetic data rows was $2000$ and the number of generations $200,000$.   }
%     \label{tab:my_label}
% \end{table}


\begin{table}[]
    \centering
    \begin{tabular}{c | c c c c c c c c}
    \toprule
    & \multicolumn{8}{c}{Run time in Seconds by Population Size} \\ 
    \rotatebox{90}{Data}  \text{}  &   \text {10} &\text {20} &\text {40} &\text {80} &\text {160} &\text {320} &\text{640}&\text{1280} \\
         \midrule 
 	 T	&  0.48/(458)  &  0.43/(467)   &  0.39/(554)   & 0.41/(657)  &  0.41/(740)  &  0.38/(1173)   &  0.36/(1675)   &  0.38/(2934) \\
				% &  0.48  &  0.43  &  0.39  &  0.41  &  0.41  &  0.38  &  0.36  &  0.38 \\
  C 	&  0.43/(206)  &  0.44/(123)  &  0.46 /(116)  &   0.44 /(109)  &  0.49 /(101)  &  0.44/(102)  &  0.47/(100)  &  0.49/(148) \\
% 				&  0.43  &  0.44  &  0.46  &  0.44  &  0.49  &  0.44  &  0.47  &  0.49 \\
{ E } 	&     0.54/(144)  &  0.34/(139)  &  0.34/(108)  &  0.26/(91)  &  0.27/(94)  &  0.29/(68)  &  0.25/(72)  &  0.25/(119) \\
% 	 &  0.54  &  0.34  &  0.34  &  0.26  &  0.27  &  0.29  &  0.25  &  0.25 \\
{I }  &  0.36/(312)  &  0.31/(283)  &  0.31/(270)  &  0.26/(445)  &  0.26 /(457)  &  0.26 /(551)  &  0.23/(523)  &  0.26/(998) \\
% 		 &  0.36  &  0.31  &  0.31  &  0.26  &  0.26  &  0.26  &  0.23  &  0.26 \\
{ M } 	  &  0.92/(184)  &  0.97/(168)  &  0.97/(141)  &  0.82 /(107)  &   0.87 /(104)  &  0.92/(109)  &  0.92/(180)  &  0.87/(261) \\
% 		  0.92  &  0.97  &  0.97  &  0.82  &  0.87  &  0.92  &  0.92  &  0.87 \\

\bottomrule
    \end{tabular}
    \caption{ Study of effect of the population size parameter on the performance of \GSD. 
    The numbers represent the \emph{max} error (multiplied by $100$) for answering $2$-way range queries and, in parenthesis, it is the total runtime in seconds.
    Each row corresponds to the input dataset (\acstradata{CA} (T),
 \acscovdata{CA} (C),
 \acsempdata{CA} (E),
 \acsincdata{CA} (I), 
 \acsmobdata{CA} (M)) and the  columns correspond to the population size parameter ($\{10, 20, 40, 80, 160, 320, 640, 1280\})$.  For all runs we fixed the other parameters as follows: The privacy parameter  $\epsilon$ was fixed to $1$, the number of synthetic data rows was $2000$ and the number of generations $200,000$.   }
    \label{tab:populationsize}.
\end{table}
